Synchronous Forwarders

Session types are types for specifying protocols that processes must follow when communicating with each other. Session types are in a propositions-as-types correspondence with linear logic. Previous work has shown that a multiparty session type, a generalisation of session types to protocols of two or more parties, can be modelled as a proof of coherence, a generalisation of linear logic duality. And, protocols expressed as coherence can be simulated by arbiters, processes that act as a middleware by forwarding messages according to the given protocol. In this paper, we generalise the concept of arbiter to that of synchronous forwarder, that is a processes that implements the behaviour of an arbiter in several different ways. In a propositions-as-types fashion, synchronous forwarders form a logic equipped with cut elimination which is a special restriction of classical linear logic. Our main result shows that synchronous forwarders are a characterisation of coherence, i.e., coherence proofs can be transformed into synchronous forwarders and, viceversa, every synchronous forwarder corresponds to a coherence proofs.

==> additives.tex <==
ciao


==> app-cut.tex <==

\newcommand{\ax}[0]{\textsc{ax}}
\renewcommand{\Left}[1]{\mathcal{L}\dbr{#1}}
\renewcommand{\Right}[1]{\mathcal{R}\dbr{#1}}
\renewcommand{\Query}[1]{\mathcal{Q}\dbr{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\section{Cut-elimination Proof for Synchronous Forwarders}
\label{app:cut}

\subsection{Rules}
\begin{displaymath}
  \small
  \begin{array}{c}
    \infer[\ax]
    {A^\perp, A}
    {}
    \qquad
    \infer[\one]
    {\one, [\ast]^n}
    {}
    \qquad
    \infer[\bot]
    {\Gamma, \bot}
    {\Gamma, [\ast]}
    \\\\
    \infer[\tensor]
    {\Gamma, [\Delta_1]\Delta_2, A \tensor B}
    {\Delta_1, A \quad \Gamma, \Delta_2, B}
    \qquad
    \infer[\parr]
    {\Gamma, A \parr B}
    {\Gamma, [A] B}     
    \\\\
    \infer[\with]
    {\Gamma,\oplus\Delta,A \with B}
    {\Gamma, \Left{\oplus\Delta}A
    \quad
    \Gamma, \Right{\oplus\Delta} B}
    \qquad
    \infer[\Left]
    {\Gamma, \Left{\cdot}C}
    {\Gamma, C}
    
    \qquad
    \infer[\Right]
    {\Gamma, \Right{\cdot}C}
    {\Gamma, C}
	
    \\\\
    \infer[\oplus_1]
    {\Gamma,  \Left{\Delta, A\oplus B} C}
    {\Gamma,  \Left{\Delta} C, A}
    \qquad
    \infer[\oplus_2]
    {\Gamma, \Right{\Delta, A\oplus B}C}
    {\Gamma, \Right{\Delta} C, B}
    \\\\
    \infer[\bang]
    {\query \Delta, \bang A} 
    {\Query{\query\Delta} A}
    \qquad
    \infer[\query]
    {\Gamma, \Query{\Delta, \query A}C}
    {\Gamma, \Query{\Delta}C, A}
    \quad
    \infer[\Query]
    {\Gamma, \Query{\cdot}C}
    {\Gamma, C}
  \end{array}
\end{displaymath}

\subsection{Theory}

\begin{lemma} \label{lem:star}
  If $\DD :: \Gamma, [\ast]$ then $\Gamma, [\ast]^n$.
\end{lemma}
\begin{proof} to be completed.
\end{proof}

\begin{theorem}[Cut-admissibility] \ \par
  \begin{enumerate}  
  \item If $\DD:: \Gamma_1, A$
    and $\EE:: \Gamma_2,\dual{A}$
    then $ \Gamma_1,\Gamma_2$.\label{cuta}
  % \item \red{If $\DD:: ?\Delta, A$
  %   and $\EE:: \Gamma,!\dual{A}$
  %   then $ ?\Delta,\Gamma$.}\label{cutb}
  \item If $\DD:: \Delta_1, A$
    and $\EE:: \Delta_2, \Gamma_2, B$
    and $\FF:: \Gamma_3,[A^\perp]B^\perp$
    then $ [\Delta_1]\Delta_2,\Gamma_2, \Gamma_3$.\label{cutb}
  % \item If $\DD:: \Gamma_1, \Left{\Delta_1, A \oplus B} C$
  %   and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
  %   and $ \FF :: \Gamma_2, \Right{\Delta_2} B^\perp$
  %   then $ \Gamma_1, \Left{\Delta_1, \Delta_2} C,  \Gamma_2$.\label{cutc}
  % \item If $\DD ::  \Gamma_1, \Right{ \Delta_1,A \oplus B} C$
  %   and $\EE ::  \Gamma_2, \Left{ \Delta_2} A^\perp$
  %   and	$\FF ::	 \Gamma_2, \Right{ \Delta_2} B^\perp$
  %   then $ \Gamma_1, \Right{ \Delta_1, \Delta_2}C ,  \Gamma_2$.\label{cutd}
  % \item If $\DD ::\Gamma_1, \Left{\Delta_1} C, A$
  %   and $\EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
  %   then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2}C$.\label{cute}
  % \item If $\DD :: \Gamma_1, \Right{\Delta_1} C, A$
  %   and $\EE :: \Gamma_2, \Right{\Delta_2}A^\perp$
  %   then $ \Gamma_1,  \Gamma_2, \Right{\Delta_1, \Delta_2}C $.\label{cutf}
  % \item If  $\DD :: \Gamma, \Query{?\Delta_1,\query A}C$
  %   and $\EE:: \query\Delta_2,\bang A^\perp$
  %   then $\Gamma, \Query {?\Delta_1,\query\Delta_2}C$.\label{cutg}
  % \item If $\DD :: \Gamma_1, \Query{?\Delta_1}C, A$
  %   and $\EE :: \Gamma_2, \Query{?\Delta_2} A^\perp$
  %   then $\Gamma_1,\Gamma_2, \Query{?\Delta_1,?\Delta_2} C$.\label{cuth}
  %   \bigskip

  \item If $\DD:: \Gamma_1, \Left{\Delta_1, A \oplus B} C$
    and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
 %   and $ \FF :: \Gamma_2, \Right{\Delta_2} B^\perp$
    then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2} C$.\label{cs1}
  \item If $\DD:: \Gamma_1, \Right{\Delta_1, A \oplus B} C$
%    and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
    and $ \EE :: \Gamma_2, \Right{\Delta_2} B^\perp$
    then $ \Gamma_1,  \Gamma_2, \Right{\Delta_1, \Delta_2} C$.\label{cs2}

  \item If  $\DD :: \Gamma_1, \Query{\Delta_1,\query A}C$
    and $\EE :: \Gamma_2, \Query{\Delta_2} A^\perp$ 
    then $\Gamma_1,\Gamma_2, \Query {\Delta_1,\Delta_2}C$.\label{cs3}

  \end{enumerate}
\end{theorem}

\begin{theorem}[Cut-admissibility (ii)] \ \par
  \begin{enumerate}  
  \item If $\DD:: \Gamma_1, A$
    and $\EE:: \Gamma_2,\dual{A}$
    then $ \Gamma_1,\Gamma_2$.\label{cuta}    
  \item If $\DD:: \Delta_1, A$
    and $\EE:: \Delta_2, \Gamma_2, B$
    and $\FF:: \Gamma_3,[A^\perp]B^\perp$
    then $ [\Delta_1]\Delta_2,\Gamma_2, \Gamma_3$.\label{cutb}
  \item If $\DD:: \Gamma_1, \Left{\Delta_1, A \oplus B} C$
    and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
    then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2} C$.\label{cs1}
  \item If $\DD:: \Gamma_1, \Right{\Delta_1, A \oplus B} C$
    and $ \EE :: \Gamma_2, \Right{\Delta_2} B^\perp$
    then $ \Gamma_1,  \Gamma_2, \Right{\Delta_1, \Delta_2} C$.\label{cs2}

  \item If  $\DD :: \Gamma_1, \Query{\Delta_1,\query A}C$
    and $\EE :: \Gamma_2, \Query{\Delta_2} A^\perp$ 
    then $\Gamma_1,\Gamma_2, \Query {\Delta_1,\Delta_2}C$.\label{cs3}

  \end{enumerate}
\end{theorem}

\begin{proof} by induction over the cut formula and the left and right derivation. (This has to be made much more precise).
  \begin{enumerate}
    % ---------------------------------------------------------------------
  \item % 1.
    \begin{description}
    \item [Impossible Cases:] 
    \item [Axiom Case:]
      \[
        \DD =
        \infer[\ax]
        {A^\perp, A}
        {}
      \]
      \begin{tabbing}
        $A^\perp, \Gamma_2$ \` by $\EE$ 
      \end{tabbing}
    \item [Essential Case:]
      \[
        \DD = \infer[\one]
        {\one, [\ast]^n}
        {}
      \]
      and
      \[
        \EE =
        \infer[\bot]
        {\Gamma_2, \bot}
        {\EE_1 :: \Gamma_2, [\ast]}
      \]
      \begin{tabbing}
        $\Gamma_2, [\ast]^n$ \` by Lemma~\ref{lem:star} on $\EE_1$
      \end{tabbing}
    \item [Essential Case:] 
      \[\DD =
        \infer[\tensor]
        {\Gamma_1, [\Delta_1]\Delta_2, A \tensor B}
        { \DD_1 :: \Delta_1, A
          \quad 
          \DD_2 :: \Gamma_1, \Delta_2, B}
      \] 
      and 
      \[
        \EE = 
        \infer[\parr]
        {\Gamma_2, A^\perp \parr B^\perp}
        {\EE_1 :: \Gamma_2, [A^\perp] B^\perp} 
      \]
        \begin{tabbing}
          $[\Delta_1] \Delta_2, \Gamma_1, \Gamma_2$ \` by i.h.~\ref{cutb} on $\DD_1$, $\DD_2$, and $\EE_1$
      \end{tabbing}
    \item [Essential Case:] \[\DD =     \infer[\with]
        {\Gamma_1,A \oplus B, \oplus\Delta_1,C \with D}
        {\DD_1 :: \Gamma_1, \Left{A \oplus B,\oplus\Delta_1}C
          \quad
          \DD_2 :: \Gamma_1, \Right{A \oplus B,\oplus\Delta_1} D}
      \] and \[ \EE =     \infer[\with]
        {\Gamma_2,\oplus\Delta_2,A^\perp \with B^\perp}
        {\EE_1 :: \Gamma_2, \Left{\oplus\Delta_2}A^\perp
          \quad
          \EE_2 :: \Gamma_2, \Right{\oplus\Delta_2} B^\perp} \]
      \begin{tabbing}
        $ \GG_1 :: \Gamma_1,  \Gamma_2, \Left{\oplus \Delta_1, \oplus \Delta_2} C$ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE_1$ \\
        $ \GG_2 :: \Gamma_1,  \Gamma_2, \Right{\oplus \Delta_1, \oplus \Delta_2} D$ \` by i.h.~\ref{cs2} on $\DD_2$ and $\EE_2$ \\
        $ \Gamma_1,  \Gamma_2, \oplus \Delta_1, \oplus \Delta_2, C \with D$ \` by $\with$ on $\GG_1$ and $\GG_2$
      \end{tabbing}
    \item [Essential Case:]
      \[\DD =   \infer[\bang]
      {\query \Delta_1, ? A, \bang C} 
      {\DD_1
        :: \Query{\query\Delta_1, ? A} C}
    \]
    and
    \[\EE =
      \infer[\bang]
      {\query \Delta_2, \bang A^\perp} 
      { \EE_1 :: \Query{\query\Delta_2} A^\perp}
    \]

    
    \begin{tabbing}
      $\GG :: \Query {?\Delta_1,\query\Delta_2}C$  \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE_1$\\
      $?\Delta_1,\query\Delta_2, \bang C$  \` by $\bang$ on $\GG$\\
    \end{tabbing}

  \item [Left-Commutative Case:]
    \[\DD  =
      \infer[\bot]
      {\Gamma_1,A, \bot}
      {\DD_1 :: \Gamma_1,A, [\ast]}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, [\ast]$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2, \bot$ \` by $\bot$ on $\GG$
    \end{tabbing}
 \item [Left-Commutative Case:]
   \[\DD  =
     \infer[\tensor]
     {\Gamma_1, A, [\Delta_1]\Delta_2, D \tensor E}
     { \DD_1 :: \Delta_1, D
       \quad
       \DD_2 :: \Gamma_1, A, \Delta_2, E
     }
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, \Delta_2, E$ \` by i.h.~\ref{cuta} on $\DD_2$ and $\EE$ \\
      $\Gamma_1, \Gamma_2, [\Delta_1]\Delta_2,D \tensor E,$ \` by $\tensor$ on $\DD_1$ and $\GG$ \\
    \end{tabbing}

 \item [Left-Commutative Case:]
   \[\DD  =
     \infer[\parr]
     {\Gamma_1, A, D \parr E}
     {\DD_1::\Gamma_1, A, [D] E}     
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, [D]E $ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2, D \parr E$ \` by $\parr$ on $\GG$
    \end{tabbing}

 \item [Left-Commutative Case:]
    \[\DD  =
      \infer[\with]
      {\Gamma_1,A,\oplus\Delta,D \with E}
      {\DD_1 :: \Gamma_1,A, \Left{\oplus\Delta}D
        \quad
        \DD_2 :: \Gamma_1,A, \Right{\oplus\Delta} E}
    \]
    \begin{tabbing}
      $\GG_1 ::\Gamma_1, \Gamma_2, \Left{\oplus\Delta}D $ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\GG_2 ::\Gamma_1, \Gamma_2,  \Right{\oplus\Delta} E$ \` by i.h.~\ref{cuta} on $\DD_2$ and $\EE$ \\
      $\Gamma_1, \Gamma_2, \oplus\Delta,D \with E$ \` by $\with$ on $\GG_1$ and $\GG_2$
    \end{tabbing}

 \item [Left-Commutative Case:]
   \[\DD  =
     \infer[\Left]
     {\Gamma_1,A, \Left{\cdot}C}
     {\DD_1 :: \Gamma_1,A, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, C$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2, \Left{\cdot}C$ \` by $\Left$ on $\GG$
    \end{tabbing}

 \item [Left-Commutative Case:]
    \[\DD  =
      \infer[\Right]
      {\Gamma_1, A, \Right{\cdot}C}
      {\Gamma_1, A, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, C$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2,\Right{\cdot}C$ \` by $\Right$ on $\GG$
    \end{tabbing}

 \item [Left-Commutative Case:]
   \[\DD  =
     \infer[\oplus_1]
     {\Gamma_1, A,  \Left{\Delta, D\oplus E} C}
    {\DD_1::\Gamma_1, A,  \Left{\Delta} C, D}    
  \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Left{\Delta} C, D$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2,\Left{\Delta, D\oplus E} C$ \` by $\oplus_1$ on $\GG$
    \end{tabbing}

 \item [Left-Commutative Case:]
   \[\DD  =  \infer[\oplus_2]
     {\Gamma_1, A, \Right{\Delta, D\oplus E}C}
     {\DD_1 :: \Gamma_1, A,\Right{\Delta} C, E}
   \]
   \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Right{\Delta} C, E$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2,\Right{\Delta, D\oplus E} C$ \` by $\oplus_2$ on $\GG$
   \end{tabbing}


  % \item [Mixed-Left-Commutative Case:]
  %   \[\DD  =
  %     \infer[\bang]
  %     {\query \Delta, \query C, \bang A} 
  %     {\DD_1 :: \Query{\query\Delta, \query C} A}
  %   \]
  %   and
  %   \[\EE =
  %     \infer[\ax]
  %     {\query A^\perp, \bang A}
  %     {}
  %   \]
  %   \begin{tabbing}
  %     $\query \Delta, \query C, \bang A$ \` by $\DD$
  %   \end{tabbing}
  \item [Mixed-Left-Commutative Case:] $\DD$ ending in $\one$ impossible
  \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\bot]
      {\Gamma_2, \query A^\perp, \bot}
      {\EE_1::\Gamma_2,  \query A^\perp,  [\ast]}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, [\ast]$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \bot$ \` by $\bot$ on $\GG$
    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\tensor]
      {\Gamma_2, \query A^\perp,[\Delta_3]\Delta_4, D \tensor E}
      {\EE_1 :: \Delta_3, D \quad \EE_2 ::\Gamma_2,\query A^\perp, \Delta_4, E}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, \Delta_4, E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_2$\\
      $\query \Delta, \query C, \Gamma_2, [\Delta_3]\Delta_4, D \tensor E$ \` by $\tensor$ on $\EE_1$ and $\GG$
    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\parr]
      {\Gamma_2, \query A^\perp,  D \parr E}
      {\EE_1 :: \Gamma_2, \query A^\perp, [D] E}           
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, [D]E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2,  D \parr E$ \` by $\parr$ on $\GG$
    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\with]
      {\Gamma_2, \query A^\perp,\oplus\Delta,D \with E}
      {\EE_1 :: \Gamma_2, \query A^\perp, \Left{\oplus\Delta}D
        \quad
        \EE_2 :: \Gamma_2, \query A^\perp, \Right{\oplus\Delta} E
      }
    \]
    \begin{tabbing}
      $\GG_1 :: \query \Delta, \query C, \Gamma_2, \Left{\oplus\Delta}D $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\GG_2 :: \query \Delta, \query C, \Gamma_2, \Right{\oplus\Delta} E $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_2$\\
      $\query \Delta, \query C, \Gamma_2, \oplus\Delta, D \with E $ \` by $\with$ on $\GG_1$ and $\GG_2$\\
   \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\Left]
      {\Gamma_2, \query A^\perp, \Left{\cdot}D}
      {\EE_1 :: \Gamma_2, \query A^\perp, D}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, D $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \Left{\cdot}D $ \` by $\Left$ on $\GG$ 
    \end{tabbing}
    \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\Right]
      {\Gamma_2, \query A^\perp, \Right{\cdot}D}
      {\EE_1 :: \Gamma_2, \query A^\perp, D}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, D $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \Right{\cdot}D $ \` by $\Right$ on $\GG$ 
    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\oplus_1]
    {\Gamma_2,  \query A^\perp, \Left{\Delta, D\oplus E} C}
    {\EE_1 :: \Gamma_2,  \query A^\perp, \Left{\Delta} C, D}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, \Left{\Delta} C, D$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \Left{\Delta, D\oplus E} C$ \` by $\oplus_1$ on  $\GG$\\
    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\oplus_2]
    {\Gamma_2,  \query A^\perp, \Left{\Delta, D\oplus E} C}
    {\EE_1 :: \Gamma_2,  \query A^\perp, \Left{\Delta} C, E}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, \Left{\Delta} C, E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \Left{\Delta, D\oplus E} C$ \` by $\oplus_2$ on  $\GG$\\
    \end{tabbing}

 \item [Mixed-Left-Commutative Case:] there is no commutative case for $\bang$, $\bang$, other than the essential case. 
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\query]
      {\Gamma_2,  \query A^\perp,\Query{\Delta_2, \query E}D}
      {\EE_1 :: \Gamma_2,  \query A^\perp,\Query{\Delta_2}D, E}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, \Query{\Delta_2}D, E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \Query{\Delta_2, \query E}D$ \` by $?$ on $\GG$\\

    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\Query]
      {\Gamma_2,  \query A^\perp,\Query{\cdot}C}
      {\EE_1 :: \Gamma_2,  \query A^\perp, C}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, C$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2,\Query{\cdot} C$ \` by $\Query$ on $\GG$       
    \end{tabbing}

  \item [Left-Commutative Case:]
    \[\DD  =     \infer[\query]
      {\Gamma_1,A, \Query{\Delta, \query D}C}
      {\DD_1 :: \Gamma_1,A, \Query{\Delta}C, D}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Query{\Delta}C, D$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2,\Query{\Delta, \query D}C$ \` by $\query$ on $\GG$
    \end{tabbing}
  \item [Left-Commutative Case:]
    \[\DD  =
[      \infer[\Query]
      {\Gamma_1, A, \Query{\cdot}C}
      {\DD_1 :: \Gamma_1, A, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  C$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2,\Query{}C$ \` by $\Query$ on $\GG$
    \end{tabbing}

    % ################################################################
    % Start
    % ################################################################

    
  \item [Right-Commutative Case:]
    \[\EE  =
      \infer[\bot]
      {\Gamma_2,A^\perp, \bot}
      {\EE_1 :: \Gamma_2,A^\perp, [\ast]}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, [\ast], \Gamma_2$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2, \bot$ \` by $\bot$ on $\GG$
    \end{tabbing}
 \item [Right-Commutative Case:]
   \[\EE  =
     \infer[\tensor]
     {\Gamma_2, A^\perp, [\Delta_1]\Delta_2, D \tensor E}
     { \EE_1 :: \Delta_1, D
       \quad
       \EE_2 :: \Gamma_2, A^\perp, \Delta_2, E
     }
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, \Delta_2, E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2, [\Delta_1]\Delta_2,D \tensor E,$ \` by $\tensor$ on $\DD_1$ and $\GG$ \\
    \end{tabbing}

 \item [Right-Commutative Case:]
   \[\EE  =
     \infer[\parr]
     {\Gamma_2, A^\perp, D \parr E}
     {\EE_1::\Gamma_2, A^\perp, [D] E}     
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, [D]E $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2, D \parr E$ \` by $\parr$ on $\GG$
    \end{tabbing}

 \item [Right-Commutative Case:]
    \[\EE  =
      \infer[\with]
      {\Gamma_2,A^\perp,\oplus\Delta,D \with E}
      {\EE_1 :: \Gamma_2,A^\perp, \Left{\oplus\Delta}D
        \quad
        \EE_2 :: \Gamma_2,A^\perp, \Right{\oplus\Delta} E}
    \]
    \begin{tabbing}
      $\GG_1 ::\Gamma_1, \Gamma_2, \Left{\oplus\Delta}D $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\GG_2 ::\Gamma_1, \Gamma_2,  \Right{\oplus\Delta} E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_2$ \\
      $\Gamma_1, \Gamma_2, \oplus\Delta,D \with E$ \` by $\with$ on $\GG_1$ and $\GG_2$
    \end{tabbing}

 \item [Right-Commutative Case:]
   \[\EE  =
     \infer[\Left]
     {\Gamma_2,A^\perp, \Left{\cdot}C}
     {\EE_1 :: \Gamma_2,A^\perp, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, C$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2, \Left{\cdot}C$ \` by $\Left$ on $\GG$
    \end{tabbing}

 \item [Right-Commutative Case:]
    \[\EE  =
      \infer[\Right]
      {\Gamma_2, A^\perp, \Right{\cdot}C}
      {\Gamma_2, A^\perp, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, C$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2,\Right{\cdot}C$ \` by $\Right$ on $\GG$
    \end{tabbing}

 \item [Right-Commutative Case:]
   \[\EE  =
     \infer[\oplus_1]
     {\Gamma_2, A^\perp,  \Left{\Delta, D\oplus E} C}
    {\EE_1::\Gamma_2, A^\perp,  \Left{\Delta} C, D}    
  \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Left{\Delta} C, D$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2,\Left{\Delta, D\oplus E} C$ \` by $\oplus_1$ on $\GG$
    \end{tabbing}

 \item [Right-Commutative Case:]
   \[\EE  =  \infer[\oplus_2]
     {\Gamma_2, A^\perp, \Right{\Delta, D\oplus E}C}
     {\EE_1 :: \Gamma_2, A^\perp,\Right{\Delta} C, E}
   \]
   \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Right{\Delta} C, E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2,\Right{\Delta, D\oplus E} C$ \` by $\oplus_2$ on $\GG$
   \end{tabbing}

   %%%% CARSTEN
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\bot]
     {\Gamma_1,\bang A, \bot}
     {\DD_1 :: \Gamma_1, \bang A, [\ast]}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1:: \Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1, [\ast], \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, \bot, \query \Delta, \bang C$
     \` by $\bot$ on $\GG$ 
   \end{tabbing}

    \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\tensor]
     {\Gamma_1, \bang A, [\Delta_1]\Delta_2,  D \tensor E}
     {\DD_1 :: \Delta_1, D \quad \DD_1 :: \Gamma_1,\bang A, \Delta_2, E}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1,  \Delta_2, E, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_2$ and $\EE$ \\
     $\Gamma_1,  [\Delta_1]\Delta_2,  D \tensor E, \query \Delta, \bang C$
     \` by $\tensor$ on $\DD_1$ and $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\parr]
     {\Gamma_1, \bang A, D \parr E}
     {\DD_1 :: \Gamma_1, \bang A, [D] E}     
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1, [D] E, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, D \parr E, \query \Delta, \bang C$
     \` by $\parr$ on $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\with]
     {\Gamma_1, \bang A,\oplus\Delta,D \with E}
     {\DD_1:: \Gamma_1, \bang A, \Left{\oplus\Delta}D
       \quad
       \DD_2 :: \Gamma_1, \bang A, \Right{\oplus\Delta} E}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG_1 :: \Gamma_1, \Left{\oplus\Delta}D, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\GG_2 :: \Gamma_1, \Right{\oplus\Delta} E, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, \oplus\Delta, D \with E, \query \Delta, \bang C$
     \` by $\with$ on $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\Left]
     {\Gamma_1, \bang A, \Left{\cdot}C}
     {\DD_1 :: \Gamma_1, \bang A, C}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1, C, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, \Left{\cdot}C, \query \Delta, \bang C$
     \` by $\Left$ on $\GG$ 
    \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\Right]
     {\Gamma_1, \bang A, \Right{\cdot}C}
     {\DD_1 :: \Gamma_1, \bang A, C}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1, C, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, \Right{\cdot}C, \query \Delta, \bang C$
     \` by $\Right$ on $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\oplus_1]
     {\Gamma_1, \bang A, \Left{\Delta, D\oplus E} C}
     {\DD_1 :: \Gamma_1, \bang A, \Left{\Delta} C, D} 
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1,  \Left{\Delta} C, D, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1,\Left{\Delta, D\oplus E} C, \query \Delta, \bang C$
     \` by $\oplus_1$ on $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\oplus_2]
     {\Gamma_1, \bang A, \Right{\Delta, D\oplus E} C}
     {\DD_2 \Gamma_1, \bang A, \Right{\Delta} C, E} 
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1,  \Right{\Delta} C, E, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1,\Right{\Delta, D\oplus E} C, \query \Delta, \bang C$
     \` by $\oplus_2$ on $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:] no additional case for $\bang$, $\bang$
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\query]
     {\Gamma_1, \bang A, \Query{\Delta, \query D}C}
     {\DD_1 :: \Gamma, \bang A, \Query{\Delta}C, D}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1,  \Query{\Delta}C, D, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, \Query{\Delta, \query D}C, \query \Delta, \bang C$
     \` by $\query$ on $\GG$ 

   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\Query]
     {\Gamma_1, \bang A, \Query{\cdot}C}
     {\DD_1 :: \Gamma_1, \bang A, C}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1, C, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1,  \Query{\cdot}C, \query \Delta, \bang C$
     \` by $\Query$ on $\GG$      
   \end{tabbing}

   %%% END CARSTEN
   
  \item [Right-Commutative Case:]
    \[\EE  =     \infer[\query]
      {\Gamma_2,A^\perp, \Query{\Delta, \query D}C}
      {\EE_1 :: \Gamma_2,A^\perp, \Query{\Delta}C, D}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Query{\Delta}C, D$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2,\Query{\Delta, \query D}C$ \` by $\query$ on $\GG$
    \end{tabbing}
  \item [Right-Commutative Case:]
    \[\EE  =
      \infer[\Query]
      {\Gamma_2, A^\perp, \Query{\cdot}C}
      {\EE_1 :: \Gamma_2, A^\perp, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  C$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2,\Query{}C$ \` by $\Query$ on $\GG$
    \end{tabbing}




    % ################################################################
    % End
    % ################################################################
  \end{description}

    % ---------------------------------------------------------------------
  \item by induction on $\FF$. This case is complete.  % 2.
    \begin{description}
    \item [Impossible Cases:] $\ax$, $\one$, $\bang$. 
    \item [Essential Case:] $\FF = \infer[\tensor]
      {\Gamma_3, C \tensor D, [A^\perp]B^\perp}
      {\FF_1 :: A^\perp, C \quad \FF_2 :: \Gamma_3 , B^\perp, D}$ 
      \begin{tabbing}
        $\GG_1 :: \Delta_1, C$ \` by i.h.~\ref{cuta} on $\DD$ and $\FF_1$ \\
        $\GG_2 :: \Delta_2, \Gamma_2, \Gamma_3, D$ \` by i.h.~\ref{cuta} on $\EE$ and $\FF_2$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, C \tensor D$ \` by  $\tensor$ on $\GG_1$ and $\GG_2$
      \end{tabbing}
    \item [Commutative Case:] $\FF = \infer[\tensor]
      {\Gamma_3, [\Delta'_1]\Delta'_2, C \tensor D, [A^\perp]B^\perp}
      {\FF_1 :: \Delta'_1, C \quad \FF_2 :: \Gamma_3 , [A^\perp]B^\perp, \Delta'_2, D}$ 
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Delta_2', D$ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_2$ \\
        $[\Delta'_1] \Delta'_2, C \tensor D,  [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3$ \` by  $\tensor$ on $\FF_1$ and $\GG$
      \end{tabbing}
    \item [Commutative Case:]  $\FF = \infer[\bot]
      {\Gamma_3,  [A^\perp]B^\perp, \bot}
      {\FF_1:: \Gamma_3,  [A^\perp]B^\perp, [\ast]}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, [\ast] $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \bot $ \` by $\bot$ on $\GG$
      \end{tabbing}
    \item [Commutative Case:] $\FF =  \infer[\parr]
      {\Gamma_3, [A^\perp]B^\perp, C \parr D}
      {\FF_1 :: \Gamma_3, [A^\perp]B^\perp, [C] D}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, [C] D  $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, C \parr D $ \` by $\parr$ on $\GG$
      \end{tabbing}
    \item [Commutative Case:] $\FF =  \infer[\with]
      {\Gamma_3, [A^\perp]B^\perp,\oplus\Delta,C \with D}
      {\FF_1 :: \Gamma_3,  [A^\perp]B^\perp,\Left{\oplus\Delta}C
        \quad
        \FF_2 :: \Gamma_3,  [A^\perp]B^\perp,\Right{\oplus\Delta} D}$
      \begin{tabbing}
        $\GG_1 :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\oplus\Delta}C $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $\GG_2 :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3,\Right{\oplus\Delta} D$ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_2$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \oplus \Delta, C \with D$ \` by $\with$ on $\GG_1$ and $\GG_2$
      \end{tabbing}
    \item [Commutative Case:] $\FF =  \infer[\Left]
      {\Gamma_3,  [A^\perp]B^\perp, \Left{\cdot}C}
      {\FF_1::\Gamma_3,  [A^\perp]B^\perp}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3 $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\cdot}C $ \` by $\Left$ on  $\GG$
      \end{tabbing}
    \item [Commutative Case:] $\FF =  \infer[\Right]
      {\Gamma_3,  [A^\perp]B^\perp, \Right{\cdot}C}
      {\FF_1::\Gamma_3,  [A^\perp]B^\perp}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3 $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Right{\cdot}C $ \` by $\Right$ on  $\GG$
      \end{tabbing}
      
    \item [Commutative Case:] $\FF =  \infer[\oplus_1]
      {\Gamma_3,  [A^\perp]B^\perp, \Left{\Delta, D\oplus E} C}
      {\FF_1::\Gamma_3,  [A^\perp]B^\perp, \Left{\Delta} C, D}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\Delta} C,D $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $ [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\Delta, D \oplus E} C $ \` by $\oplus_1$ on  $\GG$ \\
      \end{tabbing}
      
    \item [Commutative Case:] $\FF =  \infer[\oplus_2]
      {\Gamma_3,  [A^\perp]B^\perp, \Left{\Delta, D\oplus E} C}
      {\FF_1::\Gamma_3,  [A^\perp]B^\perp, \Left{\Delta} C, E}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\Delta} C,E $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $ [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\Delta, D \oplus E} C $ \` by $\oplus_2$ on  $\GG$ \\
      \end{tabbing}
      
    \item [Commutative Case:] $\FF =   \infer[\query]
      {\Gamma_3, [A^\perp]B^\perp, \Query{\Delta, \query D}C}
      {\FF_1 :: \Gamma_3, [A^\perp]B^\perp, \Query{\Delta}C, D}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Query{\Delta}C, D $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $ [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Query{\Delta, ?D}C $ \` by $\query$ on  $\GG$ \\
      \end{tabbing}
      
    \item [Commutative Case:] $\FF = \infer[\Query]
      {\Gamma_3, [A^\perp]B^\perp, \Query{\cdot}C}
      {\FF_1 :: \Gamma_3, [A^\perp]B^\perp}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3 $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $ [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Query{\cdot}C $ \` by $\Query$ on  $\GG$ \\
      \end{tabbing}
      
    \end{description}
    % ---------------------------------------------------------------------
  \item This should be by induction on $\DD$ and $\EE$ % 3.
    % This case is complete.
   % \item If $\DD:: \Gamma_1, \Left{\Delta_1, A \oplus B} C$
   %  and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
   %  then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2} C$.
    \begin{description}
    \item [Impossible Cases:]  $\ax$, $\one$, $\bang$
    \item [Essential Case:]
      \[\DD  =
        \infer[\oplus_1]
        {\Gamma_1,  \Left{\Delta_1, A\oplus B} C}
        {\DD_1 :: \Gamma_1,  \Left{\Delta_1} C, A}\]
      and
      \[\EE =
        \infer[\Left]
        {\Gamma_2, \Left{\cdot}A^\perp}
        {\EE_1::\Gamma_2, A^\perp}
      \]
      \begin{tabbing}
        $\Gamma_1, \Gamma_2, \Left{\Delta_1}C$ \` by i.h. \ref{cuta} on $\DD_1$ and $\EE_1$
      \end{tabbing}
% %%%%%%%%%%
% Left Commutative Cases
% %%%%%%%%%%%%%%%%%
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\bot]
        {\Gamma_1, \Left{\Delta_1, A \oplus B} C, \bot}
        {\DD_1 :: \Gamma_1, \Left{\Delta_1, A \oplus B} C, [\ast]} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2,[\ast], \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE$\\
        $\GG :: \Gamma_1, \Gamma_2, \bot, \Left{\Delta_1,  \Delta_2} C $ \` by $\bot$ on $\GG$
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =  \infer[\tensor]
        {\Gamma_1, \Left{\Delta_1, A \oplus B} C, [\Delta_3]\Delta_4, D \tensor E}
        {\DD_1::\Delta_3, D \quad \DD_2::\Gamma_1, \Left{\Delta_1, A \oplus B} C, \Delta_4, E} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Delta_4, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_2$ and $\EE$\\
        $ \Gamma_1, \Gamma_2, [\Delta_3]\Delta_4, D \tensor E, \Left{\Delta_1,  \Delta_2} C $ \` by $\tensor$ on $\DD_1$ and $\GG$
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
       \infer[\parr]
       {\Gamma_1, \Left{\Delta_1, A \oplus B} C, D \parr E}
       {\DD_1::\Gamma_1, \Left{\Delta_1, A \oplus B} C, [D] E} \]
     \begin{tabbing}
       $\GG :: \Gamma_1, \Gamma_2, [D]E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, D \parr E, \Left{\Delta_1,  \Delta_2} C $ \` by $\parr$ on $\GG$ 
      \end{tabbing}

      
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\with]
        {\Gamma_1,\Left{\Delta_1, A \oplus B} C,\oplus\Delta,D \with E}
        {\DD_1 :: \Gamma_1, \Left{\Delta_1, A \oplus B} C,\Left{\oplus\Delta}D
          \quad
          \DD_2 ::\Gamma_1, \Left{\Delta_1, A \oplus B} C,\Right{\oplus\Delta} E}
      \]
      \begin{tabbing}
      $\GG_1 :: \Gamma_1, \Gamma_2, \Left{\oplus\Delta}D , \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE$\\
      $\GG_2 :: \Gamma_1, \Gamma_2, \Right{\oplus\Delta} E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_2$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, D \with E, \Left{\Delta_1,  \Delta_2} C $ \` by $\with$ on $\GG_1$ and $\GG_2$
     \end{tabbing}


    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Left]
        {\Gamma_1,\Left{\Delta_1, A \oplus B} C, \Left{\cdot}D}
        {\DD_1 ::\Gamma_1,\Left{\Delta_1, A \oplus B} C, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, \Left{\cdot}D , \Left{\Delta_1,  \Delta_2} C $ \` by $\Left$ on $\GG_1$
      \end{tabbing}

    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Right]
        {\Gamma_1,\Left{\Delta_1, A \oplus B} C, \Right{\cdot} D}
        {\DD_1 :: \Gamma_1,\Left{\Delta_1, A \oplus B} C, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, \Right{\cdot}D , \Left{\Delta_1,  \Delta_2} C $ \` by $\Right$ on $\GG_1$
      \end{tabbing}




      
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\oplus_1]
        {\Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Right{\Delta_3, D\oplus E}F}
        {\DD_1 :: \Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Right{\Delta_3} F, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Left{\Delta_1,  \Delta_2} C $ \` by $\oplus_1$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\oplus_2]
        {\Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Right{\Delta_3, D\oplus E}F}
        {\DD_1 :: \Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Right{\Delta_3} F, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Left{\Delta_1,  \Delta_2} C $ \` by $\oplus_2$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  = \infer[\query]
        {\Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Query{\Delta, \query D}E}
        {\DD_1:: \Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Query{\Delta}E, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Query{\Delta}E, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Query{\Delta, \query D}E, \Left{\Delta_1,  \Delta_2} C $ \` by $\query$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Query]
        {\Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Query{\cdot}E}
        {\DD_1 :: \Gamma_1,  \Left{\Delta_1, A \oplus B} C, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Query{\cdot}E, \Left{\Delta_1,  \Delta_2} C $ \` by $\Query$ on $\GG$      
      \end{tabbing}
      % %%%%%%%%%%%%%%%%%%%
      % Right Commutative Cases
      %%%%%%%%%%%%%%%%%%%%%
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\bot]
        {\Gamma_2, \Left{\Delta_2}A^\perp, \bot}
        {\EE_1 :: \Gamma_2, \Left{\Delta_2}A^\perp, [\ast]} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2,[\ast], \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_1$\\
        $\GG :: \Gamma_1, \Gamma_2, \bot, \Left{\Delta_1,  \Delta_2} C $ \` by $\bot$ on $\GG$
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =  \infer[\tensor]
        {\Gamma_2, \Left{\Delta_2}A^\perp, [\Delta_3]\Delta_4, D \tensor E}
        {\EE_1::\Delta_3, D \quad \EE_2::\Gamma_2, \Left{\Delta_2}A^\perp, \Delta_4, E} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Delta_4, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_2$\\
        $ \Gamma_1, \Gamma_2, [\Delta_3]\Delta_4, D \tensor E, \Left{\Delta_1,  \Delta_2} C $ \` by $\tensor$ on $\EE_1$ and $\GG$
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
       \infer[\parr]
       {\Gamma_2, \Left{\Delta_2}A^\perp, D \parr E}
       {\EE_1::\Gamma_2, \Left{\Delta_2}A^\perp, [D] E} \]
     \begin{tabbing}
       $\GG :: \Gamma_1, \Gamma_2, [D]E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, D \parr E, \Left{\Delta_1,  \Delta_2} C $ \` by $\parr$ on $\GG$ 
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\with]
        {\Gamma_2,\Left{\Delta_2}A^\perp,\oplus\Delta,D \with E}
        {\EE_1 :: \Gamma_2, \Left{\Delta_2}A^\perp,\Left{\oplus\Delta}D
          \quad
          \EE_2 ::\Gamma_2, \Left{\Delta_2}A^\perp,\Right{\oplus\Delta} E}
      \]
      \begin{tabbing}
      $\GG_1 :: \Gamma_1, \Gamma_2, \Left{\oplus\Delta}D , \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_1$\\
      $\GG_2 :: \Gamma_1, \Gamma_2, \Right{\oplus\Delta} E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_2$\\
       $ \Gamma_1, \Gamma_2, D \with E, \Left{\Delta_1,  \Delta_2} C $ \` by $\with$ on $\GG_1$ and $\GG_2$
     \end{tabbing}

    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Left]
        {\Gamma_2,\Left{\Delta_2}A^\perp, \Left{\cdot}D}
        {\EE_1 ::\Gamma_2,\Left{\Delta_2}A^\perp, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, \Left{\cdot}D , \Left{\Delta_1,  \Delta_2} C $ \` by $\Left$ on $\GG_1$
      \end{tabbing}

    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Right]
        {\Gamma_2,\Left{\Delta_2}A^\perp, \Right{\cdot} D}
        {\EE_1 :: \Gamma_2,\Left{\Delta_2}A^\perp, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, \Right{\cdot}D , \Left{\Delta_1,  \Delta_2} C $ \` by $\Right$ on $\GG_1$
      \end{tabbing}

      
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\oplus_1]
        {\Gamma_2,  \Left{\Delta_2}A^\perp, \Right{\Delta_3, D\oplus E}F}
        {\EE_1 :: \Gamma_2,  \Left{\Delta_2}A^\perp, \Right{\Delta_3} F, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Left{\Delta_1,  \Delta_2} C $ \` by $\oplus_1$ on $\GG$      
      \end{tabbing}


      
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\oplus_2]
        {\Gamma_2,  \Left{\Delta_2}A^\perp, \Right{\Delta_3, D\oplus E}F}
        {\EE_1 :: \Gamma_2,  \Left{\Delta_2}A^\perp, \Right{\Delta_3} F, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Left{\Delta_1,  \Delta_2} C $ \` by $\oplus_2$ on $\GG$      
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  = \infer[\query]
        {\Gamma_2,  \Left{\Delta_2}A^\perp, \Query{\Delta, \query D}E}
        {\EE_1:: \Gamma_2,  \Left{\Delta_2}A^\perp, \Query{\Delta}E, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Query{\Delta}E, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Query{\Delta, \query D}E, \Left{\Delta_1,  \Delta_2} C $ \` by $\query$ on $\GG$      
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Query]
        {\Gamma_2,  \Left{\Delta_2}A^\perp, \Query{\cdot}E}
        {\EE_1 :: \Gamma_2,  \Left{\Delta_2}A^\perp, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Query{\cdot}E, \Left{\Delta_1,  \Delta_2} C $ \` by $\Query$ on $\GG$      
      \end{tabbing}
    \end{description}
    \item The proof is analogous to (\ref{cs1}),  simply by replacing $\LL$ by $\RR$.

      % ---------------------------------------------------------------------
  \item This should be by induction on $\DD$ and $\EE$ % 5.
    % This case is complete.
   % \item If $\DD:: \Gamma_1, \Left{\Delta_1, A \oplus B} C$
   %  and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
   %  then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2} C$.
    \begin{description}
    \item [Impossible Cases:]  $\ax$, $\one$, $\bang$
    \item [Essential Case:]
      \[\DD  =
        \infer[\query]
        {\Gamma_1, \Query{\Delta_1, \query A}C}
        {\DD_1::\Gamma_1, \Query{\Delta_1}C, A}
      \]
        and
      \[\EE =
        \infer[\Query]
        {\Gamma_2, \Query{\cdot}A^\perp}
        {\EE_1::\Gamma_2, A^\perp}
      \]
      \begin{tabbing}
        $\Gamma_1, \Gamma_2,  \Query {\Delta_1}C$ \` by i.h. \ref{cuta} on $\DD_1$ and $\EE_1$
      \end{tabbing}
% %%%%%%%%%%%%%%%%%
% Left Commutative Cases
% %%%%%%%%%%%%%%%%%
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\bot]
        {\Gamma_1,\Query{\Delta_1,\query A} C, \bot}
        {\DD_1 :: \Gamma_1,\Query{\Delta_1,\query A} C, [\ast]} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2,[\ast], \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
        $\GG :: \Gamma_1, \Gamma_2, \bot, \Query{\Delta_1,  \Delta_2} C $ \` by $\bot$ on $\GG$
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =  \infer[\tensor]
        {\Gamma_1,\Query{\Delta_1,\query A} C, [\Delta_3]\Delta_4, D \tensor E}
        {\DD_1::\Delta_3, D \quad \DD_2::\Gamma_1,\Query{\Delta_1,\query A} C, \Delta_4, E} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Delta_4, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_2$ and $\EE$\\
        $ \Gamma_1, \Gamma_2, [\Delta_3]\Delta_4, D \tensor E, \Query{\Delta_1,  \Delta_2} C $ \` by $\tensor$ on $\DD_1$ and $\GG$
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
       \infer[\parr]
       {\Gamma_1,\Query{\Delta_1,\query A} C, D \parr E}
       {\DD_1::\Gamma_1,\Query{\Delta_1,\query A} C, [D] E} \]
     \begin{tabbing}
       $\GG :: \Gamma_1, \Gamma_2, [D]E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, D \parr E, \Query{\Delta_1,  \Delta_2} C $ \` by $\parr$ on $\GG$ 
      \end{tabbing}

      
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\with]
        {\Gamma_1,\Query{\Delta_1,\query A} C,\oplus\Delta,D \with E}
        {\DD_1 :: \Gamma_1,\Query{\Delta_1,\query A} C,\Left{\oplus\Delta}D
          \quad
          \DD_2 ::\Gamma_1,\Query{\Delta_1,\query A} C,\Right{\oplus\Delta} E}
      \]
      \begin{tabbing}
      $\GG_1 :: \Gamma_1, \Gamma_2, \Left{\oplus\Delta}D , \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
      $\GG_2 :: \Gamma_1, \Gamma_2, \Right{\oplus\Delta} E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_2$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, D \with E, \Query{\Delta_1,  \Delta_2} C $ \` by $\with$ on $\GG_1$ and $\GG_2$
     \end{tabbing}


    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Left]
        {\Gamma_1,\Query{\Delta_1,\query A} C, \Left{\cdot}D}
        {\DD_1 ::\Gamma_1,\Query{\Delta_1,\query A} C, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, \Left{\cdot}D , \Query{\Delta_1,  \Delta_2} C $ \` by $\Left$ on $\GG_1$
      \end{tabbing}

    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Right]
        {\Gamma_1, \Query{\Delta_1,\query A} C, \Right{\cdot} D}
        {\DD_1 :: \Gamma_1,\Query{\Delta_1,\query A} C, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, \Right{\cdot}D , \Query{\Delta_1,  \Delta_2} C $ \` by $\Right$ on $\GG_1$
      \end{tabbing}

    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\oplus_1]
        {\Gamma_1, \Query{\Delta_1,\query A} C, \Right{\Delta_3, D\oplus E}F}
        {\DD_1 :: \Gamma_1, \Query{\Delta_1,\query A} C, \Right{\Delta_3} F, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Query{\Delta_1,  \Delta_2} C $ \` by $\oplus_1$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\oplus_2]
        {\Gamma_1, \Query{\Delta_1,\query A} C, \Right{\Delta_3, D\oplus E}F}
        {\DD_1 :: \Gamma_1, \Query{\Delta_1,\query A} C, \Right{\Delta_3} F, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Query{\Delta_1,  \Delta_2} C $ \` by $\oplus_2$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  = \infer[\query]
        {\Gamma_1, \Query{\Delta_1,\query A} C, \Query{\Delta, \query D}E}
        {\DD_1:: \Gamma_1, \Query{\Delta_1,\query A} C, \Query{\Delta}E, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Query{\Delta}E, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Query{\Delta, \query D}E, \Query{\Delta_1,  \Delta_2} C $ \` by $\query$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Query]
        {\Gamma_1, \Query{\Delta_1,\query A} C, \Query{\cdot}E}
        {\DD_1 :: \Gamma_1, \Query{\Delta_1,\query A} C, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Query{\cdot}E, \Query{\Delta_1,  \Delta_2} C $ \` by $\Query$ on $\GG$      
      \end{tabbing}
      % %%%%%%%%%%%%%%%%%%%
      % Right Commutative Cases
      %%%%%%%%%%%%%%%%%%%%%
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\bot]
        {\Gamma_2, \Query{\Delta_2}A^\perp, \bot}
        {\EE_1 :: \Gamma_2, \Query{\Delta_2}A^\perp, [\ast]} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2,[\ast], \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_1$\\
        $\GG :: \Gamma_1, \Gamma_2, \bot, \Query{\Delta_1,  \Delta_2} C $ \` by $\bot$ on $\GG$
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =  \infer[\tensor]
        {\Gamma_2, \Query{\Delta_2}A^\perp, [\Delta_3]\Delta_4, D \tensor E}
        {\EE_1::\Delta_3, D \quad \EE_2::\Gamma_2, \Query{\Delta_2}A^\perp, \Delta_4, E} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Delta_4, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_2$\\
        $ \Gamma_1, \Gamma_2, [\Delta_3]\Delta_4, D \tensor E, \Query{\Delta_1,  \Delta_2} C $ \` by $\tensor$ on $\EE_1$ and $\GG$
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
       \infer[\parr]
       {\Gamma_2, \Query{\Delta_2}A^\perp, D \parr E}
       {\EE_1::\Gamma_2, \Query{\Delta_2}A^\perp, [D] E} \]
     \begin{tabbing}
       $\GG :: \Gamma_1, \Gamma_2, [D]E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, D \parr E, \Query{\Delta_1,  \Delta_2} C $ \` by $\parr$ on $\GG$ 
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\with]
        {\Gamma_2,\Query{\Delta_2}A^\perp,\oplus\Delta,D \with E}
        {\EE_1 :: \Gamma_2, \Query{\Delta_2}A^\perp,\Left{\oplus\Delta}D
          \quad
          \EE_2 ::\Gamma_2, \Query{\Delta_2}A^\perp,\Right{\oplus\Delta} E}
      \]
      \begin{tabbing}
      $\GG_1 :: \Gamma_1, \Gamma_2, \Left{\oplus\Delta}D , \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_1$\\
      $\GG_2 :: \Gamma_1, \Gamma_2, \Right{\oplus\Delta} E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_2$\\
       $ \Gamma_1, \Gamma_2, D \with E, \Query{\Delta_1,  \Delta_2} C $ \` by $\with$ on $\GG_1$ and $\GG_2$
     \end{tabbing}

    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Left]
        {\Gamma_2,\Query{\Delta_2}A^\perp, \Left{\cdot}D}
        {\EE_1 ::\Gamma_2,\Query{\Delta_2}A^\perp, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, \Left{\cdot}D , \Query{\Delta_1,  \Delta_2} C $ \` by $\Left$ on $\GG_1$
      \end{tabbing}

    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Right]
        {\Gamma_2,\Query{\Delta_2}A^\perp, \Right{\cdot} D}
        {\EE_1 :: \Gamma_2,\Query{\Delta_2}A^\perp, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, \Right{\cdot}D , \Query{\Delta_1,  \Delta_2} C $ \` by $\Right$ on $\GG_1$
      \end{tabbing}

      
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\oplus_1]
        {\Gamma_2,  \Query{\Delta_2}A^\perp, \Right{\Delta_3, D\oplus E}F}
        {\EE_1 :: \Gamma_2,  \Query{\Delta_2}A^\perp, \Right{\Delta_3} F, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Query{\Delta_1,  \Delta_2} C $ \` by $\oplus_1$ on $\GG$      
      \end{tabbing}


      
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\oplus_2]
        {\Gamma_2,  \Query{\Delta_2}A^\perp, \Right{\Delta_3, D\oplus E}F}
        {\EE_1 :: \Gamma_2,  \Query{\Delta_2}A^\perp, \Right{\Delta_3} F, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Query{\Delta_1,  \Delta_2} C $ \` by $\oplus_2$ on $\GG$      
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  = \infer[\query]
        {\Gamma_2,  \Query{\Delta_2}A^\perp, \Query{\Delta, \query D}E}
        {\EE_1:: \Gamma_2,  \Query{\Delta_2}A^\perp, \Query{\Delta}E, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Query{\Delta}E, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Query{\Delta, \query D}E, \Query{\Delta_1,  \Delta_2} C $ \` by $\query$ on $\GG$      
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  = \infer[\query]
        {\Gamma_2,  \Query{\Delta_2,\query D}A^\perp}
        {\EE_1:: \Gamma_2,  \Query{\Delta_2}A^\perp, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Query{\Delta_1,  \Delta_2, \query D} C $ \` by $\query$ on $\GG$      
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Query]
        {\Gamma_2,  \Query{\Delta_2}A^\perp, \Query{\cdot}E}
        {\EE_1 :: \Gamma_2,  \Query{\Delta_2}A^\perp, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Query{\cdot}E, \Query{\Delta_1,  \Delta_2} C $ \` by $\Query$ on $\GG$      
      \end{tabbing}
    \end{description}
    
  \end{enumerate}
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

==> app-cut1.tex <==

\newcommand{\ax}[0]{\textsc{ax}}
\renewcommand{\Left}[1]{\mathcal{L}\dbr{#1}}
\renewcommand{\Right}[1]{\mathcal{R}\dbr{#1}}
\renewcommand{\Query}[1]{\mathcal{Q}\dbr{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\section{Cut-elimination Proof for Synchronous Forwarders}
\label{app:cut}

\subsection{Rules}
\begin{displaymath}
  \small
  \begin{array}{c}
    \infer[\ax]
    {A^\perp, A}
    {}
    \qquad
    \infer[\one]
    {\one, [\ast]^n}
    {}
    \qquad
    \infer[\bot]
    {\Gamma, \bot}
    {\Gamma, [\ast]}
    \\\\
    \infer[\tensor]
    {\Gamma, [\Delta_1]\Delta_2, A \tensor B}
    {\Delta_1, A \quad \Gamma, \Delta_2, B}
    \qquad
    \infer[\parr]
    {\Gamma, A \parr B}
    {\Gamma, [A] B}     
    \\\\
    \infer[\with]
    {\Gamma,\oplus\Delta,A \with B}
    {\Gamma, \Left{\oplus\Delta}A
    \quad
    \Gamma, \Right{\oplus\Delta} B}
    \qquad
    \infer[\Left]
    {\Gamma, \Left{\cdot}C}
    {\Gamma, C}
    
    \qquad
    \infer[\Right]
    {\Gamma, \Right{\cdot}C}
    {\Gamma, C}
	
    \\\\
    \infer[\oplus_1]
    {\Gamma,  \Left{\Delta, A\oplus B} C}
    {\Gamma,  \Left{\Delta} C, A}
    \qquad
    \infer[\oplus_2]
    {\Gamma, \Right{\Delta, A\oplus B}C}
    {\Gamma, \Right{\Delta} C, B}
    \\\\
    \infer[\bang]
    {\query \Delta, \bang A} 
    {\Query{\query\Delta} A}
    \qquad
    \infer[\query]
    {\Gamma, \Query{\Delta, \query A}C}
    {\Gamma, \Query{\Delta}C, A}
    \quad
    \infer[\Query]
    {\Gamma, \Query{\cdot}C}
    {\Gamma, C}
  \end{array}
\end{displaymath}

\subsection{Theory}

\begin{lemma} \label{lem:star}
  If $\DD :: \Gamma, [\ast]$ then $\Gamma, [\ast]^n$.
\end{lemma}
\begin{proof} to be completed.
\end{proof}

\begin{theorem}[Cut-admissibility] \ \par
  \begin{enumerate}  
  \item If $\DD:: \Gamma_1, A$
    and $\EE:: \Gamma_2,\dual{A}$
    then $ \Gamma_1,\Gamma_2$.\label{cuta}
  % \item \red{If $\DD:: ?\Delta, A$
  %   and $\EE:: \Gamma,!\dual{A}$
  %   then $ ?\Delta,\Gamma$.}\label{cutb}
  \item If $\DD:: \Delta_1, A$
    and $\EE:: \Delta_2, \Gamma_2, B$
    and $\FF:: \Gamma_3,[A^\perp]B^\perp$
    then $ [\Delta_1]\Delta_2,\Gamma_2, \Gamma_3$.\label{cutb}
  % \item If $\DD:: \Gamma_1, \Left{\Delta_1, A \oplus B} C$
  %   and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
  %   and $ \FF :: \Gamma_2, \Right{\Delta_2} B^\perp$
  %   then $ \Gamma_1, \Left{\Delta_1, \Delta_2} C,  \Gamma_2$.\label{cutc}
  % \item If $\DD ::  \Gamma_1, \Right{ \Delta_1,A \oplus B} C$
  %   and $\EE ::  \Gamma_2, \Left{ \Delta_2} A^\perp$
  %   and	$\FF ::	 \Gamma_2, \Right{ \Delta_2} B^\perp$
  %   then $ \Gamma_1, \Right{ \Delta_1, \Delta_2}C ,  \Gamma_2$.\label{cutd}
  % \item If $\DD ::\Gamma_1, \Left{\Delta_1} C, A$
  %   and $\EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
  %   then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2}C$.\label{cute}
  % \item If $\DD :: \Gamma_1, \Right{\Delta_1} C, A$
  %   and $\EE :: \Gamma_2, \Right{\Delta_2}A^\perp$
  %   then $ \Gamma_1,  \Gamma_2, \Right{\Delta_1, \Delta_2}C $.\label{cutf}
  % \item If  $\DD :: \Gamma, \Query{?\Delta_1,\query A}C$
  %   and $\EE:: \query\Delta_2,\bang A^\perp$
  %   then $\Gamma, \Query {?\Delta_1,\query\Delta_2}C$.\label{cutg}
  % \item If $\DD :: \Gamma_1, \Query{?\Delta_1}C, A$
  %   and $\EE :: \Gamma_2, \Query{?\Delta_2} A^\perp$
  %   then $\Gamma_1,\Gamma_2, \Query{?\Delta_1,?\Delta_2} C$.\label{cuth}
  %   \bigskip

  \item If $\DD:: \Gamma_1, \Left{\Delta_1, A \oplus B} C$
     and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
     and $ \FF :: \Gamma_2, \Right{\Delta_2} B^\perp$
 %   and $ \FF :: \Gamma_2, \Right{\Delta_2} B^\perp$
    then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2} C$.\label{cs1}
  \item If $\DD ::\Gamma_1, \Left{\Delta_1} C, A$
    and $\EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
    then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2}C$.\label{cs11}
  \item If $\DD:: \Gamma_1, \Right{\Delta_1, A \oplus B} C$
     and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
     and $ \FF :: \Gamma_2, \Right{\Delta_2} B^\perp$
    then $ \Gamma_1,  \Gamma_2, \Right{\Delta_1,  \Delta_2} C$.\label{cs2}
  \item If $\DD :: \Gamma_1, \Right{\Delta_1} C, B$
    and $\EE :: \Gamma_2, \Right{\Delta_2}B^\perp$
    then $ \Gamma_1,  \Gamma_2, \Right{\Delta_1, \Delta_2}C $.\label{cs22}
  % \item If  $\DD :: \Gamma, \Query{?\Delta_1,\query A}C$
  %   and $\EE:: \query\Delta_2,\bang A^\perp$
  %   then $\Gamma, \Query {?\Delta_1,\query\Delta_2}C$.\label{cutg}

  % \item If $\DD:: \Gamma_1, \Right{\Delta_1, A \oplus B} C$
%     and $ \EE :: \Gamma_2, \Right{\Delta_2} B^\perp$
%     then $ \Gamma_1,  \Gamma_2, \Right{\Delta_1, \Delta_2} C$.\label{cs2}

  \item If  $\DD :: \Gamma_1, \Query{\Delta_1,\query A}C$
    and $\EE :: \Query{\Delta_2} A^\perp$
    then $\Gamma_1, \Query {\Delta_1,\Delta_2}C$.\label{cs3}
  \item If $\DD :: \Gamma_1, \Query{\Delta_1}C, A$
    and $\EE :: \Gamma_2, \Query{\Delta_2} A^\perp$
    then $\Gamma_1,\Gamma_2, \Query{\Delta_1,\Delta_2} C$.\label{cs33}
  \end{enumerate}
\end{theorem}

\begin{proof} by induction over the cut formula and the left and right derivation. (This has to be made much more precise).
  \begin{enumerate}
    % ---------------------------------------------------------------------
  \item % 1.
    \begin{description}
    \item [Impossible Cases:] 
    \item [Axiom Case:]
      \[
        \DD =
        \infer[\ax]
        {A^\perp, A}
        {}
      \]
      \begin{tabbing}
        $A^\perp, \Gamma_2$ \` by $\EE$ 
      \end{tabbing}
    \item [Essential Case:]
      \[
        \DD = \infer[\one]
        {\one, [\ast]^n}
        {}
      \]
      and
      \[
        \EE =
        \infer[\bot]
        {\Gamma_2, \bot}
        {\EE_1 :: \Gamma_2, [\ast]}
      \]
      \begin{tabbing}
        $\Gamma_2, [\ast]^n$ \` by Lemma~\ref{lem:star} on $\EE_1$
      \end{tabbing}
    \item [Essential Case:] 
      \[\DD =
        \infer[\tensor]
        {\Gamma_1, [\Delta_1]\Delta_2, A \tensor B}
        { \DD_1 :: \Delta_1, A
          \quad 
          \DD_2 :: \Gamma_1, \Delta_2, B}
      \] 
      and 
      \[
        \EE = 
        \infer[\parr]
        {\Gamma_2, A^\perp \parr B^\perp}
        {\EE_1 :: \Gamma_2, [A^\perp] B^\perp} 
      \]
        \begin{tabbing}
          $[\Delta_1] \Delta_2, \Gamma_1, \Gamma_2$ \` by i.h.~\ref{cutb} on $\DD_1$, $\DD_2$, and $\EE_1$
      \end{tabbing}
    \item [Essential Case:] \[\DD =     \infer[\with]
        {\Gamma_1,A \oplus B, \oplus\Delta_1,C \with D}
        {\DD_1 :: \Gamma_1, \Left{A \oplus B,\oplus\Delta_1}C
          \quad
          \DD_2 :: \Gamma_1, \Right{A \oplus B,\oplus\Delta_1} D}
      \] and \[ \EE =     \infer[\with]
        {\Gamma_2,\oplus\Delta_2,A^\perp \with B^\perp}
        {\EE_1 :: \Gamma_2, \Left{\oplus\Delta_2}A^\perp
          \quad
          \EE_2 :: \Gamma_2, \Right{\oplus\Delta_2} B^\perp} \]
      \begin{tabbing}
        $ \GG_1 :: \Gamma_1,  \Gamma_2, \Left{\oplus \Delta_1, \oplus \Delta_2} C$ \` by i.h.~\ref{cs1} on $\DD_1$ and $\EE_1$ and $\EE_2$ \\
        $ \GG_2 :: \Gamma_1,  \Gamma_2, \Right{\oplus \Delta_1, \oplus \Delta_2} D$ \` by i.h.~\ref{cs2} on $\DD_2$ and $\EE_1$ and $\EE_2$ \\
        $ \Gamma_1,  \Gamma_2, \oplus \Delta_1, \oplus \Delta_2, C \with D$ \` by $\with$ on $\GG_1$ and $\GG_2$
      \end{tabbing}
    \item [Essential Case:]
      \[\DD =   \infer[\bang]
      {\query \Delta_1, ? A, \bang C} 
      {\DD_1
        :: \Query{\query\Delta_1, ? A} C}
    \]
    and
    \[\EE =
      \infer[\bang]
      {\query \Delta_2, \bang A^\perp} 
      { \EE_1 :: \Query{\query\Delta_2} A^\perp}
    \]

    
    \begin{tabbing}
      $\GG :: \Query {?\Delta_1,\query\Delta_2}C$  \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE_1$\\
      $?\Delta_1,\query\Delta_2, \bang C$  \` by $\bang$ on $\GG$\\
    \end{tabbing}

  \item [Left-Commutative Case:]
    \[\DD  =
      \infer[\bot]
      {\Gamma_1,A, \bot}
      {\DD_1 :: \Gamma_1,A, [\ast]}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, [\ast]$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2, \bot$ \` by $\bot$ on $\GG$
    \end{tabbing}
 \item [Left-Commutative Case:]
   \[\DD  =
     \infer[\tensor]
     {\Gamma_1, A, [\Delta_1]\Delta_2, D \tensor E}
     { \DD_1 :: \Delta_1, D
       \quad
       \DD_2 :: \Gamma_1, A, \Delta_2, E
     }
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, \Delta_2, E$ \` by i.h.~\ref{cuta} on $\DD_2$ and $\EE$ \\
      $\Gamma_1, \Gamma_2, [\Delta_1]\Delta_2,D \tensor E,$ \` by $\tensor$ on $\DD_1$ and $\GG$ \\
    \end{tabbing}

 \item [Left-Commutative Case:]
   \[\DD  =
     \infer[\parr]
     {\Gamma_1, A, D \parr E}
     {\DD_1::\Gamma_1, A, [D] E}     
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, [D]E $ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2, D \parr E$ \` by $\parr$ on $\GG$
    \end{tabbing}

 \item [Left-Commutative Case:]
    \[\DD  =
      \infer[\with]
      {\Gamma_1,A,\oplus\Delta,D \with E}
      {\DD_1 :: \Gamma_1,A, \Left{\oplus\Delta}D
        \quad
        \DD_2 :: \Gamma_1,A, \Right{\oplus\Delta} E}
    \]
    \begin{tabbing}
      $\GG_1 ::\Gamma_1, \Gamma_2, \Left{\oplus\Delta}D $ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\GG_2 ::\Gamma_1, \Gamma_2,  \Right{\oplus\Delta} E$ \` by i.h.~\ref{cuta} on $\DD_2$ and $\EE$ \\
      $\Gamma_1, \Gamma_2, \oplus\Delta,D \with E$ \` by $\with$ on $\GG_1$ and $\GG_2$
    \end{tabbing}

 \item [Left-Commutative Case:]
   \[\DD  =
     \infer[\Left]
     {\Gamma_1,A, \Left{\cdot}C}
     {\DD_1 :: \Gamma_1,A, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, C$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2, \Left{\cdot}C$ \` by $\Left$ on $\GG$
    \end{tabbing}

 \item [Left-Commutative Case:]
    \[\DD  =
      \infer[\Right]
      {\Gamma_1, A, \Right{\cdot}C}
      {\Gamma_1, A, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, C$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2,\Right{\cdot}C$ \` by $\Right$ on $\GG$
    \end{tabbing}

 \item [Left-Commutative Case:]
   \[\DD  =
     \infer[\oplus_1]
     {\Gamma_1, A,  \Left{\Delta, D\oplus E} C}
    {\DD_1::\Gamma_1, A,  \Left{\Delta} C, D}    
  \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Left{\Delta} C, D$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2,\Left{\Delta, D\oplus E} C$ \` by $\oplus_1$ on $\GG$
    \end{tabbing}

 \item [Left-Commutative Case:]
   \[\DD  =  \infer[\oplus_2]
     {\Gamma_1, A, \Right{\Delta, D\oplus E}C}
     {\DD_1 :: \Gamma_1, A,\Right{\Delta} C, E}
   \]
   \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Right{\Delta} C, E$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2,\Right{\Delta, D\oplus E} C$ \` by $\oplus_2$ on $\GG$
   \end{tabbing}


  % \item [Mixed-Left-Commutative Case:]
  %   \[\DD  =
  %     \infer[\bang]
  %     {\query \Delta, \query C, \bang A} 
  %     {\DD_1 :: \Query{\query\Delta, \query C} A}
  %   \]
  %   and
  %   \[\EE =
  %     \infer[\ax]
  %     {\query A^\perp, \bang A}
  %     {}
  %   \]
  %   \begin{tabbing}
  %     $\query \Delta, \query C, \bang A$ \` by $\DD$
  %   \end{tabbing}
  \item [Mixed-Left-Commutative Case:] $\DD$ ending in $\one$ impossible
  \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\bot]
      {\Gamma_2, \query A^\perp, \bot}
      {\EE_1::\Gamma_2,  \query A^\perp,  [\ast]}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, [\ast]$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \bot$ \` by $\bot$ on $\GG$
    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\tensor]
      {\Gamma_2, \query A^\perp,[\Delta_3]\Delta_4, D \tensor E}
      {\EE_1 :: \Delta_3, D \quad \EE_2 ::\Gamma_2,\query A^\perp, \Delta_4, E}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, \Delta_4, E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_2$\\
      $\query \Delta, \query C, \Gamma_2, [\Delta_3]\Delta_4, D \tensor E$ \` by $\tensor$ on $\EE_1$ and $\GG$
    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\parr]
      {\Gamma_2, \query A^\perp,  D \parr E}
      {\EE_1 :: \Gamma_2, \query A^\perp, [D] E}           
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, [D]E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2,  D \parr E$ \` by $\parr$ on $\GG$
    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\with]
      {\Gamma_2, \query A^\perp,\oplus\Delta,D \with E}
      {\EE_1 :: \Gamma_2, \query A^\perp, \Left{\oplus\Delta}D
        \quad
        \EE_2 :: \Gamma_2, \query A^\perp, \Right{\oplus\Delta} E
      }
    \]
    \begin{tabbing}
      $\GG_1 :: \query \Delta, \query C, \Gamma_2, \Left{\oplus\Delta}D $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\GG_2 :: \query \Delta, \query C, \Gamma_2, \Right{\oplus\Delta} E $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_2$\\
      $\query \Delta, \query C, \Gamma_2, \oplus\Delta, D \with E $ \` by $\with$ on $\GG_1$ and $\GG_2$\\
   \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\Left]
      {\Gamma_2, \query A^\perp, \Left{\cdot}D}
      {\EE_1 :: \Gamma_2, \query A^\perp, D}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, D $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \Left{\cdot}D $ \` by $\Left$ on $\GG$ 
    \end{tabbing}
    \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\Right]
      {\Gamma_2, \query A^\perp, \Right{\cdot}D}
      {\EE_1 :: \Gamma_2, \query A^\perp, D}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, D $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \Right{\cdot}D $ \` by $\Right$ on $\GG$ 
    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\oplus_1]
    {\Gamma_2,  \query A^\perp, \Left{\Delta, D\oplus E} C}
    {\EE_1 :: \Gamma_2,  \query A^\perp, \Left{\Delta} C, D}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, \Left{\Delta} C, D$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \Left{\Delta, D\oplus E} C$ \` by $\oplus_1$ on  $\GG$\\
    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\oplus_2]
    {\Gamma_2,  \query A^\perp, \Left{\Delta, D\oplus E} C}
    {\EE_1 :: \Gamma_2,  \query A^\perp, \Left{\Delta} C, E}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, \Left{\Delta} C, E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \Left{\Delta, D\oplus E} C$ \` by $\oplus_2$ on  $\GG$\\
    \end{tabbing}

 \item [Mixed-Left-Commutative Case:] there is no commutative case for $\bang$, $\bang$, other than the essential case. 
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\query]
      {\Gamma_2,  \query A^\perp,\Query{\Delta_2, \query E}D}
      {\EE_1 :: \Gamma_2,  \query A^\perp,\Query{\Delta_2}D, E}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, \Query{\Delta_2}D, E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2, \Query{\Delta_2, \query E}D$ \` by $?$ on $\GG$\\

    \end{tabbing}
 \item [Mixed-Left-Commutative Case:]
    \[\DD  =
      \infer[\bang]
      {\query \Delta, \query C, \bang A} 
      {\DD_1 :: \Query{\query\Delta, \query C} A}
    \]
    and
    \[\EE =
      \infer[\Query]
      {\Gamma_2,  \query A^\perp,\Query{\cdot}C}
      {\EE_1 :: \Gamma_2,  \query A^\perp, C}
    \]
    \begin{tabbing}
      $\GG :: \query \Delta, \query C, \Gamma_2, C$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$\\
      $\query \Delta, \query C, \Gamma_2,\Query{\cdot} C$ \` by $\Query$ on $\GG$       
    \end{tabbing}

  \item [Left-Commutative Case:]
    \[\DD  =     \infer[\query]
      {\Gamma_1,A, \Query{\Delta, \query D}C}
      {\DD_1 :: \Gamma_1,A, \Query{\Delta}C, D}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Query{\Delta}C, D$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2,\Query{\Delta, \query D}C$ \` by $\query$ on $\GG$
    \end{tabbing}
  \item [Left-Commutative Case:]
    \[\DD  =
[      \infer[\Query]
      {\Gamma_1, A, \Query{\cdot}C}
      {\DD_1 :: \Gamma_1, A, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  C$ \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
      $\Gamma_1, \Gamma_2,\Query{}C$ \` by $\Query$ on $\GG$
    \end{tabbing}

    % ################################################################
    % Start
    % ################################################################

    
  \item [Right-Commutative Case:]
    \[\EE  =
      \infer[\bot]
      {\Gamma_2,A^\perp, \bot}
      {\EE_1 :: \Gamma_2,A^\perp, [\ast]}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, [\ast], \Gamma_2$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2, \bot$ \` by $\bot$ on $\GG$
    \end{tabbing}
 \item [Right-Commutative Case:]
   \[\EE  =
     \infer[\tensor]
     {\Gamma_2, A^\perp, [\Delta_1]\Delta_2, D \tensor E}
     { \EE_1 :: \Delta_1, D
       \quad
       \EE_2 :: \Gamma_2, A^\perp, \Delta_2, E
     }
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, \Delta_2, E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2, [\Delta_1]\Delta_2,D \tensor E,$ \` by $\tensor$ on $\DD_1$ and $\GG$ \\
    \end{tabbing}

 \item [Right-Commutative Case:]
   \[\EE  =
]     \infer[\parr]
     {\Gamma_2, A^\perp, D \parr E}
     {\EE_1::\Gamma_2, A^\perp, [D] E}     
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, [D]E $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2, D \parr E$ \` by $\parr$ on $\GG$
    \end{tabbing}

 \item [Right-Commutative Case:]
    \[\EE  =
      \infer[\with]
      {\Gamma_2,A^\perp,\oplus\Delta,D \with E}
      {\EE_1 :: \Gamma_2,A^\perp, \Left{\oplus\Delta}D
        \quad
        \EE_2 :: \Gamma_2,A^\perp, \Right{\oplus\Delta} E}
    \]
    \begin{tabbing}
      $\GG_1 ::\Gamma_1, \Gamma_2, \Left{\oplus\Delta}D $ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\GG_2 ::\Gamma_1, \Gamma_2,  \Right{\oplus\Delta} E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_2$ \\
      $\Gamma_1, \Gamma_2, \oplus\Delta,D \with E$ \` by $\with$ on $\GG_1$ and $\GG_2$
    \end{tabbing}

 \item [Right-Commutative Case:]
   \[\EE  =
     \infer[\Left]
     {\Gamma_2,A^\perp, \Left{\cdot}C}
     {\EE_1 :: \Gamma_2,A^\perp, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, C$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2, \Left{\cdot}C$ \` by $\Left$ on $\GG$
    \end{tabbing}

 \item [Right-Commutative Case:]
    \[\EE  =
      \infer[\Right]
      {\Gamma_2, A^\perp, \Right{\cdot}C}
      {\Gamma_2, A^\perp, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2, C$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2,\Right{\cdot}C$ \` by $\Right$ on $\GG$
    \end{tabbing}

 \item [Right-Commutative Case:]
   \[\EE  =
     \infer[\oplus_1]
     {\Gamma_2, A^\perp,  \Left{\Delta, D\oplus E} C}
    {\EE_1::\Gamma_2, A^\perp,  \Left{\Delta} C, D}    
  \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Left{\Delta} C, D$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2,\Left{\Delta, D\oplus E} C$ \` by $\oplus_1$ on $\GG$
    \end{tabbing}

 \item [Right-Commutative Case:]
   \[\EE  =  \infer[\oplus_2]
     {\Gamma_2, A^\perp, \Right{\Delta, D\oplus E}C}
     {\EE_1 :: \Gamma_2, A^\perp,\Right{\Delta} C, E}
   \]
   \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Right{\Delta} C, E$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2,\Right{\Delta, D\oplus E} C$ \` by $\oplus_2$ on $\GG$
   \end{tabbing}

   %%%% CARSTEN
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\bot]
     {\Gamma_1,\bang A, \bot}
     {\DD_1 :: \Gamma_1, \bang A, [\ast]}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1:: \Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1, [\ast], \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, \bot, \query \Delta, \bang C$
     \` by $\bot$ on $\GG$ 
   \end{tabbing}

    \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\tensor]
     {\Gamma_1, \bang A, [\Delta_1]\Delta_2,  D \tensor E}
     {\DD_1 :: \Delta_1, D \quad \DD_1 :: \Gamma_1,\bang A, \Delta_2, E}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1,  \Delta_2, E, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_2$ and $\EE$ \\
     $\Gamma_1,  [\Delta_1]\Delta_2,  D \tensor E, \query \Delta, \bang C$
     \` by $\tensor$ on $\DD_1$ and $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\parr]
     {\Gamma_1, \bang A, D \parr E}
     {\DD_1 :: \Gamma_1, \bang A, [D] E}     
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1, [D] E, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, D \parr E, \query \Delta, \bang C$
     \` by $\parr$ on $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\with]
     {\Gamma_1, \bang A,\oplus\Delta,D \with E}
     {\DD_1:: \Gamma_1, \bang A, \Left{\oplus\Delta}D
       \quad
       \DD_2 :: \Gamma_1, \bang A, \Right{\oplus\Delta} E}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG_1 :: \Gamma_1, \Left{\oplus\Delta}D, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\GG_2 :: \Gamma_1, \Right{\oplus\Delta} E, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, \oplus\Delta, D \with E, \query \Delta, \bang C$
     \` by $\with$ on $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\Left]
     {\Gamma_1, \bang A, \Left{\cdot}C}
     {\DD_1 :: \Gamma_1, \bang A, C}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1, C, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, \Left{\cdot}C, \query \Delta, \bang C$
     \` by $\Left$ on $\GG$ 
    \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\Right]
     {\Gamma_1, \bang A, \Right{\cdot}C}
     {\DD_1 :: \Gamma_1, \bang A, C}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1, C, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, \Right{\cdot}C, \query \Delta, \bang C$
     \` by $\Right$ on $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\oplus_1]
     {\Gamma_1, \bang A, \Left{\Delta, D\oplus E} C}
     {\DD_1 :: \Gamma_1, \bang A, \Left{\Delta} C, D} 
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1,  \Left{\Delta} C, D, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1,\Left{\Delta, D\oplus E} C, \query \Delta, \bang C$
     \` by $\oplus_1$ on $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\oplus_2]
     {\Gamma_1, \bang A, \Right{\Delta, D\oplus E} C}
     {\DD_2 \Gamma_1, \bang A, \Right{\Delta} C, E} 
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1,  \Right{\Delta} C, E, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1,\Right{\Delta, D\oplus E} C, \query \Delta, \bang C$
     \` by $\oplus_2$ on $\GG$ 
   \end{tabbing}
 \item [Mixed-Right-Commutative Case:] no additional case for $\bang$, $\bang$
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\query]
     {\Gamma_1, \bang A, \Query{\Delta, \query D}C}
     {\DD_1 :: \Gamma, \bang A, \Query{\Delta}C, D}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1,  \Query{\Delta}C, D, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1, \Query{\Delta, \query D}C, \query \Delta, \bang C$
     \` by $\query$ on $\GG$ 

   \end{tabbing}
 \item [Mixed-Right-Commutative Case:]
   \[\DD =
     \infer[\Query]
     {\Gamma_1, \bang A, \Query{\cdot}C}
     {\DD_1 :: \Gamma_1, \bang A, C}
   \]
   and
   \[\EE  =
     \infer[\bang]
     {\query \Delta,\query A^\perp, \bang C} 
     {\EE_1::\Query{\query\Delta,A^\perp} C}
   \]
   \begin{tabbing}
     $\GG :: \Gamma_1, C, \query \Delta, \bang C$
     \` by i.h.~\ref{cuta} on $\DD_1$ and $\EE$ \\
     $\Gamma_1,  \Query{\cdot}C, \query \Delta, \bang C$
     \` by $\Query$ on $\GG$      
   \end{tabbing}

   %%% END CARSTEN
   
  \item [Right-Commutative Case:]
    \[\EE  =     \infer[\query]
      {\Gamma_2,A^\perp, \Query{\Delta, \query D}C}
      {\EE_1 :: \Gamma_2,A^\perp, \Query{\Delta}C, D}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  \Query{\Delta}C, D$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2,\Query{\Delta, \query D}C$ \` by $\query$ on $\GG$
    \end{tabbing}
  \item [Right-Commutative Case:]
    \[\EE  =
      \infer[\Query]
      {\Gamma_2, A^\perp, \Query{\cdot}C}
      {\EE_1 :: \Gamma_2, A^\perp, C}
    \]
    \begin{tabbing}
      $\GG ::\Gamma_1, \Gamma_2,  C$ \` by i.h.~\ref{cuta} on $\DD$ and $\EE_1$ \\
      $\Gamma_1, \Gamma_2,\Query{}C$ \` by $\Query$ on $\GG$
    \end{tabbing}




    % ################################################################
    % End
    % ################################################################
  \end{description}

    % ---------------------------------------------------------------------
  \item by induction on $\FF$. This case is complete.  % 2.
    \begin{description}
    \item [Impossible Cases:] $\ax$, $\one$, $\bang$. 
    \item [Essential Case:] $\FF = \infer[\tensor]
      {\Gamma_3, C \tensor D, [A^\perp]B^\perp}
      {\FF_1 :: A^\perp, C \quad \FF_2 :: \Gamma_3 , B^\perp, D}$ 
      \begin{tabbing}
        $\GG_1 :: \Delta_1, C$ \` by i.h.~\ref{cuta} on $\DD$ and $\FF_1$ \\
        $\GG_2 :: \Delta_2, \Gamma_2, \Gamma_3, D$ \` by i.h.~\ref{cuta} on $\EE$ and $\FF_2$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, C \tensor D$ \` by  $\tensor$ on $\GG_1$ and $\GG_2$
      \end{tabbing}
    \item [Commutative Case:] $\FF = \infer[\tensor]
      {\Gamma_3, [\Delta'_1]\Delta'_2, C \tensor D, [A^\perp]B^\perp}
      {\FF_1 :: \Delta'_1, C \quad \FF_2 :: \Gamma_3 , [A^\perp]B^\perp, \Delta'_2, D}$ 
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Delta_2', D$ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_2$ \\
        $[\Delta'_1] \Delta'_2, C \tensor D,  [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3$ \` by  $\tensor$ on $\FF_1$ and $\GG$
      \end{tabbing}
    \item [Commutative Case:]  $\FF = \infer[\bot]
      {\Gamma_3,  [A^\perp]B^\perp, \bot}
      {\FF_1:: \Gamma_3,  [A^\perp]B^\perp, [\ast]}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, [\ast] $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \bot $ \` by $\bot$ on $\GG$
      \end{tabbing}
    \item [Commutative Case:] $\FF =  \infer[\parr]
      {\Gamma_3, [A^\perp]B^\perp, C \parr D}
      {\FF_1 :: \Gamma_3, [A^\perp]B^\perp, [C] D}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, [C] D  $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, C \parr D $ \` by $\parr$ on $\GG$
      \end{tabbing}
    \item [Commutative Case:] $\FF =  \infer[\with]
      {\Gamma_3, [A^\perp]B^\perp,\oplus\Delta,C \with D}
      {\FF_1 :: \Gamma_3,  [A^\perp]B^\perp,\Left{\oplus\Delta}C
        \quad
        \FF_2 :: \Gamma_3,  [A^\perp]B^\perp,\Right{\oplus\Delta} D}$
      \begin{tabbing}
        $\GG_1 :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\oplus\Delta}C $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $\GG_2 :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3,\Right{\oplus\Delta} D$ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_2$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \oplus \Delta, C \with D$ \` by $\with$ on $\GG_1$ and $\GG_2$
      \end{tabbing}
    \item [Commutative Case:] $\FF =  \infer[\Left]
      {\Gamma_3,  [A^\perp]B^\perp, \Left{\cdot}C}
      {\FF_1::\Gamma_3,  [A^\perp]B^\perp}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3 $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\cdot}C $ \` by $\Left$ on  $\GG$
      \end{tabbing}
    \item [Commutative Case:] $\FF =  \infer[\Right]
      {\Gamma_3,  [A^\perp]B^\perp, \Right{\cdot}C}
      {\FF_1::\Gamma_3,  [A^\perp]B^\perp}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3 $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $[\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Right{\cdot}C $ \` by $\Right$ on  $\GG$
      \end{tabbing}
      
    \item [Commutative Case:] $\FF =  \infer[\oplus_1]
      {\Gamma_3,  [A^\perp]B^\perp, \Left{\Delta, D\oplus E} C}
      {\FF_1::\Gamma_3,  [A^\perp]B^\perp, \Left{\Delta} C, D}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\Delta} C,D $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $ [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\Delta, D \oplus E} C $ \` by $\oplus_1$ on  $\GG$ \\
      \end{tabbing}
      
    \item [Commutative Case:] $\FF =  \infer[\oplus_2]
      {\Gamma_3,  [A^\perp]B^\perp, \Left{\Delta, D\oplus E} C}
      {\FF_1::\Gamma_3,  [A^\perp]B^\perp, \Left{\Delta} C, E}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\Delta} C,E $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $ [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Left{\Delta, D \oplus E} C $ \` by $\oplus_2$ on  $\GG$ \\
      \end{tabbing}
      
    \item [Commutative Case:] $\FF =   \infer[\query]
      {\Gamma_3, [A^\perp]B^\perp, \Query{\Delta, \query D}C}
      {\FF_1 :: \Gamma_3, [A^\perp]B^\perp, \Query{\Delta}C, D}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Query{\Delta}C, D $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $ [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Query{\Delta, ?D}C $ \` by $\query$ on  $\GG$ \\
      \end{tabbing}
      
    \item [Commutative Case:] $\FF = \infer[\Query]
      {\Gamma_3, [A^\perp]B^\perp, \Query{\cdot}C}
      {\FF_1 :: \Gamma_3, [A^\perp]B^\perp}$
      \begin{tabbing}
        $\GG :: [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3 $ \` by i.h.~\ref{cutb} on $\DD$, $\EE$, and $\FF_1$ \\
        $ [\Delta_1] \Delta_2, \Gamma_2, \Gamma_3, \Query{\cdot}C $ \` by $\Query$ on  $\GG$ \\
      \end{tabbing}
      
    \end{description}
    % ---------------------------------------------------------------------
  \item This should be by induction on $\DD$ and $\EE$ % 3.
    % This case is complete.
   % \item If $\DD:: \Gamma_1, \Left{\Delta_1, A \oplus B} C$
   %  and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
   %  then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2} C$.
    \begin{description}
    \item [Impossible Cases:]  $\ax$, $\one$, $\bang$
    \item [Essential Case:]
      \[\DD  =
        \infer[\oplus_1]
        {\Gamma_1,  \Left{\Delta_1, A\oplus B} C}
        {\DD_1 :: \Gamma_1,  \Left{\Delta_1} C, A}\]
      \begin{tabbing}
        $\Gamma_1, \Gamma_2, \Left{\Delta_1, \Delta_2}C$ \` by i.h. \ref{cs11} on $\DD_1$, $\EE$, and $\FF$
      \end{tabbing}
% %%%%%%%%%%
% Left Commutative Cases
% %%%%%%%%%%%%%%%%%
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\bot]
        {\Gamma_1, \Left{\Delta_1, A \oplus B} C, \bot}
        {\DD_1 :: \Gamma_1, \Left{\Delta_1, A \oplus B} C, [\ast]} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2,[\ast], \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$, $\EE$, and $\FF$\\
        $\GG :: \Gamma_1, \Gamma_2, \bot, \Left{\Delta_1,  \Delta_2} C $ \` by $\bot$ on $\GG$
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =  \infer[\tensor]
        {\Gamma_1, \Left{\Delta_1, A \oplus B} C, [\Delta_3]\Delta_4, D \tensor E}
        {\DD_1::\Delta_3, D \quad \DD_2::\Gamma_1, \Left{\Delta_1, A \oplus B} C, \Delta_4, E} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Delta_4, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_2$, $\EE$, and $\FF$\\
        $ \Gamma_1, \Gamma_2, [\Delta_3]\Delta_4, D \tensor E, \Left{\Delta_1,  \Delta_2} C $ \` by $\tensor$ on $\DD_1$ and $\GG$
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
       \infer[\parr]
       {\Gamma_1, \Left{\Delta_1, A \oplus B} C, D \parr E}
       {\DD_1::\Gamma_1, \Left{\Delta_1, A \oplus B} C, [D] E} \]
     \begin{tabbing}
       $\GG :: \Gamma_1, \Gamma_2, [D]E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$, $\EE$, and $\FF$\\
       $ \Gamma_1, \Gamma_2, D \parr E, \Left{\Delta_1,  \Delta_2} C $ \` by $\parr$ on $\GG$ 
      \end{tabbing}

      
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\with]
        {\Gamma_1,\Left{\Delta_1, A \oplus B} C,\oplus\Delta,D \with E}
        {\DD_1 :: \Gamma_1, \Left{\Delta_1, A \oplus B} C,\Left{\oplus\Delta}D
          \quad
          \DD_2 ::\Gamma_1, \Left{\Delta_1, A \oplus B} C,\Right{\oplus\Delta} E}
      \]
      \begin{tabbing}
      $\GG_1 :: \Gamma_1, \Gamma_2, \Left{\oplus\Delta}D , \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$, $\EE$, and $\FF$\\
      $\GG_2 :: \Gamma_1, \Gamma_2, \Right{\oplus\Delta} E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_2$, $\EE$, and $\FF$\\
       $ \Gamma_1, \Gamma_2, D \with E, \Left{\Delta_1,  \Delta_2} C $ \` by $\with$ on $\GG_1$ and $\GG_2$
     \end{tabbing}


    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Left]
        {\Gamma_1,\Left{\Delta_1, A \oplus B} C, \Left{\cdot}D}
        {\DD_1 ::\Gamma_1,\Left{\Delta_1, A \oplus B} C, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$, $\EE$, and $\FF$\\
       $ \Gamma_1, \Gamma_2, \Left{\cdot}D , \Left{\Delta_1,  \Delta_2} C $ \` by $\Left$ on $\GG_1$
      \end{tabbing}

    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Right]
        {\Gamma_1,\Left{\Delta_1, A \oplus B} C, \Right{\cdot} D}
        {\DD_1 :: \Gamma_1,\Left{\Delta_1, A \oplus B} C, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$, $\EE$, and $\FF$\\
       $ \Gamma_1, \Gamma_2, \Right{\cdot}D , \Left{\Delta_1,  \Delta_2} C $ \` by $\Right$ on $\GG_1$
      \end{tabbing}




      
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\oplus_1]
        {\Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Right{\Delta_3, D\oplus E}F}
        {\DD_1 :: \Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Right{\Delta_3} F, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$, $\EE$, and $\FF$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Left{\Delta_1,  \Delta_2} C $ \` by $\oplus_1$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\oplus_2]
        {\Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Right{\Delta_3, D\oplus E}F}
        {\DD_1 :: \Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Right{\Delta_3} F, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$, $\EE$, and $\FF$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Left{\Delta_1,  \Delta_2} C $ \` by $\oplus_2$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  = \infer[\query]
        {\Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Query{\Delta, \query D}E}
        {\DD_1:: \Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Query{\Delta}E, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Query{\Delta}E, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$, $\EE$, and $\FF$\\
        $\Gamma_1, \Gamma_2, \Query{\Delta, \query D}E, \Left{\Delta_1,  \Delta_2} C $ \` by $\query$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Query]
        {\Gamma_1,  \Left{\Delta_1, A \oplus B} C, \Query{\cdot}E}
        {\DD_1 :: \Gamma_1,  \Left{\Delta_1, A \oplus B} C, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs1} on $\DD_1$, $\EE$, and $\FF$\\
        $\Gamma_1, \Gamma_2, \Query{\cdot}E, \Left{\Delta_1,  \Delta_2} C $ \` by $\Query$ on $\GG$      
      \end{tabbing}

%%%XXXXXXXXXX

    \end{description}
  \item This should be by induction on $\DD$ and $\EE$ % 4.
    % This case is complete.
   % \item If $\DD:: \Gamma_1, \Left{\Delta_1, A \oplus B} C$
   %  and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
   %  then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2} C$.
    \begin{description}
    \item [Impossible Cases:]  $\ax$, $\one$, $\bang$
    \item [Essential Case:]
      \[\EE =
        \infer[\Left]
        {\Gamma_2, \Left{\cdot}A^\perp}
        {\EE_1::\Gamma_2, A^\perp}
      \]
      \begin{tabbing}
        $\Gamma_1, \Gamma_2, \Left{\Delta_1}C$ \` by i.h. \ref{cuta} on $\DD$ and $\EE_1$
      \end{tabbing}
      % %%%%%%%%%%%%%%%%%%%
      % Right Commutative Cases
      %%%%%%%%%%%%%%%%%%%%%
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\bot]
        {\Gamma_2, \Left{\Delta_2}A^\perp, \bot}
        {\EE_1 :: \Gamma_2, \Left{\Delta_2}A^\perp, [\ast]} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2,[\ast], \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_1$\\
        $\GG :: \Gamma_1, \Gamma_2, \bot, \Left{\Delta_1,  \Delta_2} C $ \` by $\bot$ on $\GG$
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =  \infer[\tensor]
        {\Gamma_2, \Left{\Delta_2}A^\perp, [\Delta_3]\Delta_4, D \tensor E}
        {\EE_1::\Delta_3, D \quad \EE_2::\Gamma_2, \Left{\Delta_2}A^\perp, \Delta_4, E} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Delta_4, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_2$\\
        $ \Gamma_1, \Gamma_2, [\Delta_3]\Delta_4, D \tensor E, \Left{\Delta_1,  \Delta_2} C $ \` by $\tensor$ on $\EE_1$ and $\GG$
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
       \infer[\parr]
       {\Gamma_2, \Left{\Delta_2}A^\perp, D \parr E}
       {\EE_1::\Gamma_2, \Left{\Delta_2}A^\perp, [D] E} \]
     \begin{tabbing}
       $\GG :: \Gamma_1, \Gamma_2, [D]E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, D \parr E, \Left{\Delta_1,  \Delta_2} C $ \` by $\parr$ on $\GG$ 
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\with]
        {\Gamma_2,\Left{\Delta_2}A^\perp,\oplus\Delta,D \with E}
        {\EE_1 :: \Gamma_2, \Left{\Delta_2}A^\perp,\Left{\oplus\Delta}D
          \quad
          \EE_2 ::\Gamma_2, \Left{\Delta_2}A^\perp,\Right{\oplus\Delta} E}
      \]
      \begin{tabbing}
      $\GG_1 :: \Gamma_1, \Gamma_2, \Left{\oplus\Delta}D , \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_1$\\
      $\GG_2 :: \Gamma_1, \Gamma_2, \Right{\oplus\Delta} E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_2$\\
       $ \Gamma_1, \Gamma_2, D \with E, \Left{\Delta_1,  \Delta_2} C $ \` by $\with$ on $\GG_1$ and $\GG_2$
     \end{tabbing}

    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Left]
        {\Gamma_2,\Left{\Delta_2}A^\perp, \Left{\cdot}D}
        {\EE_1 ::\Gamma_2,\Left{\Delta_2}A^\perp, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, \Left{\cdot}D , \Left{\Delta_1,  \Delta_2} C $ \` by $\Left$ on $\GG_1$
      \end{tabbing}

    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Right]
        {\Gamma_2,\Left{\Delta_2}A^\perp, \Right{\cdot} D}
        {\EE_1 :: \Gamma_2,\Left{\Delta_2}A^\perp, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, \Right{\cdot}D , \Left{\Delta_1,  \Delta_2} C $ \` by $\Right$ on $\GG_1$
      \end{tabbing}

      
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\oplus_1]
        {\Gamma_2,  \Left{\Delta_2}A^\perp, \Right{\Delta_3, D\oplus E}F}
        {\EE_1 :: \Gamma_2,  \Left{\Delta_2}A^\perp, \Right{\Delta_3} F, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Left{\Delta_1,  \Delta_2} C $ \` by $\oplus_1$ on $\GG$      
      \end{tabbing}


      
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\oplus_2]
        {\Gamma_2,  \Left{\Delta_2}A^\perp, \Right{\Delta_3, D\oplus E}F}
        {\EE_1 :: \Gamma_2,  \Left{\Delta_2}A^\perp, \Right{\Delta_3} F, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Left{\Delta_1,  \Delta_2} C $ \` by $\oplus_2$ on $\GG$      
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  = \infer[\query]
        {\Gamma_2,  \Left{\Delta_2}A^\perp, \Query{\Delta, \query D}E}
        {\EE_1:: \Gamma_2,  \Left{\Delta_2}A^\perp, \Query{\Delta}E, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Query{\Delta}E, D, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Query{\Delta, \query D}E, \Left{\Delta_1,  \Delta_2} C $ \` by $\query$ on $\GG$      
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Query]
        {\Gamma_2,  \Left{\Delta_2}A^\perp, \Query{\cdot}E}
        {\EE_1 :: \Gamma_2,  \Left{\Delta_2}A^\perp, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, E, \Left{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs11} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Query{\cdot}E, \Left{\Delta_1,  \Delta_2} C $ \` by $\Query$ on $\GG$      
      \end{tabbing}
    \end{description}
      % ---------------------------------------------------------------------
  \item The proof is analogous to (\ref{cs1}),  simply by replacing $\LL$ by $\RR$. % 5
  \item The proof is analogous to (\ref{cs11}),  simply by replacing $\LL$ by $\RR$. % 6

      % ---------------------------------------------------------------------
  \item This should be by induction on $\DD$ and $\EE$ % 7.
    \begin{description}
    \item [Impossible Cases:]  $\ax$, $\one$, $\bang$
    \item [Essential Case:]
      \[\DD  =
        \infer[\query]
        {\Gamma_1, \Query{\Delta_1, \query A}C}
        {\DD_1::\Gamma_1, \Query{\Delta_1}C, A}
      \]
      \begin{tabbing}
        $\Gamma_1, \Gamma_2,  \Query {\Delta_1, \Delta_2}C$ \` by i.h. \ref{cs33} on $\DD_1$ and $\EE$
      \end{tabbing}
   % %%%%%%%%%%%%%%%%%
% Left Commutative Cases
% %%%%%%%%%%%%%%%%%
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\bot]
        {\Gamma_1,\Query{\Delta_1,\query A} C, \bot}
        {\DD_1 :: \Gamma_1,\Query{\Delta_1,\query A} C, [\ast]} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2,[\ast], \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
        $\GG :: \Gamma_1, \Gamma_2, \bot, \Query{\Delta_1,  \Delta_2} C $ \` by $\bot$ on $\GG$
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =  \infer[\tensor]
        {\Gamma_1,\Query{\Delta_1,\query A} C, [\Delta_3]\Delta_4, D \tensor E}
        {\DD_1::\Delta_3, D \quad \DD_2::\Gamma_1,\Query{\Delta_1,\query A} C, \Delta_4, E} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Delta_4, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_2$ and $\EE$\\
        $ \Gamma_1, \Gamma_2, [\Delta_3]\Delta_4, D \tensor E, \Query{\Delta_1,  \Delta_2} C $ \` by $\tensor$ on $\DD_1$ and $\GG$
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
       \infer[\parr]
       {\Gamma_1,\Query{\Delta_1,\query A} C, D \parr E}
       {\DD_1::\Gamma_1,\Query{\Delta_1,\query A} C, [D] E} \]
     \begin{tabbing}
       $\GG :: \Gamma_1, \Gamma_2, [D]E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, D \parr E, \Query{\Delta_1,  \Delta_2} C $ \` by $\parr$ on $\GG$ 
      \end{tabbing}

      
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\with]
        {\Gamma_1,\Query{\Delta_1,\query A} C,\oplus\Delta,D \with E}
        {\DD_1 :: \Gamma_1,\Query{\Delta_1,\query A} C,\Left{\oplus\Delta}D
          \quad
          \DD_2 ::\Gamma_1,\Query{\Delta_1,\query A} C,\Right{\oplus\Delta} E}
      \]
      \begin{tabbing}
      $\GG_1 :: \Gamma_1, \Gamma_2, \Left{\oplus\Delta}D , \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
      $\GG_2 :: \Gamma_1, \Gamma_2, \Right{\oplus\Delta} E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_2$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, D \with E, \Query{\Delta_1,  \Delta_2} C $ \` by $\with$ on $\GG_1$ and $\GG_2$
     \end{tabbing}


    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Left]
        {\Gamma_1,\Query{\Delta_1,\query A} C, \Left{\cdot}D}
        {\DD_1 ::\Gamma_1,\Query{\Delta_1,\query A} C, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, \Left{\cdot}D , \Query{\Delta_1,  \Delta_2} C $ \` by $\Left$ on $\GG_1$
      \end{tabbing}

    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Right]
        {\Gamma_1, \Query{\Delta_1,\query A} C, \Right{\cdot} D}
        {\DD_1 :: \Gamma_1,\Query{\Delta_1,\query A} C, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
       $ \Gamma_1, \Gamma_2, \Right{\cdot}D , \Query{\Delta_1,  \Delta_2} C $ \` by $\Right$ on $\GG_1$
      \end{tabbing}

    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\oplus_1]
        {\Gamma_1, \Query{\Delta_1,\query A} C, \Right{\Delta_3, D\oplus E}F}
        {\DD_1 :: \Gamma_1, \Query{\Delta_1,\query A} C, \Right{\Delta_3} F, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Query{\Delta_1,  \Delta_2} C $ \` by $\oplus_1$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\oplus_2]
        {\Gamma_1, \Query{\Delta_1,\query A} C, \Right{\Delta_3, D\oplus E}F}
        {\DD_1 :: \Gamma_1, \Query{\Delta_1,\query A} C, \Right{\Delta_3} F, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Query{\Delta_1,  \Delta_2} C $ \` by $\oplus_2$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  = \infer[\query]
        {\Gamma_1, \Query{\Delta_1,\query A} C, \Query{\Delta, \query D}E}
        {\DD_1:: \Gamma_1, \Query{\Delta_1,\query A} C, \Query{\Delta}E, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Query{\Delta}E, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Query{\Delta, \query D}E, \Query{\Delta_1,  \Delta_2} C $ \` by $\query$ on $\GG$      
      \end{tabbing}
    \item [Left-Commutative Case:]
      \[\DD  =
        \infer[\Query]
        {\Gamma_1, \Query{\Delta_1,\query A} C, \Query{\cdot}E}
        {\DD_1 :: \Gamma_1, \Query{\Delta_1,\query A} C, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs3} on $\DD_1$ and $\EE$\\
        $\Gamma_1, \Gamma_2, \Query{\cdot}E, \Query{\Delta_1,  \Delta_2} C $ \` by $\Query$ on $\GG$      
      \end{tabbing}

    \end{description}

  \item This should be by induction on $\DD$ and $\EE$ % 8.
    % This case is complete.
   % \item If $\DD:: \Gamma_1, \Left{\Delta_1, A \oplus B} C$
   %  and $ \EE :: \Gamma_2, \Left{\Delta_2} A^\perp$
   %  then $ \Gamma_1,  \Gamma_2, \Left{\Delta_1, \Delta_2} C$.
    \begin{description}
    \item [Impossible Cases:]  $\ax$, $\one$, $\bang$
    \item [Essential Case:]
      \[\EE =
        \infer[\Query]
        {\Gamma_2, \Query{\cdot}A^\perp}
        {\EE_1::\Gamma_2, A^\perp}
      \]
      \begin{tabbing}
        $\Gamma_1, \Gamma_2,  \Query {\Delta_1}C$ \` by i.h. \ref{cuta} on $\DD$ and $\EE_1$
      \end{tabbing}
    \item [Essential Case:]
      \[\EE =
        \infer[\Query]
        {\Gamma_2, \Query{\Delta_2,\query D}A^\perp}
        {\EE_1::\Gamma_2, D, \Query{\Delta_2}A^\perp}
      \]
      \begin{tabbing}
        $\GG::\Gamma_1, \Gamma_2,D,  \Query {\Delta_1,\Delta_2}C$ \` by i.h. \ref{cs33} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2,  \Query {\Delta_1, \Delta_2, \query D}C$ \` by $\Query$ on $\GG$
      \end{tabbing}
      % %%%%%%%%%%%%%%%%%%%
      % Right Commutative Cases
      %%%%%%%%%%%%%%%%%%%%%
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\bot]
        {\Gamma_2, \Query{\Delta_2}A^\perp, \bot}
        {\EE_1 :: \Gamma_2, \Query{\Delta_2}A^\perp, [\ast]} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2,[\ast], \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_1$\\
        $\GG :: \Gamma_1, \Gamma_2, \bot, \Query{\Delta_1,  \Delta_2} C $ \` by $\bot$ on $\GG$
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =  \infer[\tensor]
        {\Gamma_2, \Query{\Delta_2}A^\perp, [\Delta_3]\Delta_4, D \tensor E}
        {\EE_1::\Delta_3, D \quad \EE_2::\Gamma_2, \Query{\Delta_2}A^\perp, \Delta_4, E} \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Delta_4, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_2$\\
        $ \Gamma_1, \Gamma_2, [\Delta_3]\Delta_4, D \tensor E, \Query{\Delta_1,  \Delta_2} C $ \` by $\tensor$ on $\EE_1$ and $\GG$
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
       \infer[\parr]
       {\Gamma_2, \Query{\Delta_2}A^\perp, D \parr E}
       {\EE_1::\Gamma_2, \Query{\Delta_2}A^\perp, [D] E} \]
     \begin{tabbing}
       $\GG :: \Gamma_1, \Gamma_2, [D]E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, D \parr E, \Query{\Delta_1,  \Delta_2} C $ \` by $\parr$ on $\GG$ 
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\with]
        {\Gamma_2,\Query{\Delta_2}A^\perp,\oplus\Delta,D \with E}
        {\EE_1 :: \Gamma_2, \Query{\Delta_2}A^\perp,\Left{\oplus\Delta}D
          \quad
          \EE_2 ::\Gamma_2, \Query{\Delta_2}A^\perp,\Right{\oplus\Delta} E}
      \]
      \begin{tabbing}
      $\GG_1 :: \Gamma_1, \Gamma_2, \Left{\oplus\Delta}D , \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_1$\\
      $\GG_2 :: \Gamma_1, \Gamma_2, \Right{\oplus\Delta} E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_2$\\
       $ \Gamma_1, \Gamma_2, D \with E, \Query{\Delta_1,  \Delta_2} C $ \` by $\with$ on $\GG_1$ and $\GG_2$
     \end{tabbing}

    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Left]
        {\Gamma_2,\Query{\Delta_2}A^\perp, \Left{\cdot}D}
        {\EE_1 ::\Gamma_2,\Query{\Delta_2}A^\perp, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, \Left{\cdot}D , \Query{\Delta_1,  \Delta_2} C $ \` by $\Left$ on $\GG_1$
      \end{tabbing}

    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Right]
        {\Gamma_2,\Query{\Delta_2}A^\perp, \Right{\cdot} D}
        {\EE_1 :: \Gamma_2,\Query{\Delta_2}A^\perp, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_1$\\
       $ \Gamma_1, \Gamma_2, \Right{\cdot}D , \Query{\Delta_1,  \Delta_2} C $ \` by $\Right$ on $\GG_1$
      \end{tabbing}

      
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\oplus_1]
        {\Gamma_2,  \Query{\Delta_2}A^\perp, \Right{\Delta_3, D\oplus E}F}
        {\EE_1 :: \Gamma_2,  \Query{\Delta_2}A^\perp, \Right{\Delta_3} F, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Query{\Delta_1,  \Delta_2} C $ \` by $\oplus_1$ on $\GG$      
      \end{tabbing}


      
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\oplus_2]
        {\Gamma_2,  \Query{\Delta_2}A^\perp, \Right{\Delta_3, D\oplus E}F}
        {\EE_1 :: \Gamma_2,  \Query{\Delta_2}A^\perp, \Right{\Delta_3} F, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Right{\Delta_3} F, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Right{\Delta_3, D\oplus E} F, \Query{\Delta_1,  \Delta_2} C $ \` by $\oplus_2$ on $\GG$      
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  = \infer[\query]
        {\Gamma_2,  \Query{\Delta_2}A^\perp, \Query{\Delta, \query D}E}
        {\EE_1:: \Gamma_2,  \Query{\Delta_2}A^\perp, \Query{\Delta}E, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, \Query{\Delta}E, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Query{\Delta, \query D}E, \Query{\Delta_1,  \Delta_2} C $ \` by $\query$ on $\GG$      
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  = \infer[\query]
        {\Gamma_2,  \Query{\Delta_2,\query D}A^\perp}
        {\EE_1:: \Gamma_2,  \Query{\Delta_2}A^\perp, D}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, D, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Query{\Delta_1,  \Delta_2, \query D} C $ \` by $\query$ on $\GG$      
      \end{tabbing}
    \item [Right-Commutative Case:]
      \[\EE  =
        \infer[\Query]
        {\Gamma_2,  \Query{\Delta_2}A^\perp, \Query{\cdot}E}
        {\EE_1 :: \Gamma_2,  \Query{\Delta_2}A^\perp, E}
      \]
      \begin{tabbing}
        $\GG :: \Gamma_1, \Gamma_2, E, \Query{\Delta_1,  \Delta_2} C $ \` by i.h.~\ref{cs33} on $\DD$ and $\EE_1$\\
        $\Gamma_1, \Gamma_2, \Query{\cdot}E, \Query{\Delta_1,  \Delta_2} C $ \` by $\Query$ on $\GG$      
      \end{tabbing}
    \end{description}
    
  \end{enumerate}
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

==> calculus.tex <==
\section{Processes}\label{sec:calculus}
We now introduce the syntax of processes, the language we use to
express entities that communicate over channel endpoints.
% %
% We then identify exactly when a process is a forwarder, based on
% purely syntactic properties that formalise the three principles i) \emph{no message loss}, 
% ii) \emph{no data processing}, and iii) \emph{no message creation}, that we discussed in the introduction. 
%In the next sections, we
%will introduce some mechanisms based on logic that guarantee forwarder
%compositionality, as well as in \S~\ref{sec:sync_system}, we will
%consider a set of forwarder satisfying principle iv).
% Well-typed forwarders also satisfy principle iv) (see
% Section~\ref{sec:core_system}), even when restricted to those
% satifying principle v) (see Section~\ref{sec:sync_system}).

% \noindent {\bf Processes.}
% \subsection{Processes}
Our process language is a variant of the $\pi$-calculus~\cite{MPW92}
with specific communication primitives as usually done for session
calculi. Moreover, given that the theory of this paper is based on the
Curry-Howard correspondence with classical linear logic, we adopt a
syntax akin to that of \cite{W14}. Below, let
$\phl{\mathcal N}$ be a set of names, ranged over by
$\phl{x,y,z,\ldots}$ and used for denoting communication endpoints.
%
\begin{displaymath}
  \small
  \begin{array}{l@{\quad}l@{\quad}l@{\qquad}l@{\quad}l@{\quad}l@{\qquad}l}
    \phl P,\phl Q ::= & \fwd xy          & \text{(link)}
    &
      \phl{\res {xy} (P\!\!\pp\!\! Q)} & \text{(parallel)}
    \\
                      & \wait x P & \text{(wait)}
    &
      \close x & \text{(close)}
    \\
                      & \recv xyP        & \text{(input)}
                
    &
      \send xyPQ       & \text{(output)}
    \\
    % & \recvtype xXP & \text{receive type}
    % &
    % \sendtype xAP & \text{send type}
    % \\
            & \Case xPQ        & \text{(choice)}
    & \inl xP          & \text{(left select)} \\
& & & \inr xP & \text{(right select)}
    \\
            & \client xyP & \text{(client request)}
    &
      \srv xyP & \text{(server accept)}
  
  \end{array}
\end{displaymath}
% \sonia{Do we need the $\bf 0$ process?}
%
We briefly comment on the various production of the grammar above. A link
$\fwd xy$ is a binary forwarder, i.e., a process that forwards any
communication between endpoint $\phl x$ and endpoint $\phl y$. This
yields a sort of equality relation on names: it says that endpoints
$\phl x$ and $\phl y$ are equivalent, and communicating something over
$\phl x$ is like communicating it over $\phl y$.
%
The term $\phl{\res {xy}(P\pp Q)}$ is used for composing processes: it
is the parallel composition of $\phl P$ and $\phl Q$ that share a
private connection through endpoints $\phl x$ and $\phl y$.
% 
Although not used in the definition of forwarders, parallel
composition is needed to formally define forwarder compositionality
and is used when we study the semantics of forwarders in
\S~\ref{sec:core_system} and \S~\ref{sec:sync_system}.
%
Note that we use endpoints instead of channels. The difference is
subtle: the restriction here $\phl{\res {xy}}$
connects the two endpoints $\phl x$ and $\phl y$, instead of referring to the channel between them.
%
The terms $\wait xP$ and $\close x$ handle synchronisation (no message
passing); $\wait xP$ can be seen as an empty input on $\phl x$, while
$\close x$ terminates the execution of the process.
%
The term $\send xyPQ$ denotes a process that creates a fresh name
$\phl y$, spawns a new process $\phl P$, and then continues as
$\phl Q$. The intuition behind this communication operation is that
$\phl P$ uses $\phl y$ as an interface for dealing with the
continuation of the dual primitive (denoted by term $\recv xyR$, for
some $\phl R$).
%
We observe that \cite{W12} uses the syntax $x[y].(P\pp Q)$, but we
believe that our version is more intuitive and gives a better
explanation of why we require two different processes to follow after an
output. However, our format is slightly more restrictive, since
$\phl y$ is forced to be bound in $\phl P$. Also, note that output
messages are always fresh, as for the internal
$\pi$-calculus~\cite{S96}, hence the output term $\send xyPQ$ is a
compact version of the $\pi$-calculus term
$(\nu y)\, \overline x y.(P\pp Q)$.
%\sonia{do you mean $\nu y$?}
%
Branching computations are handled by $\Case xPQ$, $\inl xP$ and
$\inr xP$. The former denotes a process offering two options (external
choice) from which some other process can make a selection with
$\inl xP$ or $\inr xP$.
%
Finally, the term $\srv xyP$ denotes a persistently available service
that can be invoked by $\client xzQ$ at $\phl x$ which will spawn a
new session to be handled by a copy of process $\phl P$.


\begin{example}[2-Buyer Protocol]\label{ex:2buyer}
  Recall the 2-buyer protocol from the introduction, with a forwarder
  process (below $\phl{P_1}$) between buyers $\phl{B_1}$,
  $\phl{B_2}$ who try to make a joint decision whether to buy a book
  from seller $\phl{S}$ or not, and another forwarder (below
  $\phl{P_2}$), delegating $\phl{B_2}$'s decision to two colleagues,
  $\phl{C_1}$ and $\phl{C_2}$.
  %
  We now present both processes in our syntax, where $\phl{b_1}$,
  $\phl{b_2}$, and $\phl s$ are the endpoints connecting the forwarder
  $\phl{P_1}$ to $\phl{B_1}$, $\phl{B_2}$, and $\phl S$ respectively,
  and $\phl{b'_2}$, $\phl{c_1}$, and $\phl{c_2}$ are the endpoints
  connecting the forwarder $\phl{P_2}$ to $\phl{B_2}$, $\phl{C_1}$,
  and $\phl{C_2}$.  Note, that forwarder $\phl{B_2}$ is connected
  through two endpoints $\phl{b_2}$ and $\phl{b_2'}$ to forwarders
  $\phl{P_1}$ and $\phl{P_2}$, respectively.
  % \sonia{$\phl{b_2}$ is used twice, once between $\phl{P_1}$ and $\phl{B_2}$ and then between $\phl{P_2}$ and $\phl{B_2}$.
  % I suppose it does not pose a problem theoretically but maybe for clarity? }
  % which is a variant of the well-known 2-buyer
  % protocol from~\cite{HYC08}, that can be found in~\cite{CLMSW16}. The
  % protocol consists of two buyers, say $B_1$ and $B_2$, attempting to
  % purchase a book together from some seller $S$. The first buyer,
  % $B_1$, sends a request to the seller $S$, which reacts by sending
  % back a quote to both $B_1$ and $B_2$. At this point, $B_1$ writes to
  % $B_2$ proposing a percentage of the price it is willing to
  % pay. Finally, $B_2$ decides whether to accept such a sharing or to
  % reject it. In terms of forwarders, we can think of such forwarder as
  % a process that works as a medium component re-distributing messages
  % between the three players:
  \begin{eqnarray*}
    \phl{P_1} &=& \begin{array}[t]{@{}l}
                    \recv {b_1}{n} {\send{s}{n'}{\fwd{n}{n'}}{}}  
                    \recv {s}{x_1} {\send{b_1}{x'_1}{\fwd{x_1}{x'_1}}{}} 
                    \recv {s}{x_2} {\send{b_2}{x'_2}{\fwd{x_2}{x'_2}}{}} \\
                    \recv {b_1}{y} {\send{b_2}{y'}{\fwd{y}{y'}}{}} 
                    \Case {b_1}{\inl{s}{\recv {b_2}{a} {\send{s}{a'}{\fwd{a}{a'}}Q_1}}}{\inr{s}Q_1} \\
                  \end{array} \\
    \phl{P_2} &=& \begin{array}[t]{@{}l}
                    \recv {b_2'}{y_1} {\send{c_1}{y_1'}{\fwd{y_1}{y_1'}}{}} 
                    \recv {b_2'}{y_2} {\send{c_2}{y_2'}{\fwd{y_2}{y_2'}}{}} \\
                    \Case {c_1}{\Case{c_2}{\inl{b_2'}Q_2}{\inr{b_2'}Q_2}}
                    {\Case{c_2}{\inr{b_2'}Q_2}{\inr{b_2'}Q_2}}
                  \end{array}
  \end{eqnarray*}
  The processes $\phl{Q_1} = \wait{b_1}{\wait{b_2}{\close{s}}}$ and
  $\phl{Q_2} =\wait{c_1}{\wait{c_2}{\close{b_2'}}}$ close all
  endpoints.
  % and they are the same in the branches in their respective terms.
  % We factor them out simply to improve the readability of the process
  % terms.
  \qed
% =======
%   \marco{OLD, havent looked at it yet} We now give an example of a
%   process in our syntax which is a variant of the well-known 2-buyer
%   protocol from~\cite{HYC08}, that can be found in~\cite{CLMSW16}. The
%   protocol consists of two buyers, say $B_1$ and $B_2$, attempting to
%   purchase a book together from some seller $S$. The first buyer,
%   $B_1$, sends a request to the seller $S$, which reacts by sending
%   back a quote to both $B_1$ and $B_2$. At this point, $B_1$ writes to
%   $B_2$ proposing a percentage of the price it is willing to
%   pay. Finally, $B_2$ decides whether to accept such a sharing or to
%   reject it. In terms of forwarders, we can think of such forwarder as
%   a process that works as a medium component re-distributing messages
%   between the three players:

%   \[\phl{P_1} = \begin{array}[t]{l}
%                     \recv {b_1}{n} {\send{s}{n'}{\fwd{n}{n'}}{}} 
%                     \recv {s}{x_1} {\send{b_1}{x'_1}{\fwd{x_1}{x'_1}}{}}
%                     \recv {s}{x_2} {\send{b_2}{x'_2}{\fwd{x_2}{x'_2}}{}}
%                    \recv {b_1}{y} {\send{b_2}{y'}{\fwd{y}{y'}}{}} \\
%                    \Case {b_1}{\inl{s}{\recv {b_2}{a}
%                    {\send{s}{a'}{\fwd{a}{a'}}{\wait{b_1}{\wait{b_2}{\close{s}}}}}}}{\inr{s}{\wait{b_1}{\wait{b_2}{\close{s}}}}}
%                  \end{array}\]
%                \[\phl{P_2} = \begin{array}[t]{l}
%                                 \recv {b_1}{n} {\send{s}{n'}{\fwd{n}{n'}}{}} 
%                     \recv {s}{x_1} {\send{b_1}{x'_1}{\fwd{x_1}{x'_1}}{}}
%                     \recv {s}{x_2} {\send{b_2}{x'_2}{\fwd{x_2}{x'_2}}{}}
%                     \recv {b_1}{y} {\send{b_2}{y'}{\fwd{y}{y'}}{}} \\
%                     \Case {b_1}{\inl{s}{\recv {b_2}{a} {\send{s}{a'}{\fwd{a}{a'}}{\wait{b_1}{\wait{b_2}{\close{s}}}}}}}{\inr{s}{\wait{b_1}{\wait{b_2}{\close{s}}}}} 
%                   \end{array}\]
  
% >>>>>>> 8b68b16c87c5d570d781af116024aa4f0ce9a0c1
%   \[
%   \phl{P_{a}} = \ba{@{}l@{}} \recv{b_1}{b_1'}{\sendc{s}{s'}{\cpaxiom
%       {b_1'}{}{s'}{% \tname
%       }} \recv{s}{s'}{\sendc{b_1}{b_1'}{\cpaxiom{s'}{}{b_1'}{% \tcost
%         }}}} \\
%   \quad \recv{s}{s'}{\sendc{b_2}{b_2'}{\cpaxiom{s'}{}{b_2'}{% \tcost
%       }}
%     \recv{b_1}{b_1'}{\sendc{b_2}{b_2'}{\cpaxiom{b_1'}{}{b_2'}{% \tcost
%         }}}} \\
%   \qquad
%   \Case{b_2}{\inl{s}{\recv{b_2}{b_2'}{\send{s}{s'}{\cpaxiom{b_2'}{}{s'}{% \taddr
%           }}{\wait{b_1}{\wait{b_2}{\close{s}}}}}}}
%   {\inr{s}{\wait{b_1}{\wait{b_2}{\close{s}}}}})))) \\
%   \ea
% \]
\end{example}

Next, we turn to the type system for processes.  Among all of the many process expressionis one can write,
classical linear logic (CLL)~\cite{W12}  characterizes the subset that is well-behaved, i.e.\ they satisfy dead-lock freedom and sesion fidelity, and 
therefore interesting for our work.  For completeness reasons, we depict the rules in Figure~\ref{fig:cp_rules}. 

% \subsection{CLL and corresponding CP processes\label{sec:cll}
 \begin{figure}[t]
\begin{displaymath}
	\small
	\begin{array}{c}
		\infer[\textsc{Axiom}]
		{\phl{\cpaxiom{x}{A^\perp}{y}{A}} \seq \phl x:\thl {A^\bot}, \phl y:\thl{A}}
		{ }
		\qquad
		\infer[\bot]
		{\phl {\wait xP} \seq \thl \Gamma, \phl x:\thl\bot}
		{\phl P \seq \thl\Gamma}
		\qquad
		\infer[\one]
		{\phl{\close x} \seq \phl x: \thl\one}
		{ }
		%		\quad\qquad
		%		\text{(no rule for $\zero$)}
		%		\quad\qquad
		%		\infer[\top]
		%		{\phl{\emptyCase x\seq \thl{\Gamma}}, \phl x:\thl\top}
		%		{ }    
		\\[1ex]
		\infer[\tensor]
		{
			\phl{\send xyPQ} 
			\seq 
			\thl{\Gamma}, \thl{\Delta}, \phl x:\thl{A \tensor B}
		}
		{
			\phl P 
			\seq 
			\thl{\Gamma}, \phl y:\thl A
			& \phl Q 
			\seq 
			\thl \Delta, \phl x: \thl B
		}
		\qquad\qquad\qquad
		\infer[\parr]
		{\phl{\recv xyP} 
			\seq \thl{\Gamma}, \phl x: \thl {A \parr B}
		}       
		{\phl P \seq \thl{\Gamma}, \phl y:\thl A, \phl x:\thl B}
		\\[1ex]
		\infer[\oplus_1]
		{\phl{\inl xP} \seq \thl\Gamma, \phl x:\thl{A \oplus B}}
		{\phl P \seq \thl\Gamma, \phl x:\thl A}
		\qquad
		\infer[\oplus_2]
		{\phl{\inr xP} \seq \thl\Gamma, \phl x:\thl{A \oplus B}}
		{\phl P \seq \thl\Gamma, \phl x:\thl B}
		\qquad
		\infer[\with]
		{\phl{\Case xPQ} \seq \thl \Gamma, \phl x:\thl{A \with B}}
		{\phl P \seq \thl\Gamma, \phl x:\thl A & \phl Q \seq
			\thl\Gamma, \phl
			x:\thl B}
		\\[1ex]
		\infer[?]
		{\phl{\client xyP} \seq \thl \Gamma, \phl x:\thl {\query A}}
		{\phl P \seq \thl \Gamma, \phl y:\thl A}
		\qquad\qquad
		\infer[!]
		{\phl{\srv xyP} \seq \,\thl{\query \Gamma}, \phl x:\thl{\bang A}}
		{\phl P \seq \,\thl{\query \Gamma}, \phl y:\thl A}
		% \qquad\qquad
		% \infer[\textsc{Weaken}]
		% {\phl P \seq \thl \Gamma, \phl x:\thl{\query A}}
		% {\phl P \seq \thl \Gamma}
		% \\[1ex]
		% \infer[\exists]
		% {\phl{\sendtype xAP} \seq \thl \Gamma, \phl x:\thl{\exists X.B}}
		% {\phl P \seq \thl \Gamma, \phl x:\thl{B[A/X]}}
		% \ \quad
		% \infer[\forall]
		% {\phl{\recvtype xXP} \seq \thl\Gamma, \phl x:\thl{\forall X.B}}
		% {\phl P \seq \thl\Gamma, \phl x:\thl B & \thl X \notin \m{ftv}(\thl \Gamma)}
		% \ \quad
		% \infer[\textsc{Contract}]
		% {\phl{P\{x/y, x/z\}} \seq \thl\Gamma, \phl x:\thl{\query A}}
		% {\phl P \seq \thl\Gamma, \phl y:\thl{\query A}, \phl
		%   z:\thl{\query A}}
		\\[1ex]
		\qquad\qquad
		\infer[\textsc{Cut}]
		{\phl{\cpres{x}A{y}{A^\perp}(P \pp Q)} \seq \thl\Gamma,\thl\Delta}
		{\phl P \seq \thl\Gamma, \phl x:\thl A & \phl Q \seq \thl\Delta,
			\phl y:\thl{\dual{A}}}
	\end{array}
\end{displaymath}
   \caption{Classical Linear Logic and CP}
   \label{fig:cp_rules}
\end{figure}


% \smallbreak
% \noindent {\bf Forwarders.}


%
%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> carsten.tex <==
%We can now define the semantics based on proof transformations in the
%logic. Everything seems to be identical:
%
%Structural equivalence (Processes)
%\[
%\ba{@{}l@{}}
%      \phl{\cpaxiom yAx{\dual A}}
%        \equiv
%         \phl{\cpaxiom x{\dual A}yA} \qquad
%      \phl{\cpres y{\dual{A}}xA(Q \pp P)}  
%        \equiv
%         \phl{\cpres xAy{\dual A} (P \pp Q)} \\
%      \phl{\cpres wBz{\dual B} (P \pp \cpres xAy{\dual A} (Q \pp R))}
%        \equiv
%           \phl{\cpres xAy{\dual A}(\cpres wBz{\dual B} (P \pp Q) \pp R)} \\
%\ea
%\]
%%
%%  \multicolumn{3}{@{}c@{}}
%% {\infer{\phl{\cpres xAy{\dual A}(P \pp R)}
%%          \equiv \phl{\cpres xAy{\dual A}(Q \pp \til R)}}
%%       {\phl P \equiv \phl Q}} \\
%%
%$\eta$-expansions (Processes)
%  \[\ba{rcl@{\quad}rcl}
%    % (\eta_{\parr\tensor})&
%      \phl{\cpaxiom{x}{\dual A \parr \dual B}{y}{A \tensor B}}
%      &\reducesto&
%      \phl{\recv xu{\send yv{\cpaxiom{u}{\dual A}{v}{A}}{\cpaxiom{x}{\dual B}{y}{B}}}} &
%    % (\eta_{\perp\one})&
%      \phl{\cpaxiom{x}{\perp}{y}{\one}}
%      &\reducesto&
%      \phl{\wait{x}{\close{y}}} \\
%    % (\eta_{\with\oplus})&
%      \phl{\cpaxiom{x}{\dual A \with \dual B}{y}{A \oplus B}}
%      &\reducesto&
%      \phl{\Case x{\inl y{\cpaxiom{x}{\dual A}{y}{A}}}{\inr y {\cpaxiom{x}{\dual B}{y}{B}}}} &
%    % (\eta_{\top\zero})&
%      \phl{\cpaxiom{x}{\top}{y}{\zero}}
%      &\reducesto& \phl{\emptyCase x} \\
%    % (\eta_{\bang\query})&
%      \phl{\cpaxiom{x}{\bang \dual A}{y}{\query A}}
%      &\reducesto&
%      \phl{\srv xu{\client yv{\cpaxiom{u}{\dual A}{v}{A}}}} &
%    % (\eta_{\forall\exists})&
%      \phl{\cpaxiom{x}{\forall X.\dual A}{y}{\exists X.A}}
%      &\reducesto&
%      \phl{\recvtype xX{\sendtype yX{\cpaxiom{x}{\dual A}{y}{A}}}}
%  \ea\]
%%
%$\beta$-reductions (Processes)
%  \begin{equations}
%      % (\m{AxCut}) &
%        \phl{\cpres x{X}y{\dual X} ( \cpaxiom w{\dual X}x{X} \pp Q)}
%        &\reducesto&
%        \phl{Q \substone wy}
%      \\
%      % (\beta_{\tensor\parr}) &
%        \phl{\cpres{x}{A\tensor B}{y}{\dual A\parr \dual B}
%        (\send xuPQ  \pp \recv yvR)}
%        &\reducesto&
%        \phl{\cpres{u}{A}{v}{\dual A}
%        (P  \pp \cpres xBy{\dual B} (Q\pp R))}
%      \\
%      % (\beta_{\one\perp}) &
%        \phl{\cpres x{\one}y\perp(\close x\pp \wait yP)}
%        &\reducesto&
%        \phl{P}
%      \\
%      % (\beta_{\oplus\with_1}) &
%        \phl{\cpres x{A\oplus B}y{\dual A\with \dual B} (\inl xP\pp \Case xQR)}
%        &\reducesto&
%        \phl{\cpres xAy{\dual A} (P\pp Q)}
%      \\
%      % (\beta_{\oplus\with_2}) &
%        \phl{\cpres x{A\oplus B}y{\dual A\with \dual B} (\inr xP\pp \Case xQR)}
%        &\reducesto&
%        \phl{\cpres x{B}y{\dual B} (P\pp R)}
%      \\
%      % (\beta_{\zero\top}) &
%        & \makebox[0em][c]{\text{(no rule for $\zero$ with $\top$)}} &
%      \\
%      % (\beta_{!?}) &
%        \phl{\cpres x{\query A}y{\bang A}(\client xuQ \pp \srv yvP)}
%        &\reducesto&
%        \phl{\cpres u{A}v{\dual A}(P \pp Q)}
%      \\
%      % (\beta_{!W}) &
%        \phl{\cpres x{\query A}y{\bang A}(P \pp \srv yvQ)}
%        &\reducesto&
%        \phl{P}
%      \\
%      % (\beta_{!C}) &
%        \phl{\cpres x{\query A}y{\bang A}(P \substtwo x{x'}x{x''} \pp \srv yvQ)}
%        &\reducesto&
%      % \\ \multicolumn{3}{r}{
%        \phl{\cpres {x'}{\query A}{y'}{\bang A}
%         ((\cpres {x''}{\query A}{y''}{\bang A}
%          (P \pp \srv {y'}vQ)) \pp \srv{y''}vQ)}
%      % }
%      \\
%      % (\beta_{\exists\forall}) &
%        \phl{\cpres x{\exists X.B}y{\forall X.\dual B}(\sendtype xA{P\pp \recvtype yXQ})}
%        &\reducesto&
%        \phl{\cpres x{B \substone AX}y{B \substone AX}(P \pp Q \substone AX)}
%  \end{equations}
%
%

\[
\infer[cut]{
	\phl{\cpres{a}{A\tensor C}{a'}{}{(\send axPQ \pp \recv {a'}{x'}{P'})}}
	\seq
	\{[\phl{x_i}:\thl{C_i}]\phl{b_i}:\thl{B_i}\}_{i\le n},  \Gamma, \Gamma'
}{
	\infer[\tensor]{
		\phl{\send axPQ} 
		\seq 
		\{[\phl{x_i}:\thl{C_i}]\phl{b_i}:\thl{B_i}\}_{i\le n},\phl a:\thl{C \tensor A}, \Gamma
	}{
		\phl P 
		\seq 
		\{\phl{x_i}:\thl{C_i}\}_{i\le n}, \phl x:\thl C
		& 
		\phl Q 
		\seq 
		\{\phl{b_i}:\thl{B_i}\}_{i\le n}, \phl a: \thl A, \Gamma
	}
	&
	\infer[\parr]{
		\phl{\recv {a'}{x'}{P'}} 
		\seq 
		\phl {a'}: \thl {C^\perp \parr A^\perp}, \Gamma'
	}{
		\phl{P'}
		\seq 
		[\phl {x'}:\thl {C^\perp}]\phl {a'}:\thl {A^\perp}, \Gamma'
	}
}
\]
\[
\leadsto\quad
\infer[cut_2]{
	\phl{??}
	\seq
	\{[\phl{x_i}:\thl{C_i}]\phl{b_i}:\thl{B_i}\}_{i\le n}, \Gamma, \Gamma'
}{
	\phl{Q}
	\seq 
	\{\phl{b_i}:\thl{B_i}\}_{i\le n}, \phl a: \thl A, \Gamma
	&
	\infer[cut_1]{
		\phl{??}
		\seq
		[\boxdot\{\phl{x_i}:\thl{C_i}\}_{i\le n}]\phl{a'}:\thl{A^\perp}, \Gamma'
	}{
		\phl {P}
		\seq 
		\{\phl{x_i}:\thl{C_i}\}_{i\le n}, \phl x:\thl C
		&
		\phl {P'}
		\seq 
		[\phl {x'}:\thl C^\perp]\phl {a'}:\thl {A^\perp}, \Gamma'
	}
}
\]		

\[
\infer[cut]{
	\phl{\cpres{x}{A\oplus B}{x'}{}{({\inl xP} \pp \Case xPQ)}}
	\seq
	\Gamma_1, [\Left]\phl{y}:\thl{C}, \Gamma_2
	}{
	\infer[\oplus_1]{
		\phl{\inl xP}
		\seq
		\Gamma_1,  [\Left]\phl{y}:\thl{C}, \phl{x}:\thl{A\oplus B}
		}{
		\phl P
		\seq
		\Gamma_1, \phl{y}:\thl{C}, \phl{x}:\thl{A}
		}
	&
	\infer[\with]{
		\phl{\Case {x'}{P'}{Q'}}
		\seq
		\Gamma_2, \phl{x'}:\thl{\dual A\with\dual B}
		}{
		\phl{P'}
		\seq
		\Gamma_2, [\Left]\phl{x'}:\thl{\dual A}
		&
		\phl{Q'}
		\seq
		\Gamma_2, [\Right]\phl{x'}:\thl{\dual B}
		}
	}
\]\[\leadsto\quad
\infer[cut_3]{
	\phl{??}
	\seq
	\Gamma_1, [\Left]\phl{y}:\thl{C}, \Gamma_2	
	}{
	\phl P
	\seq
	\Gamma_1, \phl{y}:\thl{C}, \phl{x}:\thl{A}
	&
	\phl{P'}
	\seq
	\Gamma_2, [\Left]\phl{x'}:\thl{\dual A}
	}
\]

\[
\infer[cut]{
	\phl{\cpres{x}{\one}{x'}{}{({\close x} \pp  {\wait xP} )}}
	\seq
	\Gamma
	}{
	\infer[\one]{
	\syncseq{\close x} 
	{\pairQ{x}{\one}}
	}{}
	&
	\infer[\bot]
	{\syncseq {\wait xP} 
	{\Gamma, \pairQ{x}{\bot}}
	}{
	\syncseq {P} \Gamma}
}
\quad\leadsto\quad
{\syncseq {P} \Gamma}
\]

\[
\infer[cut]{
	\Gamma_1, ?\Gamma_2
	}{
	 \infer[?]{
	 	\syncseq {\client xyP}{\Gamma_1, \phl x:\thl{\query A}} 
	 	}{
	 	\syncseq {P}{\Gamma_1, \phl x: \thl A} 
	 	}
	 &
	 \infer[!]{
	 	\syncseq {\srv xyP'}{\query \Gamma_2, \phl x:\thl{\bang A} } 
	 	}{
	 	\syncseq {P'}{\query \Gamma_2, \phl y: \thl A} 
		 }
	}
\quad\leadsto\quad
\infer[cut]{\Gamma_1, ?\Gamma_2}{
	\syncseq {P}{\Gamma_1, \phl x: \thl A} 
	&
	\syncseq {P'}{\query \Gamma_2, \phl y: \thl A} 
	}
\]

\paragraph{Extra (admissible?) rules}

\[\fbox{$
	\infer[cut_1]{
		\phl{}
		\seq
		[\boxdot\{\phl{x_i}:\thl{C_i}\}_{i\le n}]\phl{b}:\thl{B}, \Gamma
	}{
		\phl {} 
		\seq 
		\{\phl{x_i}:\thl{C_i}\}_{i \le n}, \phl x:\thl {C}
		&
		\phl {}
		\seq 
		[\phl {x'}:\thl {C^\perp}]\phl {b}:\thl {B}, \Gamma
	}
	$}\]

$\boxdot$ indicates that all the formulas in that multiset need to  be processed at the same time, like a compression of many inputs into one. \sonia{or maybe a time stamp or something like that}

\[\fbox{$
	\infer[cut_2]{
		\phl{}
		\seq
		\{[\phl{x_i}:\thl{C_i}]\phl{b_i}:\thl{B_i}\}_{i\le n}, \Gamma, \Gamma'
	}{
		\phl{}
		\seq 
		\{\phl{b_i}:\thl{B_i}\}_{i\le n}, \phl a: \thl A, \Gamma
		&
		\phl{}
		\seq
		[\boxdot\{\phl{x_i}:\thl{C_i}\}_{i\le n}]\phl{a'}:\thl{A^\perp}, \Gamma'
	}
	$}\]

\[
\fbox{$
	\infer[cut_{3\Left}]{
		\phl{}
		\seq
		\Gamma_1, [\Left]\phl{y}:\thl{C}, \Gamma_2	
	}{
		\phl{}
		\seq
		\Gamma_1, \phl{y}:\thl{C}, \phl{x}:\thl{A}
		&
		\phl{}
		\seq
		\Gamma_2, [\Left]\phl{x'}:\thl{\dual A}
	}
\qquad
	\infer[cut_{3\Right}]{
		\phl{}
		\seq
		\Gamma_1, [\Right]\phl{y}:\thl{C}, \Gamma_2	
	}{
		\phl{}
		\seq
		\Gamma_1, \phl{y}:\thl{C}, \phl{x}:\thl{A}
		&
		\phl{}
		\seq
		\Gamma_2, [\Right]\phl{x'}:\thl{\dual A}
	}
$}
\]

\sonia{$cut_2$ and $cut_3$ are similar and could probably be reformulated as the same. They generalise the basic $cut$}

\paragraph{Admissibility of $cut_1$?}

\[
\infer[cut_1]{
	\phl{}
	\seq
	[\boxdot\{\phl{x_i}:\thl{C_i}\}_{i\le n}]\phl{b}:\thl{B}, \{[\phl{y_i}:\thl{F_i}]\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d:\thl{F \tensor D}, \Gamma'
}{
	\phl {} 
	\seq 
	\{\phl{x_i}:\thl{C_i}\}_{i \le n}, \phl x:\thl {C}
	&
	\infer[\tensor]{
		\phl {}
		\seq 
		[\phl {x'}:\thl {C^\perp}]\phl {b}:\thl {B}, 	\{[\phl{y_i}:\thl{F_i}]\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d:\thl{F \tensor D}, \Gamma'
	}{
		\phl {}
		\seq 
		\phl {x'}:\thl {C^\perp}, \{\phl{y_i}:\thl{F_i}\}_{i\le m}, \phl y:\thl F
		& 
		\phl {} 
		\seq 
		\phl {b}:\thl {B}, \{\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d: \thl D, \Gamma'
	}
}
\]
\[
\qquad\leadsto\qquad
\infer[\tensor_c]{
	\seq 
	[\boxdot\{\phl{x_i}:\thl{C_i}\}_{i\le n}]\phl{b}:\thl{B}, \{[\phl{y_i}:\thl{F_i}]\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d:\thl{F \tensor D}, \Gamma'
}{
	\infer[cut]{
		\seq
		\{\phl{x_i}:\thl{C_i}\}_{i \le n}, \{\phl{y_i}:\thl{F_i}\}_{i\le m}, \phl y:\thl F
	}{
		\seq
		\{\phl{x_i}:\thl{C_i}\}_{i \le n}, \phl x:\thl {C}
		&
		\phl {}
		\seq 
		\phl {x'}:\thl {C^\perp}, \{\phl{y_i}:\thl{F_i}\}_{i\le m}, \phl y:\thl F
	}
	& 
	\seq 
	\phl {b}:\thl {B}, \{\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d: \thl D, \Gamma'
}
\]

\sonia{one potential problem here is that we forget in the $cut$ that the $C_i$s came all from one source. That is, $\tensor_c$ is agnostic wrt to what to compress into channel $b$ and there could be errors. It can only be enforced at the term level.}

\paragraph{Admissibility of $cut_2$?}

\[
\infer[cut_2]{
	\phl{}
	\seq
	\{[\phl{x_i}:\thl{C_i}]\phl{b_i}:\thl{B_i}\}_{i\le n}, \Gamma, \{[\phl{y_i}:\thl{F_i}]\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d:\thl{F \tensor D}, \Gamma'
}{
	\phl{}
	\seq 
	\{\phl{b_i}:\thl{B_i}\}_{i\le n}, \phl a: \thl A, \Gamma
	&
	\infer[\tensor_c]{
		\seq 
		[\boxdot\{\phl{x_i}:\thl{C_i}\}_{i\le n}]\phl{a'}:\thl{\dual{A}}, \{[\phl{y_i}:\thl{F_i}]\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d:\thl{F \tensor D}, \Gamma'
	}{
		\seq
		\{\phl{x_i}:\thl{C_i}\}_{i \le n}, \{\phl{y_i}:\thl{F_i}\}_{i\le m}, \phl y:\thl F
		& 
		\seq 
		\phl {a'}:\thl {\dual{A}}, \{\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d: \thl D, \Gamma'
	}
}
\]
\[
\qquad\leadsto\qquad
\infer[\tensor]{
	\phl{}
	\seq
	\{[\phl{x_i}:\thl{C_i}]\phl{b_i}:\thl{B_i}\}_{i\le n}, \Gamma, \{[\phl{y_i}:\thl{F_i}]\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d:\thl{F \tensor D}, \Gamma'
	}{
	\seq
	\{\phl{x_i}:\thl{C_i}\}_{i \le n}, \{\phl{y_i}:\thl{F_i}\}_{i\le m}, \phl y:\thl F
	&
	\infer[cut]{
		\seq
		\{\phl{b_i}:\thl{B_i}\}_{i\le n}, \Gamma, \{\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d: \thl D, \Gamma'
		}{
		\phl{}
		\seq 
		\{\phl{b_i}:\thl{B_i}\}_{i\le n}, \phl a: \thl A, \Gamma
		&
		\seq 
		\phl {a'}:\thl {\dual{A}}, \{\phl{d_i}:\thl{D_i}\}_{i\le m}, \phl d: \thl D, \Gamma'
		}
	}
\]

\paragraph{Admissibility of $cut_3$?}

\[
\infer[cut_{3\Right}]{
	\phl{}
	\seq
	\Gamma_1, [\Right]\phl{y}:\thl{C}, \Gamma_2, \phl{y'}:\thl{B \oplus D}
}{
	\phl{}
	\seq
	\Gamma_1, \phl{y}:\thl{C}, \phl{x}:\thl{A}
	&
	\infer[\oplus_2]{
	\phl{}
	\seq
	\Gamma_2, \phl{y'}:\thl{B \oplus D}, [\Right]\phl{x'}:\thl{\dual A}
	}{
	\phl{}
	\seq
	\Gamma_2, \phl{y'}:\thl{D}, \phl{x'}:\thl{\dual A}
	}
}
\quad\leadsto\quad
\infer[\oplus_2]{
	\phl{}
	\seq
	\Gamma_1, [\Right]\phl{y}:\thl{C}, \Gamma_2, \phl{y'}:\thl{B \oplus D}
	}{
	\infer[cut]{
		\phl{}
		\seq
		\Gamma_1, \phl{y}:\thl{C}, \Gamma_2, \phl{y'}:\thl{D}
		}{
		\phl{}
		\seq
		\Gamma_1, \phl{y}:\thl{C}, \phl{x}:\thl{A}
		&
		\phl{}
		\seq
		\Gamma_2, \phl{y'}:\thl{D}, \phl{x'}:\thl{\dual A}
		}
	}
\]



==> core_system.tex <==
\section{Core Forwarders}\label{sec:core_system}

Our goal is to study forwarders in the context of linear
logic. Hereby, we introduce {\em core forwarders}, a class of
forwarder processes that characterises all those forwarders that are
typable in CLL according to the proposition-as-session approach
by~\cite{W12}.
% 
Core forwarders are such that received messages cannot be altered by
the forwarder, they can only be passed on (no data processing).
%
They also enforce no message creations, and no message loss.
%
In general, core forwarders are allowed to receive and
forward messages in any order, in particular independently of the
order they receive them in.
%
We will show that they characterise the set of forwarders that are
typable in linear logic.

\subsection{Judgements and Rules}

\paragraph{Syntactical categories.}  Following the propositions as
sessions approach~\cite{CPT16,W14}, {\em types}, taken to be
propositions (formulas) of classical % (propositional)
linear logic, are associated to names, denoting the way a name must be
used at runtime. Their formal syntax is given as:
%
\begin{align*}
  \thl{A,B,C,D} \Coloneqq & \quad
                            \thl{a}
                            \mid \thl{1}
                            \mid\thl{\bot}
                            \mid \thl{A\tensor B}
                            \mid \thl{A\parr B}
                            \mid \thl{A\oplus B}
                            \mid \thl{A\with B}
                            % \mid \thl{0}
                            % \mid \thl{\top}
                            % \thl{A^\perp} \mid
                            \mid\thl{!A}
                            \mid\thl{?A} 
\end{align*}
We briefly comment on their interpretation. Type $a$ is an element
from $\mathcal A\cup\mathcal A^\perp$ where $\mathcal A$ is a set of
atoms and $\dual{\mathcal A}$ is the dual of $\mathcal A$, obtained
from the operator $^\perp$ on $\mathcal A$. Types $\one$ and $\perp$
denote an endpoint that must be closed by a last synchronisation. A
type $A \tensor B$ is assigned to an endpoint that outputs something
of type $A$ and then is used as $B$. Similarly, an endpoint of type
$A\parr B$, receives something of type $A$ and then continues as
$B$. Types $A\oplus B$ and $A\with B$ denote branching. The former is
the type of an endpoint that may select to go left or right and
continues as $A$ or $B$, respectively. The latter is the type of an
endpoint that offers two choices (left or right) and then, based on
such choice, continues as $A$ or $B$. Finally, $!A$ types an endpoint
offering a service of type $A$ while $?A$ types an endpoint of a
client invoking some service and behaving as $A$. Operators can be
grouped in pairs of duals that reflect the input-output duality. As a
consequence, standard duality $^\perp$ on types is defined as:\quad
% \begin{displaymath}
$
  \dual{(\dual{a})} = a
  \qquad \dual\one=\perp
  \quad \dual{(A\tensor B)} = \dual A\parr\dual B
  \qquad \dual {(A\oplus B)}=\dual A\with\dual B
  \qquad \dual{(!A)} = ?\dual A
  $.
% \end{displaymath}
% \todo{where does
%   $a$ come from?}  \sonia{we are giiven some type variables
%   $X,Y,Z...$} \todo{define formally the dual $\thl{A^\perp}$ by De
%   Morgan laws? }

  \emph{Basic contexts} are sets $\Delta$ of propositions labelled by
  endpoints, such that each endpoint occurs at most once in
  $\Delta$.\footnote{ Sometimes, we use $\query\Delta$ as shorthand
    for
  % a context of the form
  $\phl{x_1}:\thl{\query A_1}, \ldots, \phl{x_n}:\thl{\query A_n}$
  and % , in this case,
  use $\Delta$ % (without $\query$) % will
                                                         % specifically
                                                         % denote
  for the corresponding set
  $\phl{x_1}:\thl{A_1}, \ldots, \phl{x_n}:\thl{A_n}$.  }
%
Formally, 
% \begin{align*}
$ \Delta \Coloneqq \cdot\ \mid\ \Delta, \pairQ xA $,
% \end{align*}
where $\pairQ xA$ expresses that endpoint $\phl x$ has type $A$.

During the forwarding process, contexts may evolve into
\emph{generalised contexts}, denoted by $\Gamma$.
%
Their purpose is to model messages in transit, in the process of being
forwarded, that have been received but cannot be
further decomposed before being sent.
%
Generalised contexts are given by:
%
\begin{align*}
{\Gamma} \Coloneqq &  \quad
\Delta\mid
\Gamma, \Star \mid
\Gamma, \br{\phl x:\thl A} \mid
\Gamma, \Left \mid
\Gamma, \Right \mid
%\Gamma, {\Left} \mid
%\Gamma, {\Right} \mid
\Gamma, \Query%\dbr{\query\Delta}
\end{align*}

A \emph{core forwarder} can receive and send messages. % of type
% $\thl{A}$.  When such messages are in transit, they appear in the
% context as $\br{\phl x:\thl A}$. Or, it can receive and send
% synchronisations, branching or server request messages.
Since core forwarders are forwarders, we adopt a similar technique to
that of Figure~\ref{fig:inference}. $\Star$ indicates that a request
for synchronisation request needs to be forwarded.  Messages received
need to be stored until sent so that no further computation can be
executed on them; indicated by encapsulating them into a box
$\br{\phl{x}:A}$.\footnote{ We will slightly abuse the notation and
  write $[\Delta]$ for the set of boxed propositions
  $\{[\phl{x_i}:\thl{A_i}]\}_i$ when
  $\Delta = \{\phl{x_i}:\thl{A_i}\}_i$.
%and we also use implicitely the equivalence $[\cdot] = \cdot$ for an empty context.
} 
%
In the case of a choice, the forwarder communicates just the
information on which branch to make the selection, denoted by the
presence of tokens $\Left$ and $\Right$, indicating respectively a
left or a right selection. %\footnote{ We can write only $\Select$ if
%  knowing the index is not necessary.  }
%
In the case of exponentials, forwarders connect to
processes with non-linear, potentially replicated, server/client behaviours, even though
forwarders themselves are  linear by design. Connection requests are  forwarded
using token $\Query$.
%
% \todo{rephrase following}
% This sort of interaction can lead to the storing of whole sets of
% propositions $\query\Delta$ within a \emph{query} double box written
% as $\Query\dbr{\query\Delta}$, but only if they all start with
% exponentials.\footnote{ We use implicitely the equivalence:
%   $\Query\dbr{\cdot} \equiv \cdot$.  }

% In the sequel, single boxes such as $\Star$ are used for
% \emph{gathering-like} communications, while double boxes such as
% $\Query\dbr{\query\Delta}$ are used in \emph{broadcasting-like}
% communications (this will become clearer when we discuss the typing
% rules).


\paragraph{Judgements.}
%
The {judgement} describing that a process $\phl{P}$ is a well-typed
\emph{core forwarder}, is written as $\coreseq P \Delta$ where $\thl{\Delta}$ is
defined as before.
%
$\phl{P}$ orchestrates the forwarding of messages between the
different processes captured in $ \thl{\Delta}$.
%
Judgements of the more general form $\coreseq P \Gamma$ are also
valid, but include processes that are in the midst of forwarding
information.

\paragraph{Rules.}  In~Figure~\ref{fig:core}, we report the rules for
typing processes: they correspond to the classical linear logic
sequent calculus (hence those of CP~\cite{W14}) with some extra
restrictions for characterising forwarders, that reflect the system in
Figure~\ref{fig:inference}.
%
\begin{figure}
  %	\small
  \[
    \begin{array}{c}
      \infer[\textsc{Ax}]{
      \coreseq 
      { \cpaxiom {x}{A^\perp}{y}{A}}
      { \pairQ{x}{\dual{A}}, \pairQ{y}{A}}
      }{ }
      \qquad
      \infer[\bot]
      {\coreseq {\wait xP} {\Gamma, \pairQ{x}{\bot}}}
      {\coreseq {P} {\Gamma, \Star}}
      \qquad
      \infer[\one]{%\;(n\ge 1)]{
      \coreseq{\close x} {\pairQ{x}{\one}, \Star}}{ } %^n
      \\[2ex]
      \infer[\parr]{
      \coreseq{\recv xyP} {\Gamma, \phl x: \thl{A \parr B}}
      }{
      \coreseq P {\Gamma, \br{\phl y: \thl A}, \phl x: \thl{B}}
      }     
      \qquad
      \infer[\tensor]{
      \coreseq{\send xyPQ} 
      {\Gamma, \br{\Delta}, \phl x:\thl{A \tensor B}}
      }{
      \coreseq P {\Delta, \pairQ yA}
      & \coreseq Q {\Gamma, \pairQ xB }
        \qquad \fn(\Delta)\cap \fn(\Gamma) = \emptyset
	}
      \\[2ex]
      \infer[\with]%\;{(n,m\ge 1)}]
      {\coreseq{\Case xPQ} {\Gamma, \pairQ x{A \with B}}
      }{
      \coreseq P {\Gamma, \Left, \pairQ x{A}} %^n
      &
        \coreseq Q {\Gamma,  \Right, \pairQ x{B}} %^m
	}
	\qquad
	\infer[\oplus_\#\;(\#\in\{l,r\})]
	{\coreseq {\inlr xP} {\Gamma, \Select[\#], \pairQ{x}{A_l \oplus A_r}}}
	{\coreseq P {\Gamma, \pairQ{x}{A_\#}}}
%	\\[2ex]
%	\infer[\oplus_l]
%	{\coreseq {\inl xP} {\Gamma, \Left, \pairQ{x}{A \oplus B}}}
%	{\coreseq P {\Gamma, \pairQ{x}{A}}}
%	\qquad
%	\infer[\oplus_r]
%	{\coreseq {\inr xP} {\Gamma, \Right, \pairQ{x}{A \oplus B}}}
%	{\coreseq P {\Gamma, \pairQ{x}{B}}}
	\\[2ex]
	\infer[!]{
		\coreseq {\srv xyP}{\query\Delta, \phl x:\thl{\bang A} } 
	}{
		\coreseq {P}{\Query, \query\Delta, \phl y: \thl A}  %^n
	}
	\qquad
	\infer[?]{
		\coreseq {\client xyP}{\Gamma, \Query, \phl x:\thl{\query A}}
	}{
		\coreseq {P}{\Gamma, \phl y: \thl A} 
	}
    \end{array}
  \]
  \caption{Core forwarder logic}
  \label{fig:core}
\end{figure}
% 
% We comment on the difference with the standard session typing based on
% linear logic~\cite{CP10,W14}.
%
% Comment for RULE Ax
Rule \Did{Ax} is the axiom of CLL: it denotes a process that
interfaces two endpoints of dual type.
%
% Comment for unit rules
Rules $\one$ and $\perp$ type forwarding of empty messages. In
$\phl{\wait xP}$, the typing makes sure that after an empty message is
received (of type $\perp$), it must be forwarded by adding to the
typing context for $\phl P$ the object $\Star$ which will make sure
that eventually rule $\one$ is used. In fact, rule $\one$ is
applicable only if there is $\Star$ in the context, i.e., at least one
$\perp$ rule has been encountered before.
%
%Note that we use $\Star^n := \Star, \Star^{n-1}$
%for $n \ge 1$ with $\Star^0 = \cdot$.
%
% Comment for multiplicative rules
Rule $\parr$ types reception of $\phl y$ over $\phl x$ with type
$A\parr B$. The received name of type $A$ cannot be used but must be
forwarded, therefore it is wrapped as $\br{\pairQ yA}$ for the typing
of $\phl P$. This is done by rule $\tensor$, which collects the
received $\br{\Delta}$ and spawns a new forwarder $\phl P$ of type
$\Delta,\pairQ yA$. Note that, since contexts are sets, we explicitly
require $\fn(\Delta)$ and $\fn(\Gamma)$ to be different.
%
% Comment for additive rules
Rules $\oplus_1$, $\oplus_2$ and $\with$ type branching
processes. Unlike the case of units and multiplicatives which use a
gathering communication mechanism (many-to-one), additives (and later
exponentials) use broadcasting (one-to-many). This is a choice that
follows directly from the logic principles and the way each operator
are interpreted. Rule $\with$ types the process $\phl{\Case xPQ}$: in
branches $\phl P$ and $\phl Q$ the selected choice, left and right
respectively, must be forwarded to some other endpoint. This is
enforced by adding the flags $\Left$ and $\Right$ to the context of
the premises. Then, rules $\oplus_1$ and $\oplus_2$, which type output
selections, will require $\Left$ and $\Right$ to be present in the
context, respectively.
%
% Note that, as in the case for units,
% $\Select^{n} = \Select, \Select^{n-1}$ for $n \ge 1$ with
% $\Select^{0} = \cdot$.
%
% Comment for exponential rules
Rules for exponentials work similarly to additives. Note that
forwarders do not have weakening and contraction since they do only
forward messages.



% In the tensor case, we anticipate the forwarding of $\thl A$ from
% $\thl {\Delta}$, which, by construction consists only of forwarded
% messages.
% %
% Conversely, the $\parr$-rule boxes the receiving of a message of the
% type $\thl A$.
% %
% Analogously, the rules $\oplus_1$ and $\oplus_2$ de-box which branch
% should be taken, whereas the $\with$ baxes the choice in each branch,
% accordingly.


\begin{example} \label{ex:2b}
  It is straightforward to show that the 2-buyer forwarders from
  Example~\ref{ex:2buyer} can be typed as a core forwarder by proving
  the judgement
  \[
    \coreseq {\phl P_1}{
      \begin{array}[t]{l}
        % 
        \pairQ{b_1}{\tname^\perp \parr \tcost \tensor \tcost^\perp \parr\perp},\quad
        % 
        \pairQ{b_2}{\tcost \tensor \tcost \tensor ((\taddr^\perp
        \parr \perp) \with \perp)},\\
      % 
        \pairQ{s}{\tname \tensor \tcost^\perp \parr \tcost^\perp \parr
        ((\taddr \tensor \one) \oplus \one)}
      \end{array}
      % 
    }
    %
  \]
    \[
    \coreseq {\phl P_2}{
      \begin{array}[t]{l}
        % 
        \pairQ{c_1}{\tcost \parr ((\taddr^\perp \parr \perp) \with \perp)}, \quad
        % 
        \pairQ{c_2}{\tcost \parr ((\taddr^\perp \parr \perp) \with \perp)},\\
      % 
        \pairQ{b_2'}{\tcost^\perp \parr \tcost^\perp \parr  
        ((\taddr \tensor \one) \oplus \one)}
      \end{array}
      % c
    }
    %
  \]
  where $\tname$, $\tcost$, and $\taddr$ are atomic types. \qed
\end{example}


\begin{example}\label{ex:new}

Moreover, we observe that the typing system in Figure~\ref{fig:core} is not
enforcing any order preservation of messages.
  The process
  $\recv xy{}
    \recv xz{}
    \send w s {\fwd zs}{}
    \send w t {\fwd ty}{}
    \fwd xw$
   is indeed a core forwarder, despite the fact that when forwarding
  from $x$ to $w$, the order of messages is inverted.  \qed
\end{example}

In the next section, we will see a new system that preserves the order
in which messages are received in which such process is not admitted.


\subsection{Properties of Core Forwarders}
In this subsection, we show two results: a) core forwarder proofs can
be transformed into CLL proofs; and, b) a process is typable in CLL
and is a forwarder if and only if it is a core forwarder.

We write $\enc{\cdot}$ to map core forwarder typing contexts into
simple CLL ones simply by erasing the extra conditions in the rules
defining $\coreseq{}{}$: 
\begin{align*}
  \enc{\Delta}\coloneqq \Delta
  \qquad
  \enc{\Gamma, \Star}\coloneqq \enc{\Gamma}
  \qquad
  \enc{\Gamma, \br{\phl x:\thl A}}\coloneqq  \enc{\Gamma}, \phl x:\thl
  A
  \qquad
  \enc{\Gamma, \Symbol}\coloneqq  \enc{\Gamma}
\end{align*}
%
where $\Symbol\in\{\Star,\Left,\Right,\Query\}$.  It is then immediate
to show that any proof in our system is also a proof in CLL, whose
judgment are denoted by the turnstyle $\vdash_{\text{CLL}^-}$.
%
Hereby, we adopt a subset of CLL (and corresponding terms)~\cite{W12}
without polymorphic types, weakening and contraction.  Adding
polymorphic rules to the systems presented in this paper is
straightforward. However, we leave weakening and contraction out since
we believe that they interfere with our intuition of forwarders. This
will become clearer in \S~\ref{sec:coherence}. For a complete set of
CLL$ ^-$ (just CLL from now on) rules, see Appendix~\ref{app:cll}.
%
\begin{proposition}\label{prop:coretoLL}
  If $\coreseq P {\thl\Gamma}$, then
  $\phl P \seq_{\text{CLL}^-}\thl{\enc{\Gamma}}$.
\end{proposition}

Proposition~\ref{prop:coretoLL} shows that any core forwarder
corresponds to a CLL proof. But, even more, if we consider all those
processes that are forwarders and are also typable in CLL then we get
exactly core forwarders. In the sequel, we define the partial operator
$\f{}{}$ as:
% \alert{define $\Symbols$ this is not very readable.}
\begin{displaymath}
  \begin{array}{c}
    \f{\Sigma, \phl x}{\Delta, \pairQ xA}
    \ =\
    (\f \Sigma\Delta), \pairQ xA
    \qquad
    \f{\Sigma, [\phl x]} {\Delta, \pairQ xA}
    \ =\
    (\f \Sigma\Delta), \br{\pairQ xA}
    \\[1mm]
    \f{\Sigma, \Symbol} {\Delta}
    = (\f\Sigma \Delta), \Symbol
    \quad\mbox{for}\quad\Symbol\in\{\Star,\Left,\Right,\Query\}
  \end{array}
\end{displaymath}
%
We can then state the following
%
\begin{theorem}\label{thm:fwdcharacterisation}
  $\cllseq {\phl P} \Delta$ and $\genseq\Sigma P$
%
  if and only if
%
  $\coreseq P{\f\Sigma\Delta}$
%
  such that $fv(\Delta) = fv(\Sigma)$. 
%
\end{theorem}

\begin{proof}(Sketch)
  We consider both directions separately. Core forwarders are
  obviously forwarders. This follows immediately from the structure of
  proofs in our system which straightforwardly satisfy the definition
  of forwarder and Proposition~\ref{prop:coretoLL}. 
  
  The opposite direction is harder to prove. We need to show that given a linear
  logic proof of a process that is also a forwarder we can construct a
  proof that types a core forwarder. This can be done by induction on
  the structure of $P$. The full proof can be found
  in~Appendix~\ref{app:fwdcharacterisation}.
\end{proof}

\subsection{Composition of Core Forwarders and their Semantics}
% 
\noindent
Next, we turn to the formal semantics of forwarders. In a
propositions-as-session approach, the semantics of a language is
derived by reducing processes interpreted as proofs by the process of
cut-elimination. The two \textsc{Cut}-rules defined below give
compositionality of processes in the sense of forwarder
compositionality mentioned before, where every cut-reduction step
evolves forwarders operationally. The result is a Curry-Howard
correspondence between forwarders and proofs.
%
In order to achieve that, we must have a notion for composing
forwarders (and proofs) which, in our formal syntax from
\S~\ref{sec:calculus}, is given by the term $\phl{(\nu xy)(P\pp
  Q)}$. Logically, this is interpreted as $\Did{Cut}$ rule, and, as a
consequence, the semantics is derived by the cut elimination process.
%
% We will now define the semantics of our forwarder processe; it will be
% based on proof transformations in the core forwarder logic.
%
Our starting point is the most simple cut rule from CLL (in this paper
we adopt endpoints as done by~\cite{CLMSW16}), which
% represents the parallel composition of two processes: it
connects endpoints $\phl x $ and $\phl {y}$ and joins together the
remainders of $\thl {\Delta_1}$ and $\thl {\Delta_2}$:
\[\small
\infer[\textsc{Cut}]{
	 \coreseq{\cpres{x}A{y}{A^\perp}(P \pp P')}{\Delta_1,\Delta_2}
}{
	\coreseq{P}{\Delta_1, \phl{x}:\thl{A}}
	&
	\coreseq{P'}{\Delta_2, \phl {y}:\thl{A^\perp}}
}    
\]
%
However, since core forwarders have more complex contexts than CLL,
the rule above should be able to deal with any context $\Gamma$ rather
than just $\Delta$.
%
For example, we can have the transformation
\begin{equation}\label{eq:cc_core}\small
  \infer[\textsc{Cut}]{
    \coreseq{\cpres{x}A{x'}{A^\perp}(\recv yzP \pp P')}{\Delta_1,\phl{y}:\thl{B\parr C},\Delta_2}
  }{
    \infer[\parr]{
      \coreseq{\recv yzP} {\Delta_1, \phl{x}:\thl{A},\phl{y}:\thl{B\parr C}}
    }{
      \coreseq P {\Delta_1, \phl{x}:\thl{A}, \br{\phl z: \thl B}, \phl y: \thl{C}}
    }   
    &
    \coreseq{P'}{\Delta_2, \phl {x'}:\thl{A^\perp}}
  }
  \reducesto_\kappa
  % \]
  % into the equivalent we will want to evolve this process into the
  % following equivalent one:
  % \[\small
  \infer[\parr]{ \coreseq{\recv yz\ \cpres{x}A{x'}{A^\perp}(P \pp P')}
    {\Delta_1, \phl{y}:\thl{B\parr C},\Delta_2} }{
    \infer[\textsc{Cut}]{ \coreseq{\cpres{x}A{x'}{A^\perp}(P \pp
        P')}{\Delta_1,\br{\phl z: \thl B}, \phl y: \thl{C},\Delta_2}
    }{ \coreseq P {\Delta_1, \phl{x}:\thl{A}, \br{\phl z: \thl B},
        \phl y: \thl{C}} & \coreseq{P'}{\Delta_2, \phl
        {x'}:\thl{A^\perp}} } }
\end{equation}
%
yielding
$\phl{\cpres{x}A{x'}{A^\perp}(\recv yzP \pp P')} \reducesto_\kappa
\phl{\recv yz\ \cpres{x}A{x'}{A^\perp}(P \pp
  P')}$~\footnote{As a consequence of handling the semantics of
  processes as proof transformations from CLL, it is well-known that
  we can always permute an unrelated input with a parallel
  composition~\cite{W14}.}.  This prompts us ultimately to allow cuts
to apply in generalised contexts as well, that is:
\[\small
\infer[\textsc{Cut}]{
	\coreseq {\cpres{x}A{x'}{A^\perp}(P \pp P')} {\Gamma_1,\Gamma_2}
}{
	\coreseq{P}{\Gamma_1, \pairQ{x}{A}}
	&
	\coreseq {P'} {\Gamma_2, \phl {x'}: \thl{A^\perp}}
}    
\]

Moreover, extra constraints on contexts require special cut rules that
deal with intermediary computation (referred to as ``runtime'' rules)
and associated to new syntactic terms (``runtime syntax''), depending
on the proposition that is being cut (and the corresponding
communication operation).
%
% Once the cut is generalised as such, we can also be in a case where
% the formula being cut is the one that is being processed just above it
% (aka.~\emph{key cases}).
%
This triggers four possible cases corresponding to units,
multiplicatives, additives and exponentials.
%
In the case of multiplicatives, we are required to introduce another
version of the cut rule to deal with the boxes of our forwarder
logic. Below, we look at the four possible process reductions
corresponding to the four principal cut reductions for the forwarder
logic. Later, we will show that rule \Did{Cut} and all other
introduced rules are admissible for core forwarders, i.e., we can
always create a forwarder that has no parallel composition and it
behaves as the composition of the two original forwarders. Such result
is based on proof transformations called {\em cut reductions}, which
will define the semantics of core forwarders.
%

\smallbreak
\paragraph{Units.} In the case of units, we have the reduction
\[\small
  \infer[\textsc{Cut}]{
    \coreseq {\cpres{x}A{x'}{A^\perp}(\close x \pp \wait {x'}{P'})} {\Star,\Gamma}
  }{
    \infer[\one]{ %%\;(n\ge 1)
      \coreseq{\close x} {\pairQ{x}{\one}, \Star}
    }{}
    &
    \infer[\bot]
    {\coreseq {\wait {x'}{P'}} {\pairQ{x}{\bot}, \Gamma}}
    {\coreseq {P'} {\Star, \Gamma}}
  }
  \qquad\longrightarrow\qquad
%  \infer=[\equiv_\Star\;(n\ge 1)]{
%    \coreseq {P'} {\Star,\Gamma}
%  }{
%    \coreseq {P'} {\Star, \Gamma}
%  }
	\deduce[]{
		\coreseq {P'} {\Star,\Gamma}
	}{}
\]
This communication needs to simply continue as $\phl{P'}$ (this is
identical to that of CLL).
%for which we use the special rule $\equiv_\Star$. 
%The latter is trivially
%admissible since rule $\one$ allows for an arbitrary number of
%$\Star$'s. Hence, by induction on the size of the proof we can
%always permute $\equiv_\Star$ with any rule above, until we reach
%$\one$.

\smallbreak 
\paragraph{Multiplicatives.} This case is more delicate since
there is an actual communication to implement.
\begin{displaymath}
  \small
  \begin{array}{l}
    % 
    \infer[\textsc{Cut}]{
    \coreseq {\cpres{x}A{x'}{A^\perp}(\send xyPQ \pp \recv {x'}{y'}{P'})} {\Gamma_1, [\Delta], \Gamma_2}
    }{
    \infer[\tensor]{
    \coreseq{\send xyPQ} 
    {\Gamma_1, [\Delta], \phl x:\thl{A \tensor B}}
    }{
    \coreseq P {\Delta, \pairQ yA}
    & 
      \coreseq Q {\Gamma_1, \pairQ xB }
      }
    &
      \infer[\parr]{
      \coreseq{\recv {x'}{y'}{P'}} {\Gamma_2, \phl {x'}: \thl{A^\perp \parr B^\perp}}
      }{
      \coreseq {P'} {\Gamma_2, [\phl {y'}: \thl {A^\perp}], \phl {x'}: \thl{B^\perp}}
      }    
      }
    \\[2ex]
    \qquad\qquad \reducesto
    \qquad
    \infer[\textsc{Cut}]{
    \coreseq {\cpres{x}A{x'}{A^\perp}(Q \pp \cpres{y}{}{\br{y'}}{}(P \pp P'))} {\Gamma_1, \Gamma_2, [\Delta]}
    }{
    \coreseq Q {\Gamma_1, \pairQ xB }
    &
      \infer[\textsc{Cut}_{\Box}]{
      \coreseq {\cpres{y}{}{\br{y'}}{}(P \pp P')} {\Gamma_2, [\Delta], \phl {x'}: \thl{B^\perp}}
      }{
      \coreseq P {\Delta, \pairQ yA}
    &
      \coreseq {P'} {\Gamma_2, [\phl {y'}: \thl {A^\perp}], \phl {x'}: \thl{B^\perp}}
      }
      }
  \end{array}
\end{displaymath}
%
This forces us to introduce another version of the cut to deal with
boxed propositions, called $\textsc{Cut}_{\Box}$, that allows us to
continue the computation between $\phl{P}$ and $\phl{P'}$ as expected:
it allows us to cut a proposition $A$ with a boxed proposition
$\br {A^\perp}$. 
%
Notice that this ``runtime'' rule has a special ``runtime'' term
associated to it, i.e., $\phl{\cpres{y}{}{\br{y'}}{}(P \pp P')}$.
%
% have no impact on the processes,
% \todo{change this!!}  e.g., $\Did{Cut}_{\Box}$ is regarded as a normal
% cut rule when it comes to processes.
%
Then, the new cut becomes again a normal cut when we finally forward
(for $\phl{x'} \in \fn(\phl{P'})$):
\begin{displaymath}\small
  \begin{array}{l}
    \infer[\textsc{Cut}_{\Box}]{
    \coreseq {\cpres{x}{}{\br{x'}}{}(P \pp \send uv{P'}{Q'})}
    {\Gamma, [\Delta_1], [\Delta_2] \phl {u}: \thl{B\tensor C}}
    }{
    \coreseq P {\Delta_1, \pairQ xA}
    &
      \infer[\tensor]{
      \coreseq {\send uv{P'}{Q'}} {\Gamma, [\phl {x'}: \thl {A^\perp}], [\Delta_2], \phl {u}: \thl{B\tensor C}}
      }{
      \coreseq {P'} {\phl {x'}: \thl {A^\perp}, \Delta_2, \phl v: \thl B}
    &
      \coreseq {Q'}{\Gamma, \phl u: \thl C}
      }
      }
    \\[2ex]
    \qquad\qquad\reducesto\quad
    \infer[\tensor]{
    \coreseq {\send uv{\cpres{x}{}{x'}{}
    (P \pp {P'})}{Q'}} {\Gamma, [\Delta_1], [\Delta_2], \phl {u}: \thl{B\tensor C}}
    }{
    \infer[\textsc{Cut}]{
    \coreseq  {\cpres{x}{}{x'}{}(P \pp{P'})} {\Delta_1, \Delta_2, \phl {v}: \thl{B}}
    }{
    \coreseq P {\Delta_1, \pairQ xA}
    &
      \coreseq {P'} {\phl {x'}: \thl {A^\perp}, \Delta_2, \phl v: \thl{B}}
      }
    &
      \coreseq {Q'}{\Gamma, \phl u: \thl C}
      }
  \end{array}
\end{displaymath}

\paragraph{Additives.} In the case of the additives, we have a behaviour
similar to that of units:
\begin{displaymath}\small
  \begin{array}{l}
    \infer[\textsc{Cut}]{
    	\coreseq 
    	{\cpres{x}{}{x'}{}({\inlr xP} \pp\Case {x'}{Q_l}{Q_r})} 
		{\Gamma_1,\Select[\#], \Gamma_2} 
		}{
    	\infer[\oplus_\#] {
    		\coreseq 
    		{\inlr xP} 
    		{\Gamma_1, \Select[\#],\pairQ{x}{A_l \oplus A_r}}
			}{
			\coreseq P 
			{\Gamma_1,\pairQ{x}{A_\#}} 
			}
    	& 
    	\infer[\with] {
    		\coreseq{\Case{x'}{Q_l}{Q_r}} 
    		{\Gamma_2, \pairQ {x'}{A_l^\perp \with A_r^\perp}}
      		}{ 
      		\coreseq {Q_l} 
      		{\Gamma_2, \Left, \pairQ{x'}{A_l^\perp}}
    		&
    	  	\coreseq {Q_r} 
      		{\Gamma_2, \Right, \pairQ {x'}{A_r^\perp}} 
      		} 
      	}
    \\[2ex]
    \qquad\qquad\longrightarrow\qquad 
%    \infer=[\equiv_{\Select}\;(n\ge1)]{
%    	\coreseq {\cpres{x}A{x'}{A^\perp}(P \pp P')} 
%    	{\Gamma_1, \Select[\#], \Gamma_2}
%    	}{ 
    	\infer[\textsc{Cut}]{
    		\coreseq {\cpres{x}{}{x'}{}(P \pp Q_\#)} 
    		{\Gamma_1, \Select[\#], \Gamma_2}
    		}{ 
    		\coreseq P {\Gamma_1, \pairQ{x}{A_\#}}
    		& 
    		\coreseq {Q_\#} {\Gamma_2, \Select[\#], \pairQ {x'}{A_\#^\perp}}
     	 	} 
%  		}
  \end{array}
\end{displaymath}
%
The standard \Did{Cut} does not need to be further generalised
or modified.
%but we will need to show that the rule establishing the
%structural equivalence of $\Select^n$ and $\Select$ is admissible.

\paragraph{Exponentials.} Finally, also for exponentials we have:
\[
\infer[\textsc{Cut}]{
	\coreseq {\cpres{x}A{x'}{A^\perp}(\client {x}{y}{P} \pp \srv {x'}{y'}{P'})} {\Gamma,\Query, \query\Delta}
}{
	\infer[?]
	{\coreseq {\client {x}{y}{P}} {\Gamma, \Query, \pairQ{x}{\query A}}}
	{
		\coreseq P {\Gamma, \pairQ{y}{A}}
	}
	&
	\infer[!]
	{\coreseq{\srv {x'}{y'}{P'}} {\query\Delta, \pairQ {x'}{\bang A^\perp}}
	}{
		\coreseq {P'} {\query\Delta, \Query, \pairQ {y'}{A^\perp}}
	}
}
\]
In this case as well, the cut-rule does not need to be further
generalised or modified.
%but we will need to show that the rule establishing the structural equivalence of $\Query^n$ and $\Query$ is admissible. 
\[
%\infer=[\equiv_{\Query}\;(n\ge 1)]{\Gamma,\Query, \query\Delta}{
	\infer[\textsc{Cut}]{
		\coreseq {\cpres{y}{}{y'}{}(P \pp P')} {\Gamma,\Query, \query\Delta}
	}{
		\coreseq P {\Gamma, \pairQ{y}{A}}
		&
		\coreseq {P'} {\query\Delta, \Query, \pairQ {y'}{A^\perp}}
	}
%}
\]



\begin{figure}
	\[
	\infer[\textsc{Cut}]{
		\coreseq {\cpres{x}A{x'}{A^\perp}(P \pp P')} {\Gamma_1,\Gamma_2}
	}{
		\coreseq{P}{\Gamma_1, \pairQ{x}{A}}
		&
		\coreseq {P'} {\Gamma_2, \phl {x'}: \thl{A^\perp}}
	}    
	\qquad
	\infer[\textsc{Cut}_{\Box} ]{
		\coreseq {\cpres{x}{}{\br{x'}}{}(P \pp P')} {\Gamma, [\Delta]}
	}{
		\coreseq P {\Delta, \pairQ xA}
		&
		\coreseq {P'} {\Gamma , [\phl {x'}: \thl {A^\perp}]}
	}
%	\\[2ex]
%	\infer[\textsc{Cut}_{\bang}]{
%		\coreseq {\cpres{x}A{x'}{A^\perp}(P \pp P')} {\Query\dbr{\query\Delta_1, \query\Delta_2}, \Gamma}
%	}{
%		\coreseq {P}{\query\Delta_1, \phl {x}:\thl{\bang A} } 
%		&
%		\coreseq {P'}{\Query\dbr{\phl {x}:\thl{\query A^\perp}, \query\Delta_2}, \Gamma}
%	}    
%	\\[10pt]\hline\\
%	\infer=[\equiv_{\Select}\;(n\ge 1)]{\coreseq {P} {\Gamma, \Select}}{
%		\coreseq {P} {\Gamma, \Select^n}}
%	\qquad
%	\infer=[\equiv_{\Star}\;(n\ge 1)]{\coreseq {P} {\Gamma, \Star}}{
%		\coreseq {P} {\Gamma, \Star^n}}
	\]	
	\caption{Forwarder Composition - Cut rules for core
          forwarders}
	\label{fig:cut0}
\end{figure}

\paragraph{Results and Semantics.}
The two generalised cut-rules are summarised in Figure~\ref{fig:cut0}.
%
Proving that the initial basic cut-rule is admissible requires to show
that both of these rules are admissible.
%
As in the proof of cut admissibility for CLL, we do that by defining a
set of cut reduction and commuting conversions that transform
proofs. From this, we can recover the semantics of core forwarders by
defining the relations on processes $\equiv$, $\reducesto$, and
$\reducesto_\kappa$. We report all cases in
Figure~\ref{fig:coresemantics}.
%
\begin{figure}[t]
  Structural equivalence %(Commuting Conversions)
  \begin{displaymath}\small
    \begin{array}{lr}
      %%% Axiom
      \multicolumn{2}{l}{
      \phl{\fwd xy}%{\cpaxiom yAx{\dual A}}
      \ \equiv\ 
      \phl{\fwd yx}%{\cpaxiom x{\dual A}yA} 
      \qquad %%% commutativity
      \phl{\cpres y{\dual{A}}xA(Q \pp P)}
      \ \equiv\ 
      \phl{\cpres xAy{\dual A} (P \pp Q)} 
      \qquad
      \phl{\cpres {\br{y}}{\dual{A}}{x}A(Q \pp P)}
      \ \equiv\
      \phl{\cpres {x}A{\br{y}}{\dual A} (P \pp Q)}
      }
      \\[1mm] %%%%%
      \phl{\cpres wBz{\dual B} (P \pp \cpres xAy{\dual A} (Q \pp R))}
      \ \equiv\ 
      \phl{\cpres xAy{\dual A}(\cpres wBz{\dual B} (P \pp Q) \pp R)} 
      &\mbox{\footnotesize $\phl x,\phl z \in\fn(\phl Q)$}
      \\[1mm] %%%%%
      \phl{\cpres wB{\br{z}}{\dual B} (P \pp \cpres xA{y}{\dual A} (Q \pp R))}
      \ \equiv\ 
      \phl{\cpres xA{y}{\dual A}(\cpres wB{\br{z}}{\dual B} (P \pp Q) \pp R)}
      &\mbox{\footnotesize $\phl z \in\fn(\phl Q)$}
      \\[1mm]
      \phl{\cpres wB{\br{z}}{\dual B} (P \pp \cpres xA{\br{y}}{\dual A} (Q \pp R))}
      \ \equiv\
      \phl{\cpres xA{\br{y}}{\dual A}(Q \pp\cpres wB{\br{z}}{\dual B} (P \pp R))}
      &\mbox{\footnotesize $\phl y,\phl z \in\fn(\phl R)$}
      \\[1mm]
      \phl{\cpres wB{\br{z}}{\dual B} (\cpres xA{y}{\dual A} (P \pp Q)\pp R)}
      \ \equiv\ 
      \phl{\cpres{x}{B}{\br{y}}{}(P\pp \cpres{w}{A}{\br{z}}{}(Q\pp R))}
      &\mbox{\footnotesize $\phl w,\phl y\in \fn(\phl Q)$}
    \end{array}
  \end{displaymath}
  
  \bigbreak 

  Reductions ($\beta$)
  \begin{displaymath}\small
    \begin{array}{lr}
      % (\m{AxCut}) &
    \phl{\cpres x{X}y{\dual X} ( \fwd xw \pp Q)}
    \ \reducesto\
    \phl{Q \substone wy}
    \\
    % (\m{AxCutBox}) &
    \phl{\cpres x{X}{\br{y}}{\dual X} ( \fwd xw \pp Q)}
    \ \reducesto\
    \phl{Q \substone wy}
    \\
    % (\beta_{\one\perp}) &
    \phl{\cpres x{\one}y\perp(\close x\pp \wait yP)}\quad
    \ \reducesto\
    \phl{P}
    \\
    % (\beta_{\tensor\parr}) &
    \phl{\cpres{x}{A\tensor B}{y}{\dual A\parr \dual B}(\send xuPQ  \pp \recv yvR)}
    \ \reducesto\
    \phl{\cpres{x}{A}{y}{\dual A}(Q  \pp \cpres uA{\br{v}}{\dual A} (P\pp R))}
%    \\
%    &\mbox{\footnotesize Note the apparition of $\phl{\cpres{u}{}{\br{v}}{}}$ here!}
    \\
    % (\beta_{\oplus\with_1}) &
    \phl{\cpres x{A\oplus B}y{\dual A\with \dual B} (\inl xP\pp \Case yQR)}
    \ \reducesto\
     \phl{\cpres xAy{\dual A} (P\pp Q)}
    \\
    % (\beta_{\oplus\with_2}) &
    \phl{\cpres x{A\oplus B}y{\dual A\with \dual B} (\inr xP\pp \Case yQR)}
    \ \reducesto\
    \phl{\cpres x{B}y{\dual B} (P\pp R)}
    \\
    % (\beta_{!?}) &
    \phl{\cpres x{\query A}y{\bang A}(\client xuQ \pp \srv yvP)}
    \ \reducesto\
    \phl{\cpres u{A}v{\dual A}(P \pp Q)}
    \end{array}
  \end{displaymath}
  
  \bigbreak 

  Commuting Conversions ($\kappa$)
  \begin{displaymath}\small
    \begin{array}{lr}
      %%% bot
      \phl{\cpres{x}{}{y}{}(\wait{u}{P}\pp Q)}
      \ \reducesto_\kappa\
      \wait{u}{\cpres{x}{}{y}{}(P\pp Q)}
      \\
      %%% tensor
      \phl{\cpres{x}{}{y}{}(\send uv{P}{Q} \pp R)}
      \ \reducesto_\kappa\
      \send uv{P}{\cpres{x}{}{y}{}(Q \pp R)}
%      &\mbox{\footnotesize $\phl u \in \fn(\phl Q)$}
      % because necessarily $x\in\fn(Q)$}
      \\   	
      %%% parr
      \phl{\cpres{x}{}{y}{}(\recv uv{P}\pp Q)}
      \ \reducesto_\kappa\ 
      \recv uv{\cpres{x}{}{y}{}(P \pp Q)}
      \\
      %%%% oplus
      \phl{\cpres{x}{}{y}{}(\inlr{u}{P}\pp Q)}
      \ \reducesto_\kappa\
      \phl{\inlr{u}{\cpres{x}{}{y}{}(P\pp Q)}}
      \\
      %%% with
      \phl{\cpres{x}{}{y}{}(\Case{u}{P}{Q} \pp R)}
      \ \reducesto_\kappa\
      \Case{u}{\cpres{x}{}{y}{}(P\pp R)}{\cpres{x}{}{y}{}(Q\pp R)}
      \\
      %%%% bang
      \phl{\cpres{x}A{y}{A^\perp}(\srv xzP \pp \srv {u}{v}{Q})}
      \ \reducesto_\kappa\
      \srv {u}{v}{\cpres{x}A{y}{A^\perp}(\srv xzP \pp {Q})}
      \\
      %%%% query
      \phl{\cpres{x}A{y}{A^\perp}(\client uvP \pp Q)}
      \ \reducesto_\kappa\
      \client {u}{v}{\cpres{x}A{y}{A^\perp}(P \pp {Q})}
      \\[2ex]
      %%% bot
      \phl{\cpres{x}{}{\br{y}}{}({P}\pp \wait{u}Q)}
      \ \reducesto_\kappa\
      \wait{u}{\cpres{x}{}{\br{y}}{}(P\pp Q)}
%      &\mbox{\footnotesize $\phl u \in\fn(\phl Q)$}
      \\
      %%% tensor
      \phl{\cpres{x}{}{\br{y}}{}(P \pp \send uv{Q}{R})}
      \ \reducesto_\kappa\
      \send uv{\cpres{x}{}{y}{}(P \pp {Q})}{R}
      &\mbox{\footnotesize $\phl y \in\fn(\phl Q)$}
      % \\
      % &\mbox{\footnotesize Note the change to $\phl{\cpres{x}{}{y}{}}$ here!}
      \\
      \phl{\cpres{x}{}{\br{y}}{}(P \pp \send uv{Q}{R})}
      \ \reducesto_\kappa\
      \send uv{Q}{\cpres{x}{}{\br{y}}{}(P \pp R)}
      &\mbox{\footnotesize $\phl y \in\fn(\phl R)$}
      % because necessarily $u\in\fn(R)$}
      \\
      %%% parr
      \phl{\cpres{x}{}{\br{y}}{}(P \pp \recv uv{Q})}
      \ \reducesto_\kappa\
      \recv uv{\cpres{x}{}{\br{y}}{}(P \pp {Q})}
      \\
      %%%% oplus
      \phl{\cpres{x}{}{\br{y}}{}({P}\pp \inlr{u}Q)}
      \ \reducesto_\kappa\
      \phl{\inlr{u}{\cpres{x}{}{\br{y}}{}(P\pp Q)}}
      \\
      %%% with
      \phl{\cpres{x}{}{\br{y}}{}(P \pp \Case{u}{Q}{R})}
      \ \reducesto_\kappa\
      \Case{u}{\cpres{x}{}{\br{y}}{}(P\pp Q)}{\cpres{x}{}{\br{y}}{}(P\pp R)}
      \\
      %%%% bang
      %%%% query
      \phl{\cpres{x}A{\br{y}}{A^\perp}(P \pp \client uvQ)}
      \ \reducesto_\kappa\
      \client {u}{v}{\cpres{x}A{\br{y}}{A^\perp}(P \pp {Q})}
      % \\
      % \mbox{\sonia{Actually the condition on the variables we see is not enough to have the right-to-left! }}
      % \\
      % \mbox{\sonia{
      % We would need to know for $\oplus$ and $\query$ that the $\dbr{}$ context moves to the same side as well...}}
      % \\
      % \mbox{\sonia{
      % Probably better to write it as a directed relation rather than an equivalence!}}
    \end{array}
  \end{displaymath}
   
  \caption{Semantics of Core Forwarders}
  \label{fig:coresemantics}
\end{figure}
%
%
%
In the sequel, $\Rightarrow$ corresponds to
$\reducesto_\kappa \circ \reducesto \circ \reducesto_\kappa$ and the
$*$ denotes its reflexive and transitive closure.
\begin{theorem}[Cut-admissibility]\ \par
  \begin{enumerate}
  \item If $\coreseq{P}{\Gamma_1, \pairQ{x}{A}}$ and
    $\coreseq {P'} {\Gamma_2, \phl {x'}: \thl{A^\perp}}$, then
    %
    % there exists $\phl Q$ such that
    %
    $\phl{\cpres{x}A{x'}{A^\perp}(P \pp P')} \Rightarrow^*
    \coreseq {Q} {\Gamma_1,\Gamma_2}$.
    
  \item If $\coreseq P {\Delta, \pairQ xA}$ and
    $\coreseq {P'} {\Gamma , [\phl {x'}: \thl {A^\perp}]}$, then
    % 
    % there exists $\phl Q$ such that
    %
    $\phl{\cpres{x}{}{\br{x'}}{}(P \pp P') }\Rightarrow^*
    \coreseq {Q} {\Gamma, [\Delta]}$.
  \end{enumerate}
\end{theorem}

% \sonia{The double arrow corresponds to the composition } \alert{Is
%   this standard notation? Figure 4 uses long singe arrows.  I think we
%   should stay consistent.}  \sonia{$\rightarrow$ is one step of
%   reduction. $\Rightarrow$ is one step of reduction with potentially
%   some equivalences of both sides.}

\begin{proof}(Sketch) The proof is by a mutual lexicographic induction
  on the logical complexity of $A$ and the size of $P$. It can be
  found in Appendix~\ref{app:corecutelim}.
\end{proof}

Below, let $\seq_{0+cut}$ be the extension of $\coreseq{}{}$ with the
cut rules from Figure~\ref{fig:cut0}. From the previous result, we can
then have the following
\begin{theorem}[Cut elimination]
  If $ \phl{P }\seq_{0+cut} \Gamma$, then there exists $\phl{Q}$ such
  that $\phl{P }\Rightarrow^* \phl{Q}$ and $\coreseq
  Q\Gamma$. %% is not a cut.
\end{theorem}
%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Semantics.} The proof of cut elimination contains two types
% of transformations: reductions (those just explained) and commuting
% conversions (as e.g.~in~\eqref{eq:cc_core}). Together, they define two
% relations on processes (reduction $\reducesto$ and structural
% equivalence $\equiv$) which are reported in
% Figure~\ref{fig:coresemantics}. % Such relations are identical to those
% % of CP~\cite{W14}. 
% \sonia{do we want all the structural equivalences
%   on Figure~\ref{fig:coresemantics}?}

% As a consequence of the previous theorem, the following results holds:
\begin{corollary}[Subject Reduction]
  If $\coreseq P \Gamma$ and $\phl P \reducesto \phl Q$ then
  $\coreseq Q \Gamma$.
\end{corollary}
%
\begin{corollary}[Deadlock Freedom]
  If $\coreseq P \Gamma$, then there exists a restriction-free
  $\phl Q$ such that $\phl P \Reducesto^* \phl Q$ and
  $\coreseq Q \Gamma$.
\end{corollary}

\begin{example} \label{ex:comp} We revisit the two buyer
  example~\ref{ex:2buyer}. Using compositionality, we can combine
  forwarders $\phl {P_1}$ and $\phl{P_2}$ to
  $\phl P = \phl{\nu{b_2b_2'} (P_1 | P_2)}$ simplify it using subject
  reduction and obtain the combined forwarder
  \[\coreseq {\phl P}{
      \begin{array}[t]{l}
        %
        
        \pairQ{b_1}{\tname^\perp \parr \tcost \tensor \tcost^\perp \parr\perp},
        % 
        \pairQ{c_1}{\tcost \parr ((\taddr^\perp \parr \perp) \with \perp)}, \\
        % 
        \pairQ{c_2}{\tcost \parr ((\taddr^\perp \parr \perp) \with \perp)},
      % 
      % 
        \pairQ{s}{\tname \tensor \tcost^\perp \parr \tcost^\perp \parr
        ((\taddr \tensor \one) \oplus \one)}
      \end{array}
      % 
    }
    %
  \]
  By subject reduction, we know that the resulting process is a forwarder.
  \qed
\end{example}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> mip.tex <==
\mypar{Multicut Rule.} All rules are as in the linear fragment of ILL,
but without \textsf{Cut}. Exponentials missing. No annotations. We
define \textsf{MCut} as:
\begin{displaymath}
  \begin{array}{llllll}
    \multicolumn{2}{c}{
    \infer[\textsf{MCut}]
    {
    \Gamma_1,\ldots,\Gamma_n,\Gamma\vdash C
    }
    {
    \Gamma_1\vdash A_1   &
                           \ldots
    & 
      \Gamma_n\vdash A_n
    &
      \Gamma,A\vdash C
    &
      A\vDash A_1,\ldots,A_n
      }
      }
    \\\\
    \infer[(\textsf{Ax})]
    {A\vDash A}
    {\textit{This rule makes no sense}}
                         \qquad&\qquad
                           \infer[(\textsf{1})]
                           {1\vDash 1,\ldots, 1}
                           {}
    \\\\
    \infer[(\tensor L\tensor R)]
    {
    A\tensor B\vDash\Gamma,(C_i\tensor D_i)_i
    }
    {
    A\vDash (C_i)_i & B\vDash \Gamma,(D_i)_i
                }
    &
      \infer[(\tensor L\lolli\! L)]
      {
      A\vDash\Gamma,(B_i\tensor C_i)_i,D\lolli E
      }
      {
      D\vDash (B_i)_i & A\vDash\Gamma,(C_i)_i,E
                  }
    \\\\
    \multicolumn{2}{c}{
    \infer[(\tensor L\lolli R\lolli\! L)]
    {
    A\lolli F\vDash\Gamma,(B_i\tensor C_i)_i,D\lolli E
    }
    {
    D\vDash (B_i)_i,A
                         &
                           F\vDash\Gamma,(C_i)_i,E
                           }}
    \\\\
    \infer[(\oplus\! L\oplus\! R)]
    {
    A\oplus B\vDash\Gamma,C\oplus D
    }
    {
    A\vDash\Gamma, C & B\vDash \Gamma,D
                       }
    &
      \infer[(\oplus L\& L)]
      {
      A\vDash\Gamma,B\oplus C,D\& E
      }
      {
      A\vDash \Gamma, B, D & A\vDash\Gamma,C,E
                  }
    \\\\
    \multicolumn{2}{c}{
    \infer[\& L\& R]
    {
    A\& B\vDash\Gamma,C\& D
    }
    {
    A\vDash\Gamma, C & B\vDash\Gamma,D
                }
                       }
  \end{array}
\end{displaymath}
\noindent{\em Conjecture.} \textsf{MCut}-elimination should hold (it
is necessary to have $\eta$-expansion because of no principal
reduction for non-atomic axiom).






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> proofs.tex <==
\subsection {Proofs for Axioms.}

\bigbreak

\noindent{\bf \underline{Principal Cut Ruductions for cut}}

\bigbreak

\noindent{\underline{Case: ax/left}}

\[ \small
  \infer[cut]
  {\Delta; \Gamma, A \vdash \mathbf C}
  {\infer [ax]
    { \cdot ; A \vdash A }
    {}
    \quad \Delta; \Gamma, A \vdash  \mathbf C}
\]


\[\Longrightarrow\]


\[ \small \Delta; \Gamma, A \vdash  \mathbf C \]


\bigbreak 

\noindent{\underline{Case: ax/right}}

\[ \small
  \infer[cut]
  {\Delta; \Gamma \vdash  A}
  {\Delta;\Gamma \vdash A
    \quad \infer[ax]{\cdot; A \vdash A}{}}
\]


\[\Longrightarrow\]


\[ \small \Delta; \Gamma \vdash A \]



\noindent{\bf \underline{Principal Cut Ruductions for cut$\tensor$, cut$\lolli_1$, cut$\lolli_2$ with ax as premiss}}

\bigbreak

These cases are impossible.

\subsection {Proofs for Multiplicatives.}

\bigbreak

\noindent {\bf Observation.} Axiom cut reduction  TBD.

\bigbreak
\bigbreak

\noindent{\bf \underline{Principal Cut Ruductions for\quad  $\scriptsize\infer[cut]
    {\Delta_1,\Delta_2; \Gamma_1, \Gamma_2\vdash \mathbf C}
    {\Delta_1;\Gamma_1 \vdash A
    \quad \Delta_2; \Gamma_2, A \vdash  \mathbf C}
  $}}


\bigbreak

\noindent \underline{ Case ($cut$, $\tensor$).}
\[\small
  \infer[cut]
  {\Delta,\Delta', \Gamma_1\tensor\Gamma_2;
    \Gamma,\Gamma'\vdash\mathbf C}
  {
    \infer[\tensor R]
    {\Delta, \Gamma_1\tensor\Gamma_2;\Gamma \vdash A \tensor B}
    {\cdot; \Gamma_1 \vdash A \quad \Delta; \Gamma, \Gamma_2 \vdash B}
    &
    \infer[\tensor L]
    {\Delta'; \Gamma', A \tensor B \vdash \mathbf C}
    {\Delta', A \tensor B; \Gamma'  \vdash \mathbf C}
  }
\]

\[\Longrightarrow\]

\[\small
  \infer[cut _{\tensor}]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2;
    \Gamma,\Gamma'\vdash\mathbf C
  }
  {
    \cdot; \Gamma_1 \vdash A 
    &
    \Delta; \Gamma, \Gamma_2 \vdash B
    & 
    \Delta', A \tensor B; \Gamma'  \vdash \mathbf C
  }
\]


\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case ($cut$, $\lolli_1$).}
\[\small
  \infer[cut]
  {\Delta,\Delta', \Gamma_1\tensor \Gamma_2; \Gamma,\Gamma'\vdash
    \mathbf C}
  {
    \infer[\lolli\! R]
    {\Delta; \Gamma \vdash A \lolli B}
    {\Delta; \Gamma \vdash [A] \lolli B}
    &
    \infer[\lolli\! L_1]
    {\Delta',\Gamma_1\tensor\Gamma_2; \Gamma', A \lolli B \vdash \mathbf
      C}
    {\cdot; \Gamma_1\vdash A \quad \Delta'; \Gamma', \Gamma_2, B \vdash
      \mathbf C}
  }
\]

\[\Longrightarrow\]

\[\small
  \infer[cut _{\lolli_1}]
  {
    \Delta,\Delta', \Gamma_1\tensor \Gamma_2; \Gamma,\Gamma'\vdash
    \mathbf C
  }
  {
    \cdot; \Gamma_1\vdash A
    &
    \Delta; \Gamma \vdash [A] \lolli B
    &
    \Delta'; \Gamma', \Gamma_2, B \vdash  \mathbf C
  }
\]


\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case ($cut$, $\lolli_2$).}
\[\small
  \infer[cut]
  {
    \Delta,\Delta',
    \Gamma_1\tensor\Gamma_2;\Gamma,\Gamma'\vdash[C]\lolli D
  }
  {
    \infer[\lolli\! R]
    {\Delta; \Gamma \vdash A \lolli B}
    {\Delta; \Gamma \vdash [A] \lolli B}
    &
    \infer[\lolli\! L_2]
    {\Delta', \Gamma_1\tensor\Gamma_2; \Gamma', A \lolli B \vdash [C] \lolli D}
      {\cdot; \Gamma_1, C \vdash A \quad
      \Delta'; \Gamma',\Gamma_2, B \vdash D}
  }
\]

\[\Longrightarrow\]

\[\small
  \infer[cut _{\lolli_2}]
  {
    \Delta,\Delta',
    \Gamma_1\tensor\Gamma_2;\Gamma,\Gamma'\vdash[C]\lolli D
  }
  {
    \cdot; \Gamma_1, C \vdash A 
    & \Delta; \Gamma \vdash [A] \lolli B
    & \Delta'; \Gamma',\Gamma_2, B \vdash D
  }
\]


\newpage
\noindent{\bf \underline{Principal Cut Ruductions for\quad
    $\scriptsize\infer[cut _{\tensor}] { \Delta,\Delta',
      \Gamma_1\tensor\Gamma_2; \Gamma,\Gamma' \vdash \mathbf C } {
      \cdot; \Gamma_1\vdash A & \Delta; \Gamma, \Gamma_2\vdash B &
      \Delta', A\tensor B; \Gamma'\vdash \mathbf C }$
  }} \\

\noindent \underline{ Case ($cut_{\tensor}$, $\tensor R$).}
\[\small
  \infer[cut _{\tensor}]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2, \Gamma_1'\tensor\Gamma_2';
    \Gamma,\Gamma' \vdash C\tensor D
  }
  {
    \cdot; \Gamma_1\vdash A
    &
    \Delta; \Gamma, \Gamma_2\vdash B
    & 
    \infer[\tensor R]
    {\Delta', \Gamma_1'\tensor\Gamma_2', A\tensor B;\Gamma' \vdash C \tensor D}
    {\cdot; \Gamma_1', A \vdash C \quad \Delta'; \Gamma', \Gamma_2', B \vdash D}
  }
\]


\[\Longrightarrow\]

\[\small
  \infer[\tensor R]
  {
    \Delta,\Delta', (\Gamma_1,\Gamma_1')\tensor (\Gamma_2,\Gamma_2');
    \Gamma,\Gamma'\vdash C\tensor D
  }
  {
    \infer[cut]
    {
      \cdot; \Gamma_1, \Gamma_1'\vdash C
    }
    {
      \cdot; \Gamma_1\vdash A
      &
      \cdot; \Gamma_1', A \vdash C
    }
    &
    \infer[cut]
    {
      \Delta,\Delta'; \Gamma,\Gamma', \Gamma_2,\Gamma_2'\vdash D
    }
    {
      \Delta; \Gamma, \Gamma_2\vdash B
      &
      \Delta'; \Gamma', \Gamma_2', B \vdash D
    }
  }
\]
because
$\Gamma_1\tensor \Gamma_2, \Gamma_1'\tensor \Gamma_2'
=
(\Gamma_1,\Gamma_1')\tensor (\Gamma_2,\Gamma_2')$

\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case ($cut_{\tensor}$, $\lolli L_1$).}
\[\small
  \infer[cut _{\tensor}]
  {
    \Delta_1,\Delta_2, \Gamma_1\tensor \Gamma_2, \Gamma_1',\tensor \Gamma_2';\Gamma,\Gamma', C\lolli D
    \vdash E
  }
  {
    \cdot;\Gamma_1\vdash A
    &
    \Delta;\Gamma,\Gamma_2\vdash B
    & 
    \infer[\lolli\! L_1]
    {\Delta',\Gamma_1'\tensor \Gamma_2',A \tensor B;\Gamma',  C \lolli D \vdash E}
    {\cdot;\Gamma_1',A  \vdash C \quad \Delta';\Gamma', \Gamma_2', B, D \vdash E}
  }
\]

\[\Longrightarrow\]

\[\small
  \infer[\lolli L_1]
  {
    \Delta,\Delta',(\Gamma_1,\Gamma_1')\tensor (\Gamma_2,\Gamma_2');
    \Gamma,\Gamma',
    C\lolli D
    \vdash E
  }
  {
    \infer[cut]
    {
      \cdot;\Gamma_1, \Gamma_1'\vdash C
    }
    {
      \cdot;\Gamma_1\vdash A
      &
      \cdot;\Gamma_1', A \vdash C
    }
    &
    \infer[cut]
    {
      \Delta,\Delta';\Gamma,\Gamma', \Gamma_2, \Gamma_2', D\vdash E
    }
    {
       \Delta;\Gamma,\Gamma_2 \vdash B
       &
       \Delta';\Gamma', \Gamma_2', B, D \vdash E
    }
  }
\]
because
$\small\Gamma_1\tensor \Gamma_2, \Gamma_1'\tensor \Gamma_2' =
(\Gamma_1,\Gamma_1')\tensor (\Gamma_2,\Gamma_2')$


\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case ($cut_{\tensor}$, $\lolli L_2$).}
\[\small
  \infer[cut _{\tensor}]
  {
    \Delta,\Delta',\Gamma_1\tensor\Gamma_2, \Gamma_1'\tensor \Gamma_2';\Gamma,\Gamma', C\lolli D
    \vdash [E]\lolli F
  }
  {
    \cdot;\Gamma_1\vdash A
    &
    \Delta;\Gamma,\Gamma_2\vdash B
    & 
    \infer[\lolli\! L_2]
    {\Delta',\Gamma_1'\tensor \Gamma_2', A\tensor B;\Gamma', C \lolli D \vdash
      [E]\lolli F}
    {\cdot;\Gamma_1',E,A  \vdash C \quad \Delta';\Gamma', \Gamma_2', B, D \vdash F}
  }
\]

\[\Longrightarrow\]

\[\small
  \infer[\lolli L_2]
  {
    \Delta,\Delta', (\Gamma_1,\Gamma_1') \tensor (\Gamma_2,\Gamma_2');\Gamma,\Gamma',
    C\lolli D
    \vdash [E]\lolli F
  }
  {
    \infer[cut]
    {
      \cdot;\Gamma_1,\Gamma_1', E\vdash C
    }
    {
      \cdot;\Gamma_1\vdash A
      &
      \cdot;\Gamma_1', E, A \vdash C
    }
    &
    \infer[cut]
    {
      \Delta,\Delta';\Gamma,\Gamma', \Gamma_2,\Gamma_2', D\vdash F
    }
    {
      \Delta;\Gamma,\Gamma_2\vdash B
      &
      \Delta';\Gamma', \Gamma_2', B, D \vdash F
    }
  }
\]
because
$\small\Gamma_1\tensor \Gamma_2, \Gamma_1'\tensor \Gamma_2' =
(\Gamma_1,\Gamma_1')\tensor (\Gamma_2,\Gamma_2')$



\newpage
\noindent{\bf \underline{Principal Cut Ruductions for
  $\scriptsize
  \infer[cut _{\lolli_1}]
  { \Delta,\Delta',\Gamma_1\tensor \Gamma_2; \Gamma,\Gamma'\vdash
    \mathbf C }
  { \cdot; \Gamma_1\vdash A & \Delta; \Gamma \vdash [A] \lolli B
    &
    \Delta'; \Gamma', \Gamma_2, B \vdash \mathbf C }$}} \\

\noindent \underline{ Cases ($cut_{\lolli_1}$, $\tensor R$) and ($cut_{\lolli_1}$, $\lolli L_1$).}\\

\noindent {\em Both cases are not applicable since $\tensor R$
  requires the conclusions to be a $\tensor$ and, $\lolli L_1$ does
  not use the $A$ in the conclusion. Both cases are addressed as
  commuting conversions.}

\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case ($cut_{\lolli_1}$, $\lolli L_2$).}
\[\small
  \infer[cut _{\lolli_1}]
  {
    \Delta, \Delta', \Gamma_1\tensor\Gamma_2, \Gamma_1'\tensor\Gamma_2';
    \Gamma,\Gamma', C\lolli D\vdash\mathbf C
  }
  {
    \cdot;\Gamma_1\vdash A
    &
    \infer[\lolli\! L_2]
    {\Delta, \Gamma_1'\tensor\Gamma_2'; \Gamma, C \lolli D \vdash [A] \lolli B}
    {\cdot; \Gamma_1', A \vdash C \quad
      \Delta; \Gamma,\Gamma_2', D \vdash B}
    &
    \Delta'; \Gamma', \Gamma_2, B \vdash \mathbf C 
  }
\]

\[\Longrightarrow\]

\[\small
  \infer[\lolli L_1]
  {
    \Delta,\Delta', (\Gamma_1,\Gamma_1')\tensor(\Gamma_2,\Gamma_2');
    \Gamma,\Gamma', C\lolli D\vdash\mathbf C
  }
  {
    \infer[cut]
    {
      \cdot;\Gamma_1,\Gamma_1'\vdash C
    }
    {
      \cdot;\Gamma_1\vdash A
      &
      \cdot; \Gamma_1', A \vdash C
    }
    &
    \infer[cut]
    {
      \Delta,\Delta'; \Gamma,\Gamma',\Gamma_2, \Gamma_2',
      D\vdash\mathbf C
    }
    {
      \Delta; \Gamma,\Gamma_2', D \vdash B
      &
      \Delta'; \Gamma', \Gamma_2, B \vdash \mathbf C 
    }
  }
\]
because
$\small\Gamma_1\tensor \Gamma_2, \Gamma_1'\tensor \Gamma_2' =
(\Gamma_1,\Gamma_1')\tensor (\Gamma_2,\Gamma_2')$

\bigbreak
\bigbreak

\noindent{\bf \underline{Principal Cut Ruductions for $\scriptsize
    \infer[cut _{\lolli_2}]
    {
    \Delta,\Delta',
    \Gamma_1\tensor\Gamma_2;\Gamma,\Gamma'\vdash[C]\lolli D
    }
    {
    \cdot; \Gamma_1, C \vdash A 
    & \Delta; \Gamma \vdash [A] \lolli B
    & \Delta'; \Gamma',\Gamma_2, B \vdash D
      }$}} \\

\noindent \underline{Cases ($cut_{\lolli_2}$, $\tensor R$) and ($cut_{\lolli_2}$, $\lolli L_1$).}\\

{\em Not applicable as for $cut_{\lolli_2}$.}

\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\lolli_2}$, $\lolli L_2$.}
\[\small
  \infer[cut _{\lolli_2}]
  {
    \Delta, \Delta', \Gamma_1\tensor\Gamma_2, \Gamma_1'\tensor\Gamma_2';
    \Gamma,\Gamma', C\lolli D\vdash[E]\lolli F
  }
  {
    \cdot;\Gamma_1,E\vdash A
    &
    \infer[\lolli\! L_2]
    {\Delta, \Gamma_1'\tensor\Gamma_2'; \Gamma, C \lolli D \vdash [A] \lolli B}
    {\cdot; \Gamma_1', A \vdash C \quad
      \Delta; \Gamma,\Gamma_2', D \vdash B}
    &
    \Delta'; \Gamma', \Gamma_2, B \vdash F
  }
\]

\[\Longrightarrow\]

\[\small
  \infer[\lolli L_2]
  {
    \Delta,\Delta', (\Gamma_1,\Gamma_1')\tensor(\Gamma_2,\Gamma_2');
    \Gamma,\Gamma', C\lolli D\vdash [E]\lolli F
  }
  {
    \infer[cut]
    {
      \cdot;\Gamma_1,\Gamma_1',E\vdash C
    }
    {
      \cdot;\Gamma_1,E\vdash A
      &
      \cdot; \Gamma_1', A \vdash C
    }
    &
    \infer[cut]
    {
      \Delta,\Delta'; \Gamma,\Gamma',\Gamma_2, \Gamma_2',
      D\vdash F
    }
    {
      \Delta; \Gamma,\Gamma_2', D \vdash B
      &
      \Delta'; \Gamma', \Gamma_2, B \vdash F 
    }
  }
\]
because
$\small\Gamma_1\tensor \Gamma_2, \Gamma_1'\tensor \Gamma_2' =
(\Gamma_1,\Gamma_1')\tensor (\Gamma_2,\Gamma_2')$


\newpage
\noindent{\bf Commuting Conversions for\quad
  $\scriptsize \infer[cut] {\Delta_1,\Delta_2; \Gamma_1,
    \Gamma_2\vdash \mathbf C} {\Delta_1;\Gamma_1 \vdash A \quad
    \Delta_2; \Gamma_2, A \vdash \mathbf C} $}

\bigbreak
\bigbreak
\noindent \underline{Cases ($cut$, left $\tensor R$) and ($cut$, right
  $\tensor R$, left).}\\


\noindent {\em Not applicable: if $\tensor R$ is on the left, we have
  a principal case; if $\tensor R$ is on the right premise, we cannot
  have this case because of the restriction on the left premise of
  $\tensor R$.}

\bigbreak
\bigbreak

\noindent \underline{ Case $cut$, right $\tensor R$, right.}
\smallbreak
\[\footnotesize
  \begin{array}{ccc}
    \infer[cut]
    {
    \Delta, \Delta', \Gamma_1\tensor\Gamma_2;
    \Gamma, \Gamma'\vdash A \tensor B
    }
    {
    \Delta; \Gamma\vdash C
    &
    \infer[\tensor R]
    {\Delta', \Gamma_1\tensor\Gamma_2;\Gamma' , C\vdash A \tensor B}
    {\cdot; \Gamma_1 \vdash A \quad \Delta'; \Gamma', \Gamma_2, C \vdash B}
                          }
    &
      \quad\Longrightarrow\quad
    &
      \infer[\tensor R]
      {
      \Delta,\Delta',\Gamma_1\tensor\Gamma_2; \Gamma, \Gamma'\vdash
      A\tensor B
      }
      {
      {\cdot; \Gamma_1 \vdash A}
    &
      \infer[cut]
      {\Delta,\Delta'; \Gamma, \Gamma', \Gamma_2\vdash B}
      {
      \Delta; \Gamma\vdash C
    &
      \Delta'; \Gamma', \Gamma_2, C \vdash B
      }
      }
  \end{array}
\]



\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case $cut$, left $\tensor L$.}

\[\footnotesize
  \infer[cut]
  {
    \Delta,\Delta'; \Gamma, \Gamma' \vdash \mathbf C
  }
  {
    \infer[\tensor L]
    {\Delta; \Gamma, A \tensor B \vdash C}
    {\Delta, A \tensor B; \Gamma  \vdash C}
    &
    \Delta'; \Gamma', C\vdash \mathbf C
  }
  \qquad\Longrightarrow\qquad
  \infer[\tensor L]
  {
    \Delta,\Delta';\Gamma,\Gamma', A\tensor B\vdash \mathbf C
  }
  {
    \infer[cut]
    {
      \Delta,\Delta',A\tensor B;\Gamma,\Gamma'\vdash \mathbf C
    }
    {
      \Delta, A \tensor B; \Gamma  \vdash C
      &
      \Delta';\Gamma', C\vdash \mathbf C
    }
  }
\]


\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case $cut$, right $\tensor L$.}

\[\footnotesize
  \infer[cut]
  {
    \Delta,\Delta'; \Gamma,\Gamma',A\tensor B\vdash \mathbf C
  }
  {
    \Delta;\Gamma\vdash C
    &
    \infer[\tensor L]
    {\Delta'; \Gamma', A \tensor B, C \vdash \mathbf C}
    {\Delta', A \tensor B; \Gamma', C \vdash \mathbf C}
  }
  \qquad\Longrightarrow\qquad 
  \infer[\tensor L]
  {
    \Delta,\Delta'; \Gamma,\Gamma', A\tensor B\vdash \mathbf C
  }
  {
    \infer[cut]
    {
      \Delta,\Delta', A\tensor B; \Gamma,\Gamma'\vdash \mathbf C
    }
    {
      \Delta; \Gamma\vdash C
      &
      {\Delta', A \tensor B; \Gamma', C \vdash \mathbf C}
    }
  }
\]

\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case ($cut$, left $\lolli L_1$, left).}\\

{\em Not applicable (as in ILL).}

\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case ($cut$, left $\lolli L_1$, right).}\\

\[\scriptsize
  \infer[cut]
  {
    \Delta,\Delta',\Gamma_1\tensor\Gamma_2; \Gamma,\Gamma',A\lolli B\vdash \mathbf C
  }
  {
    \infer[\lolli\! L_1]
    {
      \Delta,\Gamma_1\tensor\Gamma_2; \Gamma, A \lolli B \vdash C
    }
    {
      \cdot; \Gamma_1\vdash A
      &
      \Delta; \Gamma, \Gamma_2, B \vdash C
    }
    &
    \Delta'; \Gamma', C\vdash \mathbf C
  }
  \quad\Longrightarrow\quad 
  \infer[\lolli L_1]
  {
    \Delta,\Delta',\Gamma_1\tensor\Gamma_2;\Gamma,\Gamma',A\lolli
    B\vdash \mathbf C
  }
  {
    \cdot; \Gamma_1\vdash A
    &
    \infer[cut]
    {
      \Delta,\Delta';\Gamma,\Gamma', B\vdash \mathbf C
    }
    {
      \Delta; \Gamma, \Gamma_2, B \vdash C
      &
      {
        \Delta'; \Gamma', C\vdash \mathbf C
      }
    }
  }
\]


\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case ($cut$, right $\lolli L_1$, left).}\\

{\em Not applicable, as in the ($cut$, right $\tensor R$, left) case.}

\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case ($cut$, right $\lolli L_1$, right).}

\[\footnotesize
  \infer[cut]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2; \Gamma', \Gamma,A \lolli
    B\vdash\mathbf C
  }
  {
    \Delta;\Gamma\vdash C
    &
    \infer[\lolli\! L_1]
    {
      \Delta',\Gamma_1\tensor\Gamma_2; \Gamma', C, A \lolli B \vdash \mathbf
      C
    }
    {
      \cdot; \Gamma_1\vdash A
      &
      \Delta'; \Gamma', \Gamma_2, C, B \vdash
      \mathbf C
    }
  }
  \quad\Longrightarrow\hspace{3cm}
\]
\[\footnotesize
  \hspace{3cm}
  \infer[\lolli\! L_1]
  {
    \Delta,\Delta',\Gamma_1\tensor\Gamma_2; \Gamma,\Gamma', A\lolli
    B\vdash\mathbf C
  }
  {
    \cdot; \Gamma_1\vdash A
    &
    \infer[cut]
    {
      \Delta,\Delta'; \Gamma, \Gamma', \Gamma_2, B \vdash
      \mathbf C
    }
    {
      \Delta;\Gamma\vdash C
      &
      \Delta'; \Gamma', \Gamma_2, C, B \vdash
      \mathbf C
    }
  }
\]

\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Cases with ($cut$, left $\lolli L_2$)}\\

\noindent {\em Not applicable: $\lolli L_2$ cannot be on the left,
  since we cannot use $cut$ on a boxed $\lolli$ on the right;
  $\lolli L_2$ cannot be on the right where we swap on the its left
  premise, as for $\lolli L_1$.}

\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case ($cut$, right $\lolli L_2$, right).}

\[\scriptsize
  \infer[cut]
  {
    \Delta,\Delta',\Gamma_1\tensor\Gamma_2;\Gamma,\Gamma', A\lolli
    B\vdash [D]\lolli E
  }
  {
    \Delta;\Gamma\vdash C
    &
    \infer[\lolli\! L_2]
    {\Delta', \Gamma_1\tensor\Gamma_2; \Gamma', C, A \lolli B \vdash [D] \lolli E}
    {
      \cdot; \Gamma_1, D \vdash A
      &
      \Delta'; \Gamma',\Gamma_2, ,C, B \vdash E
    }
  }
  \quad\Longrightarrow\hspace{3cm}
\]
\[\scriptsize
  \hspace{3cm}
  \infer[\lolli\! L_2]
  {
    \Delta,\Delta',\Gamma_1\tensor\Gamma_2;\Gamma,\Gamma',A\lolli
    B\vdash[D]\lolli E
  }
  {
    \cdot; \Gamma_1, D \vdash A
    &
    \infer[cut]
    {
      \Delta,\Delta';\Gamma,\Gamma',\Gamma_2, B\vdash E
    }
    {
      \Delta;\Gamma\vdash C
      &
      \Delta'; \Gamma',\Gamma_2, C, B \vdash E
    }
  }
\]

\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case $cut$, left $\lolli\! R$.}\\

{\em Not applicable (as in ILL).}

\bigbreak
\bigbreak
\bigbreak

\noindent \underline{ Case $cut$, right $\lolli\! R$.}

\[\scriptsize
  \infer[cut]
  {
    \Delta,\Delta'; \Gamma,\Gamma'\vdash A\lolli B
  }
  {
    \Delta;\Gamma\vdash C
    &
    \infer[\lolli\! R]
    {\Delta'; \Gamma',C \vdash A \lolli B}
    {\Delta'; \Gamma',C \vdash [A] \lolli B}
  }
  \qquad\Longrightarrow\qquad
  \infer[\lolli\! R]
  {
    \Delta,\Delta';\Gamma,\Gamma'\vdash A\lolli B
  }
  {
    \infer[cut]
    {
      \Delta,\Delta';\Gamma,\Gamma'\vdash [A]\lolli B
    }
    {
      \Delta;\Gamma\vdash C
      &
      \Delta'; \Gamma',C \vdash [A] \lolli B
    }
  }
\]

\newpage
\noindent{\bf Commuting Conversions for\quad
  $\scriptsize\infer[cut _{\tensor}]
    {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2;
    \Gamma,\Gamma' \vdash \mathbf C
    }
    {
    \cdot; \Gamma_1\vdash A
    &
      \Delta; \Gamma, \Gamma_2\vdash B
    & 
      \Delta', A\tensor B; \Gamma'\vdash \mathbf C
      }
$}

\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\tensor}$, $\tensor R$, left.}\\

\noindent {\em Not applicable: we cannot have this case because of the
  restriction on the left premise of $\tensor R$  (splitting).}

\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\tensor}$, $\tensor R$, right.}

\[\footnotesize
  \infer[cut _{\tensor}]
  {
    \Delta,\Delta',\Gamma_1\tensor\Gamma_2,\Gamma_3\tensor\Gamma_4;\Gamma,\Gamma'\vdash
    C\tensor B
  }
  {
    \cdot;\Gamma_1\vdash A
    &
    \Delta;\Gamma,\Gamma_2\vdash B
    & 
    \infer[\tensor R]
    {
      \Delta', \Gamma_3\tensor\Gamma_4, A\tensor B;\Gamma' \vdash C
      \tensor D
    }
    {
      \cdot; \Gamma_3 \vdash C
      &
      \Delta', A\tensor B; \Gamma', \Gamma_4 \vdash D
    }
  }
\]
\[\Longrightarrow\]
\[\footnotesize
  \infer[\tensor R]
  {
    \Delta,\Delta',\Gamma_1\tensor\Gamma_2,\Gamma_3\tensor\Gamma_4;\Gamma,\Gamma'
    \vdash  C\tensor D
  }
  {
    \cdot;\Gamma_3\vdash C
    &
    \infer[cut _{\tensor}]
    {
      \Delta,\Delta',\Gamma_1\tensor\Gamma_2;\Gamma,\Gamma', \Gamma_4\vdash
      D
    }
    {
      \cdot;\Gamma_1\vdash A
      &
      \Delta;\Gamma,\Gamma_2\vdash B
      & 
      \Delta', A\tensor B; \Gamma', \Gamma_4 \vdash D
    }
  }
\]

\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\tensor}$, $\tensor L$.}

\[\footnotesize 
  \infer[cut _{\tensor}]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2;
    \Gamma,\Gamma',C\tensor D \vdash \mathbf C
  }
  {
    \cdot; \Gamma_1\vdash A
    &
    \Delta; \Gamma, \Gamma_2\vdash B
    &
    \infer[\tensor L]
    {
      \Delta', A\tensor B; \Gamma',C\tensor D\vdash \mathbf C
    }
    {
      \Delta', A\tensor B, C\tensor D; \Gamma',\vdash \mathbf C
    }
  }
\]
\[\Longrightarrow\]
\[\footnotesize 
  \infer[\tensor L]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2;
    \Gamma,\Gamma',C\tensor D \vdash \mathbf C
  }
  {
    \infer[cut _{\tensor}]
    {
      \Delta,\Delta', \Gamma_1\tensor\Gamma_2,C\tensor D;
      \Gamma,\Gamma' \vdash \mathbf C
    }
    {
      \cdot; \Gamma_1\vdash A
      &
      \Delta; \Gamma, \Gamma_2\vdash B
      &
      \Delta', A\tensor B, C\tensor D; \Gamma',\vdash \mathbf C
    }
  }
\]

\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\tensor}$, $\lolli L_1$, left.}\\

\noindent {\em Not applicable: we cannot have this case because of the
  restriction on the left premise of $\lolli L_1$ (splitting).}

\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\tensor}$, $\lolli L_1$, right.}

\[\footnotesize
  \infer[cut _{\tensor}]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2, \Gamma_3\tensor\Gamma_4;
    \Gamma,\Gamma', C\lolli D \vdash \mathbf C
  }
  {
    \cdot; \Gamma_1\vdash A
    &
    \Delta; \Gamma, \Gamma_2\vdash B
    & 
    \infer[\lolli\! L_1]
    {
      \Delta',\Gamma_3\tensor\Gamma_4,A\tensor B; \Gamma', C \lolli D
      \vdash \mathbf C
    }
    {
      \cdot; \Gamma_3\vdash C
      &
      \Delta'; \Gamma', \Gamma_4, A\tensor B, D \vdash \mathbf C
    }
  }
\]
\[\Longrightarrow\]
\[\footnotesize
  \infer[\lolli L_1]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2, \Gamma_3\tensor\Gamma_4;
    \Gamma,\Gamma',C\lolli D \vdash \mathbf C
  }
  {
    \cdot; \Gamma_3\vdash C
    &
    \infer[cut _{\tensor}]
    {
      \Delta,\Delta', \Gamma_1\tensor\Gamma_2;
      \Gamma,\Gamma',\Gamma_4,D \vdash \mathbf C
    }
    {
      \cdot; \Gamma_1\vdash A
      &
      \Delta; \Gamma, \Gamma_2\vdash B
      & 
      \Delta'; \Gamma', \Gamma_4, A\tensor B, D \vdash \mathbf C
    }
  }
\]



\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\tensor}$, $\lolli L_2$, left.}\\

\noindent {\em Not applicable: we cannot have this case because of the
  restriction on the left premise of $\lolli L_2$ (splitting).}

\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\tensor}$, $\lolli L_2$, right.}

\[\footnotesize
  \infer[cut _{\tensor}]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2, \Gamma_3\tensor\Gamma_4;
    \Gamma,\Gamma', C\lolli D \vdash [E]\lolli F
  }
  {
    \cdot; \Gamma_1\vdash A
    &
    \Delta; \Gamma, \Gamma_2\vdash B
    & 
    \infer[\lolli\! L_2]
    {
      \Delta',\Gamma_3\tensor\Gamma_4,A\tensor B; \Gamma', C \lolli D
      \vdash [E]\lolli F
    }
    {
      \cdot; \Gamma_3,E\vdash C
      &
      \Delta'; \Gamma', \Gamma_4, A\tensor B, D \vdash F
    }
  }
\]
\[\Longrightarrow\]
\[\footnotesize
  \infer[\lolli L_1]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2, \Gamma_3\tensor\Gamma_4;
    \Gamma,\Gamma',C\lolli D \vdash [E]\lolli F
  }
  {
    \cdot; \Gamma_3,E\vdash C
    &
    \infer[cut _{\tensor}]
    {
      \Delta,\Delta', \Gamma_1\tensor\Gamma_2;
      \Gamma,\Gamma',\Gamma_4,D \vdash F
    }
    {
      \cdot; \Gamma_1\vdash A
      &
      \Delta; \Gamma, \Gamma_2\vdash B
      & 
      \Delta'; \Gamma', \Gamma_4, A\tensor B, D \vdash F
    }
  }
\]


\newpage
\newpage
\noindent{\bf Commuting Conversions for\quad
  $\scriptsize
  \infer[cut _{\lolli_1}]
  {
    \Delta,\Delta', \Gamma_1\tensor \Gamma_2; \Gamma,\Gamma'\vdash
    \mathbf C
  }
  {
    \cdot; \Gamma_1\vdash A
    &
    \Delta; \Gamma \vdash [A] \lolli B
    &
    \Delta'; \Gamma', \Gamma_2, B \vdash  \mathbf C
  }
  $}

\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\lolli_1}$, $\tensor R$.}\\

\noindent {\em Not applicable.}


\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\lolli_1}$, $\tensor L$.}

\[\footnotesize 
  \infer[cut _{\lolli_1}]
  {
    \Delta,\Delta', \Gamma_1\tensor \Gamma_2; \Gamma,\Gamma', C\tensor D\vdash
    \mathbf C
  }
  {
    \cdot; \Gamma_1\vdash A
    &
    \infer[\tensor L]
    {
      \Delta; \Gamma,C\tensor D \vdash [A] \lolli B
    }
    {
      \Delta, C\tensor D; \Gamma \vdash [A] \lolli B
    }
    &
    \Delta'; \Gamma', \Gamma_2, B \vdash  \mathbf C
  }
\]
\[\Longrightarrow\]
\[\footnotesize
  \infer[\tensor L]
  {
    \Delta,\Delta', \Gamma_1\tensor \Gamma_2; \Gamma,\Gamma', C\tensor D\vdash
    \mathbf C
  }
  {
    \infer[cut _{\lolli_1}]
    {
      \Delta,\Delta', \Gamma_1\tensor \Gamma_2, C\tensor D; \Gamma,\Gamma'\vdash
      \mathbf C
    }
    {
      \cdot; \Gamma_1\vdash A
      &
      \Delta, C\tensor D; \Gamma \vdash [A] \lolli B
      &
      \Delta'; \Gamma', \Gamma_2, B \vdash  \mathbf C
    }
  }
\]

\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\lolli_1}$, $\lolli L_1$.}

\[\footnotesize
  \infer[cut _{\lolli_1}]
  {
    \Delta,\Delta', \Gamma_1\tensor \Gamma_2, \Gamma_3\tensor
    \Gamma_4; \Gamma,\Gamma', C\lolli D\vdash\mathbf C
  }
  {
    \cdot; \Gamma_1\vdash A
    &
    \infer[\lolli L_1]
    {
      \Delta,\Gamma_3\tensor\Gamma_4; \Gamma,C\lolli D \vdash [A] \lolli B
    }
    {
      \cdot; \Gamma_3\vdash C
      &
      \Delta; \Gamma, \Gamma_4, D \vdash \mathbf [A]\lolli B
    }
    &
    \Delta'; \Gamma', \Gamma_2, B \vdash  \mathbf C
  }
\]
\[\Longrightarrow\]
\[\footnotesize
  \infer[\lolli L_1]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2, \Gamma_3\tensor\Gamma_4;
    \Gamma,\Gamma',C\lolli D \vdash \mathbf C
  }
  {
    \cdot; \Gamma_3\vdash C
    &
    \infer[cut _{\lolli_1}]
    {
      \Delta,\Delta', \Gamma_1\tensor\Gamma_2;
      \Gamma,\Gamma',\Gamma_4,D \vdash \mathbf C
    }
    {
      \cdot; \Gamma_1\vdash A
      &
      \Delta; \Gamma, \Gamma_4, D \vdash \mathbf [A]\lolli B
      & 
      \Delta'; \Gamma', \Gamma_2, B \vdash  \mathbf C      
    }
  }
\]



\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\lolli_1}$, $\lolli L_2$.}\\

\noindent {\em Not applicable (see Principal Cut).}

\bigbreak
\bigbreak


\newpage
\newpage
\noindent{\bf Commuting Conversions for\quad
  $\scriptsize
  \infer[cut _{\lolli_2}]
  {
    \Delta,\Delta', \Gamma_1\tensor \Gamma_2; \Gamma,\Gamma'\vdash
    [C]\lolli D
  }
  {
    \cdot; \Gamma_1, C\vdash A
    &
    \Delta; \Gamma \vdash [A] \lolli B
    &
    \Delta'; \Gamma', \Gamma_2, B \vdash  D
  }
  $}

\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\lolli_2}$, $\tensor R$.}\\

\noindent {\em Not applicable.}


\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\lolli_2}$, $\tensor L$.}

\[\footnotesize 
  \infer[cut _{\lolli_2}]
  {
    \Delta,\Delta', \Gamma_1\tensor \Gamma_2; \Gamma,\Gamma', C\tensor D\vdash
    [E]\lolli F
  }
  {
    \cdot; \Gamma_1,E\vdash A
    &
    \infer[\tensor L]
    {
      \Delta; \Gamma,C\tensor D \vdash [A] \lolli B
    }
    {
      \Delta, C\tensor D; \Gamma \vdash [A] \lolli B
    }
    &
    \Delta'; \Gamma', \Gamma_2, B \vdash  F
  }
\]
\[\Longrightarrow\]
\[\footnotesize
  \infer[\tensor L]
  {
    \Delta,\Delta', \Gamma_1\tensor \Gamma_2; \Gamma,\Gamma', C\tensor D\vdash
    [E]\lolli F
  }
  {
    \infer[cut _{\lolli_2}]
    {
      \Delta,\Delta', \Gamma_1\tensor \Gamma_2, C\tensor D; \Gamma,\Gamma'\vdash
      [E]\lolli F
    }
    {
      \cdot; \Gamma_1, E\vdash A
      &
      \Delta, C\tensor D; \Gamma \vdash [A] \lolli B
      &
      \Delta'; \Gamma', \Gamma_2, B \vdash  F
    }
  }
\]

\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\lolli_2}$, $\lolli L_1$.}

\[\footnotesize
  \infer[cut _{\lolli_2}]
  {
    \Delta,\Delta', \Gamma_1\tensor \Gamma_2, \Gamma_3\tensor
    \Gamma_4; \Gamma,\Gamma', C\lolli D\vdash [E]\lolli F
  }
  {
    \cdot; \Gamma_1,E\vdash A
    &
    \infer[\lolli L_1]
    {
      \Delta,\Gamma_3\tensor\Gamma_4; \Gamma,C\lolli D \vdash [A] \lolli B
    }
    {
      \cdot; \Gamma_3\vdash C
      &
      \Delta; \Gamma, \Gamma_4, D \vdash \mathbf [A]\lolli B
    }
    &
    \Delta'; \Gamma', \Gamma_2, B \vdash F
  }
\]
\[\Longrightarrow\]
\[\footnotesize
  \infer[\lolli L_1]
  {
    \Delta,\Delta', \Gamma_1\tensor\Gamma_2, \Gamma_3\tensor\Gamma_4;
    \Gamma,\Gamma',C\lolli D \vdash [E]\lolli F
  }
  {
    \cdot; \Gamma_3\vdash C
    &
    \infer[cut _{\lolli_1}]
    {
      \Delta,\Delta', \Gamma_1\tensor\Gamma_2;
      \Gamma,\Gamma',\Gamma_4,D \vdash [E]\lolli F
    }
    {
      \cdot; \Gamma_1,E\vdash A
      &
      \Delta; \Gamma, \Gamma_4, D \vdash \mathbf [A]\lolli B
      & 
      \Delta'; \Gamma', \Gamma_2, B \vdash  F
    }
  }
\]



\bigbreak
\bigbreak

\noindent \underline{ Case $cut_{\tensor}$, $\lolli L_2$.}\\

\noindent {\em Not applicable (principal Case).}

\bigbreak
\bigbreak


\newpage
\subsection {Proofs for Additives.}

\[
  \infer[cut]
  {
    \Delta_1,\Delta_2,L(C);\Gamma_1,\Gamma_2\vdash\mathbf C
  }
  {
  \infer[\oplus R_1]
  {
    \Delta_1,L(C);\Gamma_1\vdash A\oplus B
  }
  {
    \Delta_1;\Gamma_1,C\vdash A
  }
  &
  \infer[\oplus L]
  {
    \Delta_2;\Gamma_2,A\oplus B\vdash\mathbf C
  }
  {
    \Delta_2, L(A); \Gamma_2\vdash\mathbf C
    &
    \Delta_2, R(B); \Gamma_2\vdash\mathbf C
  }
  }
\]

\[\Longrightarrow\]

\[
  \infer[cut_{\oplus_1}]
  {
    \Delta_1,\Delta_2,L(C);\Gamma_1,\Gamma_2\vdash\mathbf C
  }
  {
    \Delta_1;\Gamma_1,C\vdash A
  &
    \Delta_2, L(A); \Gamma_2\vdash\mathbf C
    &
    \Delta_2, R(B); \Gamma_2\vdash\mathbf C
  }
\]

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

